GPU-Accelerated ANNS: Quantized for Speed, Built for Change

Approximate nearest neighbor search (ANNS) is a core problem in machine learning and information retrieval applications. GPUs offer a promising path to high-performance ANNS: they provide massive parallelism for distance computations, are readily available, and can co-locate with downstream applications. Despite these advantages, current GPU-accelerated ANNS systems face three key limitations. First, real-world applications operate on evolving datasets that require fast batch updates, yet most GPU indices must be rebuilt from scratch when new data arrives. Second, high-dimensional vectors strain memory bandwidth, but current GPU systems lack efficient quantization techniques that reduce data movement without introducing costly random memory accesses. Third, the data-dependent memory accesses inherent to greedy search make overlapping compute and memory difficult, leading to reduced performance. We present Jasper, a GPU-native ANNS system with both high query throughput and updatability. Jasper builds on the Vamana graph index and overcomes existing bottlenecks via three contributions: (1) a CUDA batch-parallel construction algorithm that enables lock-free streaming insertions, (2) a GPU-efficient implementation of RaBitQ quantization that reduces memory footprint up to 8x without the random access penalties, and (3) an optimized greedy search kernel that increases compute utilization, resulting in better latency hiding and higher throughput. Our evaluation across five datasets shows that Jasper achieves up to 1.84x higher query throughput than CAGRA and achieves up to 80% peak utilization as measured by the roofline model. Jasper's construction scales efficiently and constructs indices an average of 7x faster than CAGRA while providing updatability that CAGRA lacks. Compared to BANG, the previous fastest GPU Vamana implementation, Jasper delivers 10-74x faster queries.

==> Makefile <==
DOC = main
COVER = cover_letter/cover_letter
OPTS = -pdf
LATEX = pdflatex

default: main

all: main cover

main:
	@if (command -v latexmk > /dev/null) ; then latexmk $(OPTS) $(DOC) ; else make brute; fi

cover:
	@if (command -v latexmk > /dev/null) ; then \
	  latexmk $(OPTS) -cd $(COVER) ; \
	else \
	  cd cover_letter && $(LATEX) cover_letter && $(LATEX) cover_letter ; \
	fi

cont:
	latexmk -pvc $(OPTS) $(DOC)

brute:
	$(LATEX) $(DOC)
	bibtex $(DOC)
	$(LATEX) $(DOC)
	$(LATEX) $(DOC)

clean:
	latexmk -C
	latexmk -C -cd $(COVER) || true

.PHONY: default all main cover cont brute clean





==> data/a40/bang/bigann-k1.tex <==
throughput,recall
662505.972,0.3064
301715.684,0.8729
210495.11000000002,0.9455
146002.116,0.9711
120126.34199999999,0.9817
98422.982,0.9882
95113.38,0.9911
79329.774,0.9934000000000001
68686.50200000001,0.9954999999999999
54474.60399999999,0.9973000000000001
56702.316000000006,0.9978
44856.876000000004,0.998
44763.7,0.998
47632.119999999995,0.9983
42303.406,0.9984000000000001
33222.770000000004,0.9990000000000001
11592.99,1.0


==> data/a40/bang/bigann-k10.tex <==
throughput,recall
286210.916,0.679
189846.152,0.8618000000000001
147620.352,0.9242
113698.648,0.9521999999999999
113586.72,0.9669
94261.29000000001,0.9756
78568.72400000002,0.9812000000000001
76352.602,0.9853000000000001
71334.52600000001,0.9882
59085.09199999999,0.9902
58457.454000000005,0.9918
54786.6,0.993
48658.13,0.9940000000000001
44871.456,0.9948
43624.214,0.9954999999999999
41807.908,0.9961
39907.394,0.9965
36957.432,0.9969
35387.914,0.9972
33761.8,0.9975
21648.536,0.9990000000000001
14699.12,0.9994
11726.088,0.9997


==> data/a40/bang/bigann-k50.tex <==
throughput,recall
81909.94600000001,0.7567
86671.13600000001,0.8210999999999999
78961.988,0.8665
64585.224,0.8987999999999999
67521.89000000001,0.9218999999999999
59262.512,0.9390999999999999
55248.478,0.9512999999999999
53847.578,0.9608
50884.04,0.9679000000000001
44992.036,0.9732999999999999
40297.072,0.9777
40428.426,0.981
39469.96000000001,0.9836
35484.172,0.9858
30593.958000000002,0.9876
32313.528000000002,0.9891
26854.958000000002,0.9937
22182.934,0.9958
18549.238,0.9971
14912.025999999998,0.9978
11728.84,0.9986


==> figures/construction/bigann_subfig.tex <==
%subfigure code - belongs to a full figure
\begin{subfigure}{.3\textwidth}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    insertPlot,
    legend to name=insertLegend,
    legend columns = 6,
    xlabel={Dataset Size},
    legend style={font=\small},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/jasper_bigann.txt};

    \addplot[cagraStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/cagra_bigann.txt};
    %  \addplot[jasperRqStyle] table [ x expr=\thisrowno{5}, y expr=\thisrowno{4}] {data/a40/jasper/bigann-k1-rabitq.txt};
    % \addplot[cagraStyle] table [ x expr=\thisrowno{1}, y expr=\thisrowno{0}] {data/a40/cagra/bigann-k1.txt};
    \addplot[parlayStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/parlay_bigann.txt};

    \addplot[gannsStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/ganns_bigann.txt};
    
    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
 
    \legend{Jasper, \cagra, \parlayann, GANNS}
    
  \end{axis}
  \end{tikzpicture}
  \caption{BigANN construction 1M-10M}
  \label{fig:bigann_construct}
\end{subfigure}

==> figures/construction/construction.tex <==
\begin{figure*}[t]
    \centering
    \ref{insertLegend}
    
    \input{figures/construction/bigann_subfig}\hfill
    \input{figures/construction/deep_subfig}\hfill
    \input{figures/construction/gist_subfig}\hfill

    \caption{Construction performance on A100.}

    \label{fig::construction}
    \vspace{-.5em}
\end{figure*}

==> figures/construction/deep_subfig.tex <==
%subfigure code - belongs to a full figure
\begin{subfigure}{.3\textwidth}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    insertPlot,
    legend columns = 6,
    xlabel={Dataset Size},
    legend style={font=\small},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=points, y=throughput]{data/a100/construction/jasper_deep.txt};

    \addplot[cagraStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/cagra_deep.txt};
    %  \addplot[jasperRqStyle] table [ x expr=\thisrowno{5}, y expr=\thisrowno{4}] {data/a40/jasper/bigann-k1-rabitq.txt};
    % \addplot[cagraStyle] table [ x expr=\thisrowno{1}, y expr=\thisrowno{0}] {data/a40/cagra/bigann-k1.txt};
    \addplot[parlayStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/parlay_deep.txt};

    \addplot[gannsStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/ganns_deep.txt};
    
    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
    
  \end{axis}
  \end{tikzpicture}
  \caption{Deep construction 1M-10M}
  \label{fig:deep_construct}
\end{subfigure}

==> figures/construction/gist_subfig.tex <==
%subfigure code - belongs to a full figure
\begin{subfigure}{.3\textwidth}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    insertPlot,
    legend columns = 6,
    xlabel={Dataset Size},
    legend style={font=\small},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=points, y=throughput]{data/a100/construction/jasper_gist.txt};

    \addplot[cagraStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/cagra_gist.txt};
    %  \addplot[jasperRqStyle] table [ x expr=\thisrowno{5}, y expr=\thisrowno{4}] {data/a40/jasper/bigann-k1-rabitq.txt};
    % \addplot[cagraStyle] table [ x expr=\thisrowno{1}, y expr=\thisrowno{0}] {data/a40/cagra/bigann-k1.txt};
    \addplot[parlayStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/parlay_gist.txt};

    \addplot[gannsStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/ganns_gist.txt};
    
    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
    
  \end{axis}
  \end{tikzpicture}
  \caption{Gist construction 100k-1M}
  \label{fig:gist_construct}
\end{subfigure}

==> figures/loads/load_tiled.tex <==
\begin{subfigure}[t]{.2\textwidth}
\centering
\begin{tikzpicture}[x=0.15\textwidth, y=0.05\textwidth] % scale to fit subfigure
  % force a bounding box to ensure horizontal alignment
  \useasboundingbox (0,-1) rectangle (8,4);  % adjust to cover your drawing

  % define colors
  \definecolor{cadmium}{HTML}{F28C28}
  \definecolor{celadon}{HTML}{AFE1AF}
  \definecolor{periwinkle}{HTML}{CCCCFF}

  % helper commands
  \newcommand{\roundedbox}[5]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}  % width
      \def\H{#4}  % height
      \def\R{0.25cm} % corner radius
      \draw[thick, rounded corners=\R] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }
  \newcommand{\colorroundedbox}[6]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}  % width
      \def\H{#4}  % height
      \def\R{0.25cm} % corner radius
      \draw[thick, rounded corners=\R, fill=#6] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }

  % drawing content
  \draw[thick, black](0,3.25) node [anchor=west]{Warp};
  \colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
  \colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
  \colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
  \colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

  \draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
  \roundedbox{0}{0}{10}{1}{}

  % colored slices
  \foreach \x in {0,0.5,...,7.5} {
    \pgfmathparse{int(mod(\x*2,4))}
    \edef\c{\pgfmathresult}
    \ifnum\c=0 \colorroundedbox{\x}{0}{0.5}{1}{}{pink} \fi
    \ifnum\c=1 \colorroundedbox{\x}{0}{0.5}{1}{}{periwinkle} \fi
    \ifnum\c=2 \colorroundedbox{\x}{0}{0.5}{1}{}{celadon} \fi
    \ifnum\c=3 \colorroundedbox{\x}{0}{0.5}{1}{}{cadmium} \fi
  }

  % draw diagram line
  \draw[thick] (0, 0) -- (0, -.25) -- (2,-.25) -- (2,0) -- (2,-.25) -- (1,-.25) -- (1,-.5);
  \draw[thick, black](2.25,-.5) node [anchor=north]{1-4 Bytes loaded per thread per round};

\end{tikzpicture}
\caption{Tiled load strategy}
\label{fig::cache_diagram}
\end{subfigure}


==> figures/loads/loads.tex <==
\begin{figure}[t]
\centering

% ===== Subfigure 1 =====
\begin{subfigure}[t]{.45\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
  \useasboundingbox (0,-1) rectangle (10,4);

  % Colors
  \definecolor{cadmium}{HTML}{F28C28}
  \definecolor{celadon}{HTML}{AFE1AF}
  \definecolor{periwinkle}{HTML}{CCCCFF}

  % Helper commands
  \newcommand{\roundedbox}[5]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }
  \newcommand{\colorroundedbox}[6]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R, fill=#6] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }

  % Diagram content
  \draw[thick, black](0,3.25) node [anchor=west]{Warp};
  \colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
  \colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
  \colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
  \colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

  \draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
  \roundedbox{0}{0}{10}{1}{}

  % Colored slices
  \foreach \x/\c in {0/pink, 0.5/periwinkle,1/celadon,1.5/cadmium,
                     2/pink,2.5/periwinkle,3/celadon,3.5/cadmium,
                     4/pink,4.5/periwinkle,5/celadon,5.5/cadmium,
                     6/pink,6.5/periwinkle,7/celadon,7.5/cadmium} {
    \colorroundedbox{\x}{0}{0.5}{1}{}{\c}
  }

  % Vertical lines
  % \foreach \x in {0.5,1,1.5,2.5,3,3.5,4.5,5,5.5,6.5,7,7.5} {
  %   \draw[thick] (\x,0) -- (\x,1);
  % }

  % Bottom diagram line
  \draw[thick] (0,0) -- (0,-.25) -- (2,-.25) -- (2,0) -- (2,-.25) -- (1,-.25) -- (1,-.5);
  \draw[thick, black](2,-.5) node [anchor=north]{1-4 Bytes loaded per thread per round};
\end{tikzpicture}%
}
\caption{Tiled load strategy}
\label{fig::cache_diagram1}
\end{subfigure}


% ===== Subfigure 2 =====
\begin{subfigure}[t]{.45\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
  \useasboundingbox (0,-1) rectangle (10,4);

  % Colors
  \definecolor{cadmium}{HTML}{F28C28}
  \definecolor{celadon}{HTML}{AFE1AF}
  \definecolor{periwinkle}{HTML}{CCCCFF}

  % Helper commands
  \newcommand{\roundedbox}[5]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }
  \newcommand{\colorroundedbox}[6]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R, fill=#6] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }

  % Diagram content
  \draw[thick, black](0,3.25) node [anchor=west]{Warp};
  \colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
  \colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
  \colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
  \colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

  \draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
  \roundedbox{0}{0}{10}{1}{}

  % Colored slices
  \foreach \x/\c in {0/pink,2/periwinkle,4/celadon,6/cadmium} {
    \colorroundedbox{\x}{0}{2}{1}{}{\c}
  }

  % Vertical lines
  \foreach \x in {0.5,1,1.5,2.5,3,3.5,4.5,5,5.5,6.5,7,7.5} {
    \draw[thick] (\x,0) -- (\x,1);
  }

  % Bottom diagram line
  \draw[thick] (0,0) -- (0,-.25) -- (8,-.25) -- (8,0) -- (8,-.25) -- (4,-.25) -- (4,-.5);
  \draw[thick, black](4,-.5) node [anchor=north]{16 Bytes loaded per thread per round};
\end{tikzpicture}%
}
\caption{Chunked load strategy}
\label{fig::cache_diagram2}
\end{subfigure}

\caption{Comparison of the two different load strategies tested in Jasper: tiled loads load one object per thread in the tile at a time, whereas the chunked load strategy loads a fixed amount of data (16 bytes) per thread and has each thread work on all objects loaded in that chunk.}
\label{fig:load_strategies}
\end{figure}

\begin{figure}
    \centering
    %TODO: Decide which one to use
    \includegraphics[width=\linewidth]{figures/graphs/tiled_vs_chunked.pdf}
    \includegraphics[width=\linewidth]{figures/graphs/tiled_vs_chunked_graph_only.pdf}
    \caption{Comparison of the two different load strategies tested in Jasper: tiled loads load one object per thread in the tile at a time, whereas the chunked load strategy loads a fixed amount of data (16 bytes) per thread and has each thread work on all objects loaded in that chunk.}
\end{figure}


==> figures/loads/old_load_coalesced.tex <==

%visualization of \parlayann algorithm
\begin{subfigure}{.2\textwidth}
\centering
% \begin{tikzpicture}[line width=3pt,rounded corners=3pt, x=0.5cm, y=0.5cm]

\newcommand{\roundedbox}[5]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\newcommand{\colorroundedbox}[6]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R, fill=#6]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\makebox[\linewidth][c]{%
\begin{tikzpicture}[
    membox/.style={draw, rounded corners=2pt, minimum width=2.2cm, minimum height=0.8cm, align=center},
    block/.style={draw, minimum height=0.9cm, rounded corners=1pt},
    subblock/.style={draw, minimum height=0.9cm, minimum width=0.9cm},
    warp/.style={draw, fill=gray!8, rounded corners=1pt, minimum height=0.8cm},
    small/.style={draw, minimum height=0.55cm, minimum width=0.9cm},
    arrowstyle/.style={thick},
    baseline=(current bounding box.north),
    scale=1
]

\definecolor{cadmium}{HTML}{F28C28}

\definecolor{celadon}{HTML}{AFE1AF}

\definecolor{periwinkle}{HTML}{CCCCFF}



\draw[thick, black](0,3.25) node [anchor=west]{Warp};

\colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
\colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
\colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
\colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

% \roundedbox{0}{2}{1.5}{1}{Thread 1}
% \roundedbox{1.6}{2}{1.5}{1}{Thread 2}
% \roundedbox{3.2}{2}{1.5}{1}{Thread 3}
% \roundedbox{4.8}{2}{1.5}{1}{Thread 4}

\draw[thick, black](0,1.25) node [anchor=west]{Data Vector};

\roundedbox{0}{0}{10}{1}{}

\colorroundedbox{0}{0}{2}{1}{}{pink}
\colorroundedbox{2}{0}{2}{1}{}{periwinkle}
\colorroundedbox{4}{0}{2}{1}{}{celadon}
\colorroundedbox{6}{0}{2}{1}{}{cadmium}


%new lines
\draw[thick] (.5, 0) -- (0.5, 1) node [anchor=west] {};
\draw[thick] (1, 0) -- (1, 1) node [anchor=west] {};
\draw[thick] (1.5, 0) -- (1.5, 1) node [anchor=west] {};

\draw[thick] (2.5, 0) -- (2.5, 1) node [anchor=west] {};
\draw[thick] (3, 0) -- (3, 1) node [anchor=west] {};
\draw[thick] (3.5, 0) -- (3.5, 1) node [anchor=west] {};

\draw[thick] (4.5, 0) -- (4.5, 1) node [anchor=west] {};
\draw[thick] (5, 0) -- (5, 1) node [anchor=west] {};
\draw[thick] (5.5, 0) -- (5.5, 1) node [anchor=west] {};

\draw[thick] (6.5, 0) -- (6.5, 1) node [anchor=west] {};
\draw[thick] (7, 0) -- (7, 1) node [anchor=west] {};
\draw[thick] (7.5, 0) -- (7.5, 1) node [anchor=west] {};

\draw[thick] (0, 0) -- (0, -.25) -- (8,-.25) -- (8,0) -- (8,-.25) -- (4,-.25) -- (4,-.5) node [anchor=west] {};

\draw[thick, black](4,-.5) node [anchor=north]{16 Bytes loaded per thread per round};


%Strat 1 - tiled load
%Have colored slices taken from the beveling?



\end{tikzpicture}
}
\caption{Chunked load strategy }
\label{fig::cache_diagram}
\end{subfigure}




==> figures/loads/old_load_tiled.tex <==

%visualization of \parlayann algorithm
\begin{subfigure}{.2\textwidth}
\centering
% \begin{tikzpicture}[line width=3pt,rounded corners=3pt, x=0.5cm, y=0.5cm]

\newcommand{\roundedbox}[5]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\newcommand{\colorroundedbox}[6]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R, fill=#6]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\makebox[\linewidth][c]{%
\begin{tikzpicture}[
    membox/.style={draw, rounded corners=2pt, minimum width=2.2cm, minimum height=0.8cm, align=center},
    block/.style={draw, minimum height=0.9cm, rounded corners=1pt},
    subblock/.style={draw, minimum height=0.9cm, minimum width=0.9cm},
    warp/.style={draw, fill=gray!8, rounded corners=1pt, minimum height=0.8cm},
    small/.style={draw, minimum height=0.55cm, minimum width=0.9cm},
    arrowstyle/.style={thick},
    baseline=(current bounding box.north),
    scale=1
]

\definecolor{cadmium}{HTML}{F28C28}

\definecolor{celadon}{HTML}{AFE1AF}

\definecolor{periwinkle}{HTML}{CCCCFF}

\draw[thick, black](0,3.25) node [anchor=west]{Warp};

\colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
\colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
\colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
\colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

\draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
\roundedbox{0}{0}{10}{1}{}


\colorroundedbox{0}{0}{.5}{1}{}{pink}
\colorroundedbox{.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{1}{0}{.5}{1}{}{celadon}
\colorroundedbox{1.5}{0}{.5}{1}{}{cadmium}

\colorroundedbox{2}{0}{.5}{1}{}{pink}
\colorroundedbox{2.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{3}{0}{.5}{1}{}{celadon}
\colorroundedbox{3.5}{0}{.5}{1}{}{cadmium}

\colorroundedbox{4}{0}{.5}{1}{}{pink}
\colorroundedbox{4.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{5}{0}{.5}{1}{}{celadon}
\colorroundedbox{5.5}{0}{.5}{1}{}{cadmium}

\colorroundedbox{6}{0}{.5}{1}{}{pink}
\colorroundedbox{6.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{7}{0}{.5}{1}{}{celadon}
\colorroundedbox{7.5}{0}{.5}{1}{}{cadmium}

%draw diagram
\draw[thick] (0, 0) -- (0, -.25) -- (2,-.25) -- (2,0) -- (2,-.25) -- (1,-.25) -- (1,-.5) node [anchor=west] {};

\draw[thick, black](2.25,-.5) node [anchor=north]{1-4 Bytes loaded per thread per round};


%Strat 1 - tiled load
%Have colored slices taken from the beveling?

\end{tikzpicture}
}
\caption{Tiled load strategy}
\label{fig::cache_diagram}
\end{subfigure}




==> figures/query_100_recall.tex <==
\begin{figure*}[t]
    \centering
    \ref{queryLegend100}
    
    \input{figures/a100-bigann-k100}\hfill
    \input{figures/a100-deep-k100}\hfill
    \input{figures/a100-gist-k100}\hfill
    \input{figures/a100-openai-k100}\hfill
    \input{figures/a100-t2i-k100}
    \caption{100@100 recall/throughput curves for all datasets on A100. X-axis is 100@100 recall, y-axis is throughput in queries oper second.}

    \label{fig::query_100_recall}
    \vspace{-.5em}
\end{figure*}

==> figures/roofline/bigann_roofline.tex <==
\begin{subfigure}{.45\columnwidth}
\centering
\begin{tikzpicture}
\begin{loglogaxis}[
    rooflinePlot,
    xlabel={Operational Intensity (OP/Byte)},
    ylabel={Performance (TOP/s)},
    legend to name=rooflineLegend,
    legend columns = 2,
    xtick={0.1, 1, 10, 100, 1000},
]

\addplot[jasperThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/bigann_jasper.txt};

\addplot[jasperRqThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/bigann_rq.txt};

% Memory bandwidth bound (A100 HBM2e: ~1.7 TB/s measured)
\addplot[black, thick, domain=0.01:12.2] {1.7e12*x/1e12};

% Compute bound (A100: ~20.74 TFLOP/s FP32 equivalent)
\addplot[black, thick, domain=12.2:1000000] {20.74e12/1e12};

% Ridge point line
\addplot[
    densely dotted,
    thick,
    black
] coordinates {(12.2,1e-3) (12.2,1e3)};

\legend{\sysname, \sysnameRQ}

\end{loglogaxis}
\end{tikzpicture}
\caption{Roofline model for \bigann when k=10}
\end{subfigure}


==> figures/tables/memory_breakdown.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c c c|c|}
 \toprule
 Component & \sysname & \cagra (NN-Descent) & \cagra (IVF) & Notes \\
 \midrule
 Raw vectors                & 38.5\,GB & 38.5\,GB & 38.5\,GB & Same input \\
 Graph index                & 25.6\,GB & 25.6\,GB & 25.6\,GB & R=64 \\
 Construction workspace     &  8.0\,GB & $\approx$\,90\,GB & 8.0\,GB & PRELIM --- pending collaborator confirm \\
 \midrule
 \textbf{Peak device memory}& \textbf{72.1\,GB} & $\approx$\,150\,GB & 72.1\,GB & A100 has 80\,GB; H200 has 140\,GB \\
 Fits on A100 (80\,GB)?     & yes      & no  & yes  & \\
 Fits on H200 (140\,GB)?    & yes      & no  & yes  & at 200M points \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{Construction memory footprint at \deep 100M. \sysname keeps the full
construction pipeline inside device memory; \cagra's NN-Descent pass exceeds
the device budget and falls back to its IVF construction path, sacrificing
graph quality. \emph{Numbers marked PRELIM are pending collaborator
confirmation.}}
\label{tab::memory_breakdown}
\end{table*}


==> figures/tables/reordering.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{| c | r r r r | r |} 
 \toprule
 Dataset & Jasper & Jasper (R) & Jasper Host & Jasper Host (R) & Vector Size (bytes)\\  
 \midrule
 \bigann & 1,492,730 & 1,427,520 & 14,098 & 17,212 & 128 \\
 \deep & 1,185,880 & 1,149,740 & 7,781 & 7,161 & 384 \\
 \gist & 96,881 & 96,741 & 864 & 800 & 3,840\\
 \openai & 62,883 & 69,413 & 421 & 416 & 6,144 \\
 \textToImage & 473,087 & 472,540 & 3,561 & 3,708 & 800 \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{Query throughput for the original vs reordered graph when beam width = 64 and K=50. Results presented are Kiloqueries per second.}
\label{tab::reordering}
\end{table}


==> pseudocode/cudaBeam.tex <==
\RestyleAlgo{ruled}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\SetArgSty{textrm} 
\begin{algorithm}

unvisited\_frontier = []\\
visited = []\\
\ForEach{key \textbf{in} batch \textbf{in parallel}}{%
      frontier[key] = {<key,medoid, 0>} \tcp{Distances start unitialized}
}
calculate\_distances(frontier) \tcp{Set distances}
unvisited\_frontier = set\_difference(frontier, visited)\\
\While{unvisited\_frontier.size() != 0}{%
    live\_frontier = []\\
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{
        \tcp{Grab the first W from each key in the batch}
        live\_frontier[key] = unvisited\_frontier[key:key+W]  
    }
    candidates = []\\
    \ForEach{edge \textbf{in} live\_frontier \textbf{in parallel}}{%
    candidates[edge] = graph[edge]
    }
    calculate\_distances(candidates)\\
    sort\_by\_distance(candidates)\\
    frontier = merge(frontier, candidates)\\
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{%
        frontier[key] = clip(frontier[key], beam\_width) \tcp{clip to beam width}
    }
    visited = merge(visited, live\_frontier)\\
    unvisited\_frontier = set\_difference(frontier, visited)\\
}
\textbf{Return} \{frontier, visited\}
\caption{Cuda Beam search}
\label{pseudo::cudaBeam}
\end{algorithm}


==> pseudocode/cudaPrune.tex <==
\RestyleAlgo{ruled}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\SetArgSty{textrm} 
\begin{algorithm}

work_list_id = blockDim.x;\\
tile = cg::tiled_partition<thread_block>;\\
write\_index = 0;\\
index = 0;\\
my\_edges = edges[work\_list\_id];\\
node my\_vertex = my\_edges[0].source;\\

\tcp{Iterate until edge list is full.}
\While{write\_index < R && index < my\_edges.size()}{

    \uIf{my\_edges[index] == dead\_edge}{
        index++;\\
        continue;\\
    }

    \tcp{Only one thread writes output.}
    \uIf{threadIdx.x == 0}{
        graph[my\_vertex].edges[write\_index] = my\_edges[index].sink;
    }

    \ForEach{clippable\_edge \textbf{in} my\_edges[index+1:] \textbf{in parallel}}{

        p\_star = my\_edges[index].sink;
        p\_prime = clippable\_edge.sink;
    
    }
    
    
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{
        \tcp{Grab the first W from each key in the batch}
        live\_frontier[key] = unvisited\_frontier[key:key+W]  
    }
    candidates = []\\
    \ForEach{edge \textbf{in} live\_frontier \textbf{in parallel}}{%
    candidates[edge] = graph[edge]
    }
    calculate\_distances(candidates)\\
    sort\_by\_distance(candidates)\\
    frontier = merge(frontier, candidates)\\
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{%
        frontier[key] = clip(frontier[key], beam\_width) \tcp{clip to beam width}
    }
    visited = merge(visited, live\_frontier)\\
    unvisited\_frontier = set\_difference(frontier, visited)\\
}
\textbf{Return} \{frontier, visited\}
\caption{Cuda robustPrune implementation}
\label{pseudo::cudaBeam}
\end{algorithm}


==> pseudocode/parlayANN.tex <==
\RestyleAlgo{ruled}

\begin{algorithm}
\SetArgSty{textrm} 

flipped$\_$edges = []\\
\ForEach{key \textbf{in} batch \textbf{in parallel}}{%
      visited$_{\texttt{key}}$ = beamSearch(key)\\
      neighbors$_{\texttt{key}}$ = robustPrune(visited$_{\texttt{key}}$)\\
      graph[key].edges =  neighbors$_{\texttt{key}}$\\
      flipped = flip$\_$edges(neighbors$_{\texttt{key}}$)\\
      flipped$\_$edges.append(flipped)\\
}
semisorted$\_$edges = semisort(flipped$\_$edges)\\
\ForEach{key, edges \textbf{in} semisorted\_edges \textbf{in parallel}}{
  \uIf{graph[key].size() + len(edges) <= R}{
    graph[key].edges += edges
  } \Else {
    pruned = robustPrune(graph[key].edges+edges)\\
    graph[key].edges = pruned
  }

}
\label{pseudo::parlayANN}
\caption{Batch insertion in \parlayann}
\end{algorithm}


==> related.tex <==
\section{Related work}

\label{sec::related}

In this section, we discuss the current state of the art in ANNS indexes that
are not directly evaluated against \sysname. These are indexes that are either
1) superseded in performance by the current state-of-the-art, 2) do not have a
publicly available implementation, or 3) are complementary to ANNS but not
directly comparable.

% Listing all related works worth mentioning. There are like 50 so will focus on diskANN and GPU related.
% \begin{itemize}
%     \item NSG
%     \item filteredDiskANN
%     \item scann
%     \item spann
% \end{itemize}


% \paragraph{\textbf{DiskANN}} DiskANN~\cite{Subramanya2019} is a graph-based index that performs ANN by constructing and querying a navigable search graph. The graph is queried by a greedy beam search in which a small number of close neighbors are held in memory, and in iterative steps the closest vertex to the target is queried for its neighbor list. The graph is constructed using the Vamana algorithm, which is discussed in more detail in \Cref{sec::diskann}.
% % In this algorithm, each vector in the dataset is represented by a vertex. This vertices are initialized to have random neighbors, and the graph is then iteratively improved. Each vertex in the graph is queried one at a time in random order. The nodes visited along the way are used to generate a new neighborhood for the vertex, and the vertex is bidirectionally attached to them. When the degree of a node becomes too large, a pruning algorithm calle d robustPrune is run. This pruning strategy admits only the closest neighbors and prunes any neighbors who have close 2-hop connectivity. The exact details of this algorithm are discussed in more detail in \cref{sec::diskann}.

% % The original implementation of this algorithm could not efficiently delete as they leave holes in the graph that impact output quality. FreshDiskANN~\cite{https://doi.org/10.48550/arxiv.2105.09613} uses a lazy deletion algorithm to process deletes: nodes are marked as deleted but left in the graph, and when enough nodes are deleted a stop-the-world approach is used. The graph is frozen and the ingoing neighbors of each node are connected to all outgoing neighbors of each node, with robustPrune executed on all of them. As nodes do not store their incoming neighbors, this results in a costly traverse of the entire graph.

% % IPDiskANN~\cite{https://doi.org/10.48550/arxiv.2502.13826} reduces the cost of deletions by performing them on-the-fly and in place. To generate the incoming neighbors of a deleted vertex, greedySearch is run. A parameter $c$ controls how densely the in and out-going neighbors are connected. The incoming neighbors of the deleted node are connected to the ANN results of the greedy search. The outgoing neighbors of the deleted node are connected to the visited set.

% % All of these implementations are parallelized using locks, which adds unnecessary overhead to parallel operations. \parlayann~\cite{Manohar2024} uses a batched and lock-free insertion algorithm to efficiently add new nodes to the graph. More detail on this algorithm is given in \Cref{sec::parlay}.

% \bang~\cite{Venkatasubba2025} extends the query execution of diskANN to GPUs. The product quantized vectors are stored in GPU memory, with the graph and full vector data stored in DRAM. To process queries more efficiently, bloom filters are used to represent the visited list, lowering the memory requirements for searching.


\para{\textbf{FAISS}} FAISS~\cite{FAISS} is a library for efficient similarity
search and clustering of vectors. It provides a broad collection of approximate
and exact nearest neighbor algorithms, with efficient CPU and GPU
implementations. FAISS supports multiple indexing strategies and techniques,
including inverted file indexes, product quantization, three-level
quantization, HNSW, anisotropic vector quanitization, NSG, and binary
multi-index hashing. On GPUs, FAISS leverages massive parallelism to accelerate
both index construction and query processing, making it a common choice for
large-scale similarity search workloads.



% % \paragraph{\textbf{HNSW}} HNSW~\cite{Malkov2020} constructs a probabilistic search graph akin to a skip list. In HNSW, the graph is split into levels. Each level of the graph is connected, with queries starting at the top level and bleeding down through the graph. The top level of the graph contains long range connections, with the lower level graphs having shorter and more dense edges. When new vertices are added to the graph a random roll is used to determine to how many levels the object will belong.

% \paragraph{\textbf{CAGRA}} \cagra~\cite{ootomo2024} is a GPU ANN algorithm built on top of NNDescent~\cite{Dong2011}. NNDescent takes a graph and iteratively improves the neighborhood of nodes by pulling new neighbors from their 2-hop neihgborhood. This provides a good ANN query graph, but the degree is too high for use on GPU. To reduce the memory use, \cagra executes a pruning algorithm after the graph is constructed. This prune occurs in three phases. In the first phase, the edges of each node are sorted in ascending order by their length. This ordering is then used in the second phase as a proxy for distance. In the second phase, any nodes that are directly connected but have a good 2-hop route will have their edge clipped. To avoid PQ vector comparisons in this phase, the distance between two nodes is approximated by the ranking of their edge in the outgoing vertex's edge list. This allows for this phase to be executed quickly inside of GPU memory. Finally, the graph duplicated and reversed, and the two graphs are merged together, with a final pruning pass being executed to reduce the size.

\para{\textbf{SONG}} SONG~\cite{Zhao2020} is a GPU ANNS that uses a fixed-rank
ANN search graph for ANN queries. SONG uses bulk computation processing, a
priority queue, and a cuckoo-filter to efficiently process queries. To improve
performance, the algorithm only considers vertices with a distance smaller than
those in the current Top-K. This reduces the number of vertices that need to be
remembered, but comes at the cost of additional compute to re-measure
distances. They additionally optimize hash table/filter usage by deleting keys
that fall out of the current top-\textit{K}, as these nodes can't be re-added
to the search due to having too far of a distance from the query.

\para{\textbf{GTS}} GTS~\cite{Zhu2024} is a GPU tree-based ANN index for exact
K-nearest neighbors. This tree is constructed using a bulk-synchronous
algorithm. Along with the main tree structure, the node value for each vector
is written into a table. Objects are mapped to nodes using a FFT pivot
selection, and the list is partitioned to place the objects contiguously next
to each other in device memory. This process repeats to further partition nodes
until all leaves in the tree are sufficiently small. A bulk \textit{cache list}
is used to record streaming updates until a sufficient number of updates are
recorded. The entire tree structure is then recomputed. For queries, they
utilize a batched algorithm based on iterative range queries: A list of the
top-$K$ closest nodes is kept, and all children in a level are considered
unless their distance from the query falls outside of the top-$K$ largest
distance - this search is iteratively refined until the leaves are reached and
a final set of top-$K$ results can be extracted. During updates, new keys are
held in a buffer that is checked during every query. If the buffer becomes too
large, then entire tree is regenerated.

\para{\textbf{NEOS}} NEOS~\cite{Huang2024} is an ANNS tool library that pins
GPU memory in CPU user space and offers several optimizations to improve GPU
buffer design such as pinning NVME memory, custom CPU to GPU memory copies, and
faster CPU-GPU polling. NEOS is not a vector index but instead is a buffer tool
that can be used by other indices such as HSNW. NEOS uses a large unsorted
buffer to aggreagate incoming requests; using the parallelism of an A100 and
cuBLAS matrix operations, the entirety of the buffer can be checked with low
latency. This allows for other vector managers to process streaming updates
while only possessing a batch insertion API, which can make these applications
more flexible without compromising throughput.

\para{\textbf{FusionANNs}} FusionANNs~\cite{305214} is a coprocessor vector
index that uses the GPU as a helper for performing expensive distance
comparisons. The index is based off of the posting lists used in SPANN - the
authors find that the main limit to scalability in the original SPANN algorithm
is the distance comparisons used when selecting the top-$K$ from posting lists.
Therefore, the product-quantized representation of the vectors is kept on GPU
memory. Posting lists are generated by using hierarchical balanced
clustering~\cite{Hartigan1979}. During a query, the CPU traverses the graph to
find the closest posting lists to the target query. The IDs from these posting
lists are sent to the GPU, and the distances for every item in the lists is
calculated in parallel. This listing is returned to the CPU, where a heuristic
re-ranking algorithm is executed to locate the best vectors. The full vectors
are then loaded from SSD, and an exact distance comparison is executed to
determine the final set. The code for FusionANNs is not publicly available.

\para{\textbf{LoRANN}} LoRANN~\cite{NEURIPS2024_b939da39} introduces a new
clustering methods called reduced-rank regression (RRR). This method is a
built-in replacement for product quantization, and can be used both in setting
clusters and for querying the posting lists of a cluster from the IVF. In RRR,
the data is processed as a full batch, with the goal of minimizing the value of
$\beta_{RRR} = argmin_{\beta} \Vert Y-X\beta \Vert^2_F$, where $Y$ are the true
nearest neighbors. A fast randomized algorithm is used to compute the nearest
neighbors of the training set, and predictions are made via a matrix
multiplication $\hat{y} = x^T\beta_{RRR}$. To perform operations efficiently,
the training set is first cast into a low-dimensional space by taking the
eigenvectors from PCA. The result of this is then quantized via 8-bit integer
quantization. These operations can be efficiently processed on both CPU and
GPU. In testing, the authors find that their implementation can replace PQ in
FAISS to improve performance on high-dimensional vector datasets.

% \paragraph{\textbf{GGNN}} GGNN is a KNN-based nearest neighbors algorithm parallelized for use on GPUs. The algorithm is performed in hierarchical rounds, with subgraphs being iteratively merged into a final hierarchical search graph. The connection algorithm utilizes a greedy search that terminates when the best list cannot be improved.
% To optimize for the GPU, a per-block heap and priority queue are used for searching. Entire thread blocks are allocated for individual keys. In queries, a slack value is used to stop queries from getting stuck in local minima.

% \paragraph{\textbf{GANN}} GANN is an implementation of the NSW graph algorithm optimized for GPUs. The main improvement is the use of lazy data structures - rather than maintain a priority queue, GANN maintains two lists (frontier and visited) and only occasionally updates the lists to mark vertices as visited. They avoid the use of a hash table for marking visited vertices during queries, and use multiple thread blocks per query. The construction algorithm for an NSW graph is non-trivial to parallelize, so the authors build many small graphs in parallel and then sequentially merge them.
%\subsection{Where we stand/So far}. Currently, we have a fully implemented version of \parlayann (vamana) running on the GPU. On the BigANN10M dataset, we get construction performance of 60.4K vectors added per second, compared to a peak throughput of 38.9K for cuVS! Recall with L=64, R=64 is .9858@1, 9.656@10, and 46.23@50 with full vectors. With all objects placed on host, throughput is 3.934K/s due to the increased cost of object transfer. PQ vectors are currently not working due to the distance calculation not using the distances between the centroids.


==> vldb26-revision/Makefile <==
DOC = main
COVER = cover_letter/cover_letter
OPTS = -pdf
LATEX = pdflatex

default: main

all: main cover

main:
	@if (command -v latexmk > /dev/null) ; then latexmk $(OPTS) $(DOC) ; else make brute; fi

cover:
	@if (command -v latexmk > /dev/null) ; then \
	  latexmk $(OPTS) -cd $(COVER) ; \
	else \
	  cd cover_letter && $(LATEX) cover_letter && $(LATEX) cover_letter ; \
	fi

cont:
	latexmk -pvc $(OPTS) $(DOC)

brute:
	$(LATEX) $(DOC)
	bibtex $(DOC)
	$(LATEX) $(DOC)
	$(LATEX) $(DOC)

clean:
	latexmk -C
	latexmk -C -cd $(COVER) || true

.PHONY: default all main cover cont brute clean





==> vldb26-revision/abstract.tex <==
\begin{abstract}

Approximate nearest neighbor search (ANNS) is a core problem in machine
learning and information retrieval. GPUs offer a promising path to
high-performance ANNS through massive parallelism and co-location with
downstream applications, but current GPU indices face three limitations:
inability to update without full rebuilds, lack of efficient quantization for
high-dimensional vectors, and poor latency hiding due to data-dependent memory
accesses.

We present \sysname, a GPU-native ANNS system built on the Vamana graph index
that achieves both high query throughput and full updatability via three new
techniques: (1) a batch-parallel construction algorithm enabling lock-free
streaming insertions, (2) a GPU-efficient \RQ implementation that reduces
memory footprint up to 8$\times$ without random access penalties, and (3) an
optimized search kernel with improved compute utilization and latency hiding.

Across five datasets, \sysname achieves up to \timesFasterThanCagra$\times$
higher throughput than \cagra, the current
state-of-the-art GPU index, while providing updatability that \cagra lacks,
constructs indices \avgConstruct faster on average, and delivers
\lowerBangSpeedup–\higherBangSpeedup$\times$ faster queries than \bang, the
previous fastest GPU Vamana implementation.

\end{abstract}


\if 0
\begin{abstract}

Approximate nearest neighbor search (ANNS) is a core problem in several machine
learning and information retrieval applications. 
% Among the various approaches, graph-based ANNS techniques offer superior
% trade-off between throughput and accuracy via greedy search over navigable
% graphs.
GPUs offer a promising path to high-performance ANNS: they provide massive
parallelism for distance computations, are readily available in modern data
centers, and can co-locate with downstream applications to reduce data
movement.

However, current GPU-accelerated ANNS systems face three key
limitations. First, applications operate on evolving datasets that
require fast batch updates, yet most GPU indices must be rebuilt from scratch
when new data arrives. Second, high-dimensional vectors strain memory
bandwidth, but current GPU systems lack efficient quantization techniques to
reduce data movement without introducing costly random memory accesses. Third,
the data-dependent memory accesses inherent to greedy search make overlapping
compute and memory difficult, leading to reduced performance.

We present \sysname, a GPU-native ANNS system that achieves both high query
throughput and full updatability. \sysname builds on the Vamana graph index and
overcomes existing bottlenecks via three contributions: 
% We present \sysname, a GPU-native ANNS system built on the Vamana graph index
% that supports both high query throughput and updatability. \sysname addresses
% the key bottlenecks of GPU-based ANNS systems through three major
% contributions:
(1) a batch-parallel construction algorithm adapted for CUDA
that enables lock-free streaming insertions, (2) a GPU-efficient implementation
of \RQ quantization that reduces memory footprint up to 8$\times$ without the
random access penalties, and (3) an optimized greedy search kernel that
increases compute utilization, resulting in better latency hiding and higher
throughput.

Our evaluation across five datasets shows that \sysname achieves up to
\timesFasterThanCagra$\times$ higher query throughput than \cagra, the current
state-of-the-art GPU index.
% , and achieves up to 80\% peak utilization as
% measured by the roofline model. 
\sysname's construction scales efficiently to
large datasets and constructs indices an average of \avgConstruct faster than
\cagra while providing updatability that \cagra lacks. Compared to \bang, the
previous fastest GPU Vamana implementation, \sysname delivers
\lowerBangSpeedup–\higherBangSpeedup$\times$ faster queries. 
%\sysname's incremental construction scales efficiently, a 20$\times$ increase
%in index size reduces insertion throughput by only 50\%, making it well-suited
%for production workloads where data arrives continuously.

\end{abstract}
\fi


==> vldb26-revision/algorithms/beamSearch.tex <==
\begin{algorithm}
\DontPrintSemicolon
\caption{BeamSearch (DiskANN)}
\label{alg:beamsearch}
\KwIn{Graph $G$, query vector $q$, beam width $K$, start vertex $m$ (medoid)}
\KwOut{Frontier $F$ of $K$ nearest neighbors, visited set (hash table) $V$}
$F \gets \{m\}$ (priority queue by distance) \;
$V \gets \emptyset$ \;
\While{there exists an unvisited vertex $u \in F$}{
    Mark $u$ visited: $V \gets V \cup \{u\}$ \;
    \For{each neighbor $v$ of $u$}{
        \If{$v \notin V$}{
            Compute distance $d(q,v)$ \;
            Insert $v$ into $F$ with priority $d(q,v)$ \;
        }
    }
    \If{$|F| > K$}{
        Remove furthest elements from $F$ until $|F|=K$ \;
    }
}
\Return $(F, V)$
\end{algorithm}


==> vldb26-revision/algorithms/jasperDiff.tex <==
\begin{algorithm}
\DontPrintSemicolon
\caption{\sysname BeamSearch \hspace{0.4em}\textnormal{\small (refer to \Cref{alg:beamsearch})}}
\label{alg:jasperbeam}
\KwIn{Graph $G$, query $q$, beam width $K$, start vertex $m$}
\KwOut{Frontier $F$ of $K$ nearest neighbors (each entry carries a visited flag)}

% \color{forestGreen}% R2-W1: revision-added algorithm.
$F \gets \{m\}$ \tcp*{priority queue by $d(q,\cdot)$; visited flag per entry}
\While{some entry in $F$ is unvisited}{
    $u \gets$ closest unvisited entry in $F$; mark $u$ visited\;
    \tcp{Gather: all neighbors of $u$ (no visited filter --- duplicates allowed)}
    $C \gets N(u)$\;
    \tcp{Distance: parallel tile-based chunked loads compute $d(q,v)$}
    \ForEach{$v \in C$ \textnormal{in parallel across the block's tiles}}{
        compute $d(q, v)$\;
    }
    \tcp{Sort + merge: full sort over the union}
    $F \gets \textsc{Sort}(F \cup C)$ by $d(q, \cdot)$\;
    \tcp{Prune: clip to top-$K$ (visited flags carry over)}
    truncate $F$ to $K$\;
}
\Return $F$
\end{algorithm}


==> vldb26-revision/algorithms/parlayBuild.tex <==
\begin{algorithm}
\DontPrintSemicolon
\caption{Batch Insertion (ParlayANN)}
\label{alg:parlayann}
\KwIn{Batch of new points $B$, current graph $G$, beam width $K$, degree cap $R$}
\KwOut{Graph $G$ updated with $B$}

% \BlankLine
\textbf{Step 1: Local candidate generation}\;
\ForPar{each $x \in B$}{
    $(F, V) \gets \text{BeamSearch}(G, x, K, G.medoid)$\;
    $E_x \gets \{(x, v): v \in V\}$ \tcp*{add edges for new nodes}
}

% \BlankLine
\textbf{Step 2: Global edge collection}\;
$E \gets \bigcup_{x \in B} E_x$ \tcp*{concatenate edges}

% \BlankLine
\textbf{Step 3: Semisort and parallel pruning}\;
Group $E$ by endpoint using \textbf{Semisort}\;
\ForPar{each vertex $u$ touched by $E$}{
    $N'(u) \gets \text{RobustPrune}(u, N(u) \cup E[u], R)$\;
    Update adjacency list of $u$ with $N'(u)$\;
}

\Return $G$
\end{algorithm}


==> vldb26-revision/algorithms/robustPrune.tex <==
\begin{algorithm}
\DontPrintSemicolon
\caption{RobustPrune (DiskANN)}
\label{alg:robustprune}
\KwIn{Node $p$, candidate neighbors $N(p)$, degree cap $R$, pruning factor $\alpha$, distance $d$}
\KwOut{Pruned neighbor set $N'(p)$}
Sort $N(p)$ by $d(p, \cdot)$ (closest first)\;
$N'(p) \gets \emptyset$\ (initialize as empty);

\While{$|N'(p)| < R$ and $N(p)$ not empty}{
    $p^* \gets$ extract closest from $N(p)$\;
    Add $p^*$ to $N'(p)$\;
    \For{each $p' \in N(p)$}{
        \If{$\alpha \cdot d(p^*, p') \leq  d(p, p')$}{
            Discard $p'$ from $N(p)$\;
        }
        \Else{
            Keep $p'$ in $N(p)$\;
        }
    }
}
\Return $N'(p)$
\end{algorithm}


==> vldb26-revision/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


We showed that GPU-native approximate nearest neighbor search (ANNS) can
substantially outperform CPU-based approaches while enabling high-throughput
retrieval and efficient co-location with downstream machine learning workloads.
Our study further reveals that modern GPUs expose new bottlenecks: existing GPU
ANNS systems often underutilize hardware due to synchronization overheads and
excessive shared memory usage. By simplifying search kernels and optimizing
memory access, \sysname achieves up to \timesFasterThanCagra$\times$ higher
query throughput than CAGRA while supporting streaming updates, delivers
\lowerBangSpeedup--\higherBangSpeedup$\times$ higher throughput than BANG, and
constructs indexes \avgConstruct faster than CAGRA on average. Our optimized
search kernel sustains 70--80\% of peak theoretical throughput.

Roofline analysis shows that state-of-the-art GPU ANNS kernels are already
close to the memory-bandwidth limit, suggesting that future gains will
primarily come from reducing data movement, for example through
quantization-aware designs such as RaBitQ. Scaling beyond GPU memory remains an
open challenge: even the largest GPUs can store graphs for only about 200
million vectors, requiring multi-GPU sharding or host-pinned memory for larger
datasets. Developing efficient architectures for this setting is an important
direction for future work.


% In this work, we demonstrate that GPU-native approximate nearest neighbor
% search (ANNS) can achieve substantial acceleration over CPU variants, enabling
% high-throughput queries and effective data co-location with downstream machine
% learning workloads. We show that the extreme degree of parallelism exposed by
% modern GPUs introduces new challenges: prior GPU ANNS systems often leave
% performance on the table due to synchronization overheads and limited shared
% memory. Our results show that carefully simplifying ANNS kernels to reduce
% shared memory usage and optimizing data load can significantly increase
% throughput and achieve higher parallelism.
%
% We demonstrate that \sysname achieves up to \timesFasterThanCagra$\times$ higher
% query throughput than CAGRA while providing streaming update capabilities that
% CAGRA lacks, and delivers \lowerBangSpeedup--\higherBangSpeedup$\times$ higher throughput than BANG. Our
% batch-parallel construction algorithm achieves \avgConstruct faster index
% construction than CAGRA on average. Our optimized search kernel achieves
% 70--80\% of peak theoretical throughput.
%
% Our roofline analysis reveals that state-of-the-art GPU ANNS kernels operate
% close to the memory bandwidth ceiling. Future performance gains must come
% primarily from reducing data movement, and quantization-aware designs like
% RaBitQ demonstrate a promising path forward by pushing systems closer to the
% compute roof where substantial headroom remains.
%
% While GPU-native kernels achieve close to the roofline performance, the
% problem of scaling out to full CPU DRAM with a single CPU is still unsolved.
% The largest GPUs can at most hold a graph of ~200 million vectors, to
% construct larger would require either a sharding in a multi-GPU setup
% approach  or host-pinned storage, each of which come with significant design
% constraints. We leave these approaches as future work for achieving higher
% scalability.


% \RTwoInline{W2}{Add a short "future work / scaling beyond device
% memory" paragraph here. Two angles: (1) multi-GPU sharding of the graph, and
% (2) host-pinned vector storage with on-device graph (we already prototype the
% latter under \texttt{data/a100/jasper\_host}). Keep brief — reviewer asked
% how the constraint could be relaxed in the future, not for a full design.}

% \RFourInline{W3}{}
% \RTwoInline{W2}{
% }

% \begin{itemize}
%     \item Porting ANNS to GPUS can provide massive performance benefits and allow for colocation
%     \item the extreme parallelism of GPUs can make achieving performance difficult 
%     \item Simplifying ANNS kernels can actually increase throughput by reducing shared memory kernels, increasing potential occupancy and parallelism.
%     \item Modern ANNS kernels run at close to the roofline of the processors - to further improve performance we must reduce memory transfer.
%     \item Directly comparable quantization techniques like RaBitQ are necessary to gain performance when reducing memory traffic. RaBitQ preserves accuracy while reducing memory transfer by up to 8x. This gives higher performance for larger vector datasets and increases the arithmetic intensity, suggesting that there are large potential performance gains still on the table for quantized techniques.
% \end{itemize}
%

% In this work, we demonstrate that porting approximate nearest neighbor search
% (ANNS) to GPUs can yield substantial performance improvements, enabling
% high-throughput query processing and effective co-location with downstream
% machine learning workloads. However, the extreme degree of parallelism exposed
% by modern GPUs introduces new challenges: GPU ANNS algorithms often fail to
% achieve maximum performance due to synchronization overheads and limited shared
% memory. Our results show that carefully simplifying ANNS kernels to reduce
% shared memory usage can significantly increase throughput and achieve higher
% parallelism.
%
% We further observe that the state-of-the-art GPU ANNS kernels such as \cagra
% already operate close to the architectural roofline, indicating that raw
% compute optimizations offer diminishing returns. At beam width=256, \sysname
% achieves 50\% higher FLOP/S than \cagra, but this value is 69\% of the peak
% possible throughput throughput for this arithmetic intensity - suggesting only
% a further 1.44$\times$ speedup is possible in this kernel.
%
% Consequently, future performance gains must come primarily from reducing memory
% traffic. Quantization techniques that are directly comparable to full-precision
% baselines, such as RaBitQ, provide a promising path forward by preserving
% accuracy while reducing memory transfer by up to 8$\times$. This reduction not
% only improves performance on large-scale vector datasets but also increases
% arithmetic intensity, suggesting that substantial headroom remains for further
% gains through quantization-aware ANNS designs.


==> vldb26-revision/data/a40/bang/bigann-k1.tex <==
throughput,recall
662505.972,0.3064
301715.684,0.8729
210495.11000000002,0.9455
146002.116,0.9711
120126.34199999999,0.9817
98422.982,0.9882
95113.38,0.9911
79329.774,0.9934000000000001
68686.50200000001,0.9954999999999999
54474.60399999999,0.9973000000000001
56702.316000000006,0.9978
44856.876000000004,0.998
44763.7,0.998
47632.119999999995,0.9983
42303.406,0.9984000000000001
33222.770000000004,0.9990000000000001
11592.99,1.0


==> vldb26-revision/data/a40/bang/bigann-k10.tex <==
throughput,recall
286210.916,0.679
189846.152,0.8618000000000001
147620.352,0.9242
113698.648,0.9521999999999999
113586.72,0.9669
94261.29000000001,0.9756
78568.72400000002,0.9812000000000001
76352.602,0.9853000000000001
71334.52600000001,0.9882
59085.09199999999,0.9902
58457.454000000005,0.9918
54786.6,0.993
48658.13,0.9940000000000001
44871.456,0.9948
43624.214,0.9954999999999999
41807.908,0.9961
39907.394,0.9965
36957.432,0.9969
35387.914,0.9972
33761.8,0.9975
21648.536,0.9990000000000001
14699.12,0.9994
11726.088,0.9997


==> vldb26-revision/data/a40/bang/bigann-k50.tex <==
throughput,recall
81909.94600000001,0.7567
86671.13600000001,0.8210999999999999
78961.988,0.8665
64585.224,0.8987999999999999
67521.89000000001,0.9218999999999999
59262.512,0.9390999999999999
55248.478,0.9512999999999999
53847.578,0.9608
50884.04,0.9679000000000001
44992.036,0.9732999999999999
40297.072,0.9777
40428.426,0.981
39469.96000000001,0.9836
35484.172,0.9858
30593.958000000002,0.9876
32313.528000000002,0.9891
26854.958000000002,0.9937
22182.934,0.9958
18549.238,0.9971
14912.025999999998,0.9978
11728.84,0.9986


==> vldb26-revision/defines.tex <==
\newcommand{\nearest}{$\mathcal{L}$}

% Set to true to show comments, false to hide them for submission
\newif\ifshowcomments
% \showcommentstrue  % Show comments (use \showcommentsfalse to hide)
\showcommentsfalse  % Show comments (use \showcommentsfalse to hide)


% In your preamble
\newif\iftruncate

% Toggle this line to show/hide:
\truncatetrue   % uncomment to SHOW the block
% \truncatefalse  % uncomment to HIDE the block

% Appendix toggle (revision-only material).
\newif\ifappendix
\appendixtrue   % uncomment to INCLUDE the appendix
% \appendixfalse

% Cross-reference to appendix material. When the appendix is compiled into
% this build, link to it directly with \Cref. Otherwise (e.g. the VLDB
% camera-ready, which omits the appendix) emit a compact citation to the arXiv
% extended version~\cite{McCoy2026} carrying the appendix location as the note,
% e.g. \apxref{app:memory}{Appendix~D} renders as "[N, Appendix D]".
% #1 = label to \Cref; #2 = appendix location note for the arXiv build.
\newcommand{\apxref}[2]{\ifappendix\Cref{#1}\else\cite[#2]{McCoy2026}\fi}

% \newif\ifshowtruncated
% \showtruncatedtrue  % Show truncated text (use \showcommentsfalse to hide)
% %\showtruncatedfalse  % hide truncatedtext (use \showcommentsfalse to hide)
%
\ifshowcomments
    \newcommand{\prashant}[1]{{\scriptsize \textcolor{red}{Prashant: {#1}}}}
    \newcommand{\hunter}[1]{{\scriptsize \textcolor{blue}{Hunter: {#1}}}}
    \newcommand{\zikun}[1]{{\scriptsize \textcolor{purple}{Zikun: {#1}}}}
\else
    \newcommand{\prashant}[1]{}
    \newcommand{\hunter}[1]{}
    \newcommand{\zikun}[1]{}
\fi

% \ifshowtruncated
%     \newcommand{\truncate}[1]{\textcolor{red}{\sout{#1}}}
% \else
%     \newcommand{\truncate}[1]{}
% \fi

\newcommand{\hunterinline}[1]{\hunter{#1}}
\newcommand{\prashantinline}[1]{\prashant{#1}}
\newcommand{\zikuninline}[1]{\zikun{#1}}



\newcommand{\hunterReplace}[1]{{\textcolor{blue}{Hunter - Replacement text: {#1}}}}




% \newcommand{\prashant}[1]{{\scriptsize \textcolor{red}{Prashant: {#1}}}}
% \newcommand{\hunter}[1]{{\scriptsize \textcolor{blue}{Hunter: {#1}}}}
% \newcommand{\hunterinline}[1]{\hunter{#1}}
% \newcommand{\prashantinline}[1]{\prashant{#1}}
% \newcommand{\zikun}[1]{{\scriptsize \textcolor{purple}{Zikun: {#1}}}}
% \newcommand{\zikuninline}[1]{\zikun{#1}}
%

\newcommand{\para}[1]{\smallskip\noindent\textbf{#1.}}

\newcommand{\defn}[1]{{\textit{\textbf{\boldmath #1}}}\xspace}

\newcommand{\sysname}{Jasper\xspace}
\newcommand{\sysnameRQ}{Jasper RaBitQ\xspace}
\newcommand{\RQ}{RaBitQ\xspace}
\newcommand{\cagra}{CAGRA\xspace}
\newcommand{\ganns}{GANNS\xspace}
\newcommand{\parlayann}{ParlayANN\xspace}
\newcommand{\diskann}{DiskANN\xspace}
\newcommand{\bang}{BANG\xspace}

\newcommand{\bigann}{BigANN\xspace}
\newcommand{\deep}{Deep\xspace}
\newcommand{\gist}{Gist\xspace}
\newcommand{\openai}{OpenAI\xspace}
\newcommand{\textToImage}{Text2Image\xspace}


%Size command
\newcommand{\figsize}{.24}


%Special results
\newcommand{\fastestBuild}{1,179K\xspace}
\newcommand{\timesFasterThanCagra}{1.84\xspace}
\newcommand{\lowerBangSpeedup}{10\xspace}
\newcommand{\higherBangSpeedup}{74\xspace}
\newcommand{\fastestQuery}{12.5 million\xspace}
\newcommand{\fastestOpenAIQuery}{3.2 million\xspace}
\newcommand{\latencyReduction}{14\%\xspace}

\newcommand{\avgConstruct}{7.0$\times$\xspace}
\newcommand{\maxConstruct}{25.5$\times$\xspace}


%robustPrune and beamSearch

\newcommand{\prune}{\textsc{robustPrune}\xspace}
\newcommand{\search}{\textsc{beamSearch}\xspace}

%Margin Comment
\ifshowcomments
    \newcommand{\marginComment}[1]{\marginpar{\sf \scriptsize \textcolor{red}{#1} }}
    % Reviewer-tagged inline markers used throughout the revision.
    %\newcommand{\R1Inline}[1]{{\textcolor{red}{R1: {#1}}}}
    \newcommand{\RTwoInline}[2]{{\textcolor{forestGreen}{\marginComment{R2: #1}{#2}}}}
    \newcommand{\RThreeInline}[2]{{\textcolor{blue}{\marginComment{R3: #1}{#2}}}}
    \newcommand{\RFourInline}[2]{{\textcolor{magenta}{\marginComment{R4: #1}{#2}}}}
\else
    \newcommand{\marginComment}[1]{}
    \newcommand{\RTwoInline}[2]{{#2}}
    \newcommand{\RThreeInline}[2]{{#2}}
    \newcommand{\RFourInline}[2]{{{#2}}}
\fi

% Alternative per-reviewer Marker variants (margin-only, no inline color) —
% kept commented for future use if we want to flag a section in the margin
% without coloring the body text.
% \newcommand{\R1Marker}[1]{\marginpar{\sf \scriptsize \color{red}{R1:#1} }}
% \newcommand{\R2Marker}[1]{\marginpar{\sf \scriptsize \color{blue}{R2:#1} }}
% \newcommand{\R3Marker}[1]{\marginpar{\sf \scriptsize \color{orange}{R3:#1} }}
% \newcommand{\R4Marker}[1]{\marginpar{\sf \scriptsize \color{green}{R4:#1} }}


==> vldb26-revision/diskann.tex <==
\section{Vamana Index}
\label{sec::diskann}

% \prashant{Always use ``Cref'' (capital C).}
% \prashant{Rewrite the preamble of this section stating why we choose Vamana
% rather than just stating it.} 

In this section, we cover the Vamana algorithm graph structure, construction
and query algorithm, and the batch-parallel construction algorithm. 

Our system
\sysname employs the Vamana graph~\cite{Subramanya2019}, a directed proximity
graph designed to support efficient greedy search with bounded out-degree, to
build the approximate nearest neighbor search (ANNS) index. We choose the
Vamana graph as it supports both a fast and accurate greedy search and an
efficient parallel construction algorithm introduced in
ParlayANN~\cite{Manohar2024}. 
We describe how we develop GPU-accelerated Vamana index along with several GPU
optimizations in the next section.

% Vamana serves as the foundation for several state-of-the-art graph-based ANNS
% systems, including ParlayANN~\cite{Manohar2024}, which introduces algorithmic
% refinements to improve construction efficiency and query recall. \sysname
% builds on the Vamana algorithm introduced in Suhas et
% al.~\cite{Subramanya2019}. This index construction algorithm was first used
% in DiskANN to construct efficient ANN search graphs.

% The Vamana algorithms constructs a navigable search graph (NSG) that can be
% traversed to find approximate nearest neighbors of a target. Vectors from a
% dataset are mapped one-to-one to vertices in the graph so that each vertex
% corresponds to a unique vector. Since each vertex corresponds to vector,
% distances between vertices can be calculated by using the dot product or L2
% distance between their corresponding vectors. A greedy traversal of the graph
% towards

\subsection{Graph definition} 
The Vamana index is a directed graph $G = (V, E)$ constructed over a set of
data vectors $V = \{x_1, \dots, x_N\}$, where $N$ is the total number of
vectors. Each node maintains an adjacency list of at most $R$ outgoing edges. A
distinguished entry point $s \in V$ is used to initialize both graph
construction and query traversal.

The edge set $E$ is selected to ensure that the graph remains sparse while
preserving navigability. For a given vertex in the graph and query vector,
there is a high probability that one of the outgoing edges of the vertex leads
to a vertex that is closer to the query. This property means that greedy search
will converge to a set of points close to a target query and is critical for
enabling low-latency approximate search.

\subsection{Vamana construction algorithm}

The original Vamana construction algorithm starts with all vertices contained
within a graph with a random set of edges with maximum outgoing degree $R$.
Vamana graph construction proceeds incrementally to refine the graph one vertex
at a time. Refinement of verticies proceeds in two phases. First, Vamana uses
\search to identify candidate neighbors in the existing graph for the new
vertex. Second, Vamana applies a pruning procedure, \prune, to reattach the
vertex to the graph while enforcing a strict bound on the out-degree.

% The Vamana search graph maps ANNS vectors one-to-one to vertices in a search
% graph so that a traversal of the graph yields a set of vectors that contain
% the nearest neighbors. This search graph is constructed starting from the
% medoid, the vertex closest to the center of the graph. The graph is directed
% and  each node in the graph having a fixed outgoing degree. The graph is
% represented as an edge list with a fixed maximum outgoing degree R that is
% specified during construction.

% The core of the Vamana algorithm is two functions: beamSearch and
% robustPrune, which query and refine the search graph respectively. At a high
% level, BeamSearch performs a greedy search across the graph, iteratively
% exploring the closest unvisited node while tracking both the nearest
% neighbors encountered and all nodes visited along the search. RobustPrune
% then uses the information from beamSearch to add new nodes to the graph while
% keeping the maximum degree bounded.

\input{algorithms/beamSearch}

\para{Beam search} Given a vector $x$ to be inserted, the construction algorithm starts with a search for the approximate nearest neighbors using \search (\Cref{alg:beamsearch}). \search starts at a designated start point, typically chosen as the medoid, and maintains two sets: (i) a \emph{frontier} which stores the $K$ closest candidate vertices discovered so far, and (ii) a \emph{visited list} which records all vertices whose outgoing edges have been explored. In each iteration, the algorithm \emph{expands} the closest frontier vertex not yet visited, loading the candidates from its outgoing edges, computing their distance to $x$, and inserting them into the frontier.

%%START - clipped for space
% \para{Beam search}
% Given a vector $x$ to be inserted, the construction algorithm performs an
% approximate nearest neighbor search in the current graph using \search. 
% The pseudocode for this procedure is shown in~\Cref{alg:beamsearch}.
% The search is
% initialized at a designated start vertex, typically chosen as the \emph{medoid}
% (the vector closest to the center) of the dataset.

% \search maintains two sets: (i) a \emph{frontier}, which stores the $K$
% closest candidate vertices discovered so far, ordered by increasing distance to
% the query vector $x$, and (ii) a \emph{visited list}, which records all
% vertices whose outgoing edges have been explored. At each iteration, the
% algorithm selects the closest vertex in the frontier that has not yet been
% visited, loads its outgoing edges, computes the distance between $x$ and each
% neighbor, and inserts newly encountered vertices into the frontier.
%%END - clipped for space

If the size of the frontier exceeds the beam width $K$, the furthest candidates
are discarded. This expansion process continues until all vertices in the
frontier have been visited. 
The procedure returns both the final frontier and the full list of visited vertices.

%%START - clipped for space
% The procedure returns both the final frontier,
% representing approximate nearest neighbors of $x$, and the full visited list,
% which captures the local search region explored during insertion.
%%END - clipped for space

\para{Edge attachment}
Once \search completes, the new vertex $x$ is attached to the graph using the visited list. Bidirectional edges are added
between $x$ and each vertex in the visited list, temporarily allowing the
out-degree of affected vertices to exceed the maximum degree bound $R$.

\para{Robust prune}
To restore the degree bound, Vamana applies the \prune procedure to any vertex
whose outgoing edge list exceeds $R$ (maximum out degree). 
Given a vertex $p$, \prune sorts the outgoing neighbors by increasing
distance from $p$.
The algorithm iteratively selects the closest remaining neighbor $p^*$ and
adds it to the pruned adjacency list. For each remaining candidate neighbor
$p'$, \prune compares the distance $d(p^*, p')$ to the distance
$d(p, p')$. If
\[
\alpha \cdot d(p^*, p') \le d(p, p'),
\]
then $p'$ is removed from consideration. This process repeats until either the
pruned adjacency list reaches size $R$ or no candidates remain.

%%START - clipped for space
% Intuitively, \prune removes edges that are redundant due to the existence
% of a strong two-hop path: a direct edge from $p$ to $p'$ is discarded if $p'$
% can be reached via a significantly closer neighbor $p^*$. The parameter
% $\alpha > 1$ controls the aggressiveness of pruning and trades off graph
% sparsity for navigability.

% Together, \search and \prune allow Vamana to incrementally construct
% a bounded-degree proximity graph that preserves long-range connectivity while
% supporting efficient greedy traversal during query time.
%%END - clipped for space

% The insertion of an item into the Vamana index occurs in two phases: first, beam search is used to locate the neighbors of the new vertex, and then robustPrune is used to efficiently attach it to the search graph. The pseudocode for beamSearch can be seen in \cref{alg:beamsearch}. The algorithm starts at the medoid of the graph and maintains two lists: a list of the $K$ closest vertices called the \textbf{frontier}, and a list of the vertices visited called the \textbf{visited list}. At every iteration, the beamSearch expands the closest unvisited vector by loading it's outgoing edges from memory, calculating their distance to the query vector, and adding them to the $K$ nearest seen. If the size of the frontier exceeds the limit K, the furthest vectors are clipped. This process of expansion continues until all vectors in the frontier have been visited, and returns both the frontier and the visited list.



% \prashant{Alg 2 seems a bit off. Need to recheck.}
% Once a vertex has been searched, it must be added to the graph. The challenge is adding new vertices without allowing the degree of the graph to blow up. To solve this problem, Vamana index uses a pruning algorithm called robustPrune. RobustPrune allows the index to add new edges and vertices to the graph while keeping the maximum outgoing degree bounded. Once a vector has been queried with beamSearch, the visited list is used to attach the vector to the graph. This is done by adding bidirectional edges between the new vertex and the vectors in the visited list. If the degree of any vertex exceeds a set cap R, robustPrune is run on that vertex to reduce the size of the edge list. The pseudocode for robustPrune can be seen in \cref{alg:robustprune}. robustPrune takes the outgoing edges of a node and sorts them by their length from closest to furthest. The algorithm then loops until either degree is equal to R or no more edges remain. In each iteration, the vertex \textbf{p*} with the closest outgoing edge is added back to the outgoing edges. All remaining vertices (denoted as p') that have not yet be re-added are then checked against p*. The check compares the distance between p* and p` and the original distance between p and p`. If the weighted distance to the newly added node p* is less than the distance from p` to the vertex p, p` is discarded from the neighbor list. Intuitively, this removes direct edges between nodes that have a good two-hop connection: your edge removed IFF you are much closer (by a factor of alpha) to an already-attached vertex than you are to the target vertex.


\subsection{ParlayANN}
\label{sec::parlay}

\parlayann~\cite{Manohar2024} is an extension of the Vamana construction
algorithm that addresses a fundamental scalability bottleneck in graph construction. The original \diskann~\cite{Subramanya2019} inserts vertices in parallel using fine-grained locks, leading to significant contention on high-centrality vertices such as the
\emph{medoid}.
%%START - clipped for space
% \parlayann~\cite{Manohar2024} is an extension of the Vamana construction
% algorithm that addresses a fundamental scalability bottleneck in parallel graph
% construction by adopting a batch-parallel insertion scheme. While the original
% \diskann~\cite{Subramanya2019} algorithm supports inserting points in parallel,
% it relies on fine-grained locks to update adjacency lists. In practice, this
% design leads to significant contention on high-centrality vertices, such as the
% \emph{medoid}. During the greedy search, high-centrality vertices are
% frequently traversed, and concurrent insertions attempt to add edges to these
% vertices simultaneously, resulting in serialization that limits parallel
% scalability.
%%END - clipped for space
\parlayann eliminates this bottleneck by replacing lock-based updates with a
lock-free, batch-parallel construction strategy. The core idea is to decouple
graph traversal from graph mutation, allowing expensive updates to be applied
in parallel without contention.

% ParlayANN~\cite{Manohar2024} eliminates this bottleneck by replacing
% lock-based updates with a lock-free, batch-parallel construction strategy.
% The core idea is to decouple graph traversal from graph mutation, allowing
% expensive updates to be applied in parallel without contention.

% ParlayANN is an expansion of the Vamana algorithm that fixes a
% parallelization bottleneck by using a batched insertion scheme. The original
% DiskANN~\cite{Subramanya2019} algorithm uses locks to add individual points
% to the graph in parallel: \parlayann~\cite{Manohar2024} optimizes insertions
% using a lock-free batch-parallel insertion algorithm. The motivation for this
% redesign comes from the contention of acquiring locks on centrally located
% nodes such as the medoid. During a greedy search, the nodes near the medoid
% will be traversed and all inserts will attempt to add themselves as a new
% edge to these nodes. This leads to a serialization bottleneck that restricts
% scalability.


\parlayann restructures graph construction into two
distinct, parallelizable phases. In the first phase, \search
(\Cref{alg:beamsearch}) is executed independently in parallel for each new vertex.

Each search operates on a read-only snapshot of the current graph and adjacency lists are
not modified during this phase.
%%START - clipped for space
%  Each search operates on a read-only snapshot of the
% current graph and produces a set of candidate edges corresponding to the
% vertices encountered during traversal. Importantly, no adjacency lists are
% modified during this phase.
%%END - clipped for space
Instead of applying updates immediately, all candidate edges produced by the
batch are written to a temporary edge collection. This collection is then
\emph{semisorted}, grouping edges by their target vertex. Semisort guarantees that all candidate edges incident to
a given vertex are co-located, enabling subsequent processing to be performed
independently per vertex.

In the second phase, \prune  (\apxref{alg:robustprune}{Appendix~A}) is applied in
a batch-parallel design. Each vertex that has received new candidate edges is
assigned a unique thread, which merges the proposed edges with the existing
adjacency list and applies \prune. Because all edges incident to a vertex are processed by a
single thread, this phase requires no locks or cross-thread synchronization.

This lock-free design removes contention around centrally located vertices and
allows \parlayann to efficiently exploit multicore parallelism.

%%START - clipped for space
% The key insight
% is that the pruning step, which determines the final neighborhood structure and
% dominates construction cost, can be fully decoupled from concurrent graph
% traversals by deferring updates and processing them in parallel batches. As a
% result, \parlayann achieves significantly faster index construction while
% preserving the structural guarantees of the Vamana graph and maintaining
% comparable query performance and accuracy.
%%END - clipped for space

\input{algorithms/jasperDiff}

 % \parlayann restructures the construction phase into two distinct parallelizable steps, as shown in \cref{alg:parlayann}. First, beamSearch is run independently for each vertex in parallel, producing a set of candidate edges for insertion. Rather than directly modifying the graph with locks, these edge updates are written into a temporary collection and \textbf{semisorted}. Semisort groups the edges by keys with a much lower overhead that a full sort - this is used to group all candidate edges by their target vertex. This organization step ensures that each vertex’s set of candidate edges can be processed independently.

% Once grouped, robustPrune(\cref{alg:robustprune}) is applied in a batch parallel fashion to add new edges while maintaining a constant max degree. Each vertex with updates is assigned a unique thread, ensuring pruning can be applied without requiring any cross-thread synchronization, since all edges incident to a vertex are already localized. This lock-free design removes contention around central nodes and allows for efficient utilization of multicore parallelism. The key insight is that the expensive pruning stage, which determines the final neighborhood structure, can be completely decoupled from the concurrent beamSearch traversals by deferring updates and then processing them in parallel batches. This results in significantly faster index construction while preserving the structural guarantees of the Vamana graph and maintaining comparable query performance and accuracy.

\subsection{Why is the Vamana appropriate for GPUs?} \label{sec::why-vamana}

% \prashant{I think we need this subsection. Here we need to briefly explain why
% Vamana is better suited compared to other choices such as IVF, k-NN, or HNSW.
% This is critical for the story. This should not be the repeat of text above.}

Compared to many alternative ANN indices, the Vamana graph offers a high degree
of parallelism across both index construction and query execution, enabling
efficient use of modern GPUs. Its construction is inherently parallel: vertices
are processed independently, each following a predictable sequence of steps
that minimizes thread divergence. Distance computations and graph traversal
both expose fine-grained parallelism. Vamana also supports efficient
incremental updates. Each insertion performs a bounded beam search over a small
subset of vertices and adds at most 2R edges, keeping overhead and space usage predictable. By
comparison, update procedures for methods such as NN-Descent can be
substantially more expensive, as multiple refinement rounds are required and
any visited node may become a neighbor. Prior work shows that Vamana matches or
exceeds alternative graph indices in search quality across diverse datasets,
making it a strong foundation for high-performance, updatable
ANNS~\cite{Subramanya2019}.

% Compared to many alternative ANN indices, the Vamana graph fully utilizes modern GPUs' parallelism. During construction, each vertex is independently updated and added to the graph in batches, avoids any complex synchronization. During beam search queries, distance computations admit fine-grained parallelism within a query, and graph traversal can be easily parallelized across queries. These multiple levels of parallelism allow for finer control over performance tuning on GPUs.
%
% Furthermore, Vamana construction is low-cost and predictable. The Vamana batched updates bounds the number of insertion to at most $2R$ new edges per node, keeping the memory cost predictable. In contrast, NN-Descent graph construction can be substantially more expensive, as multiple refinement rounds are required and any visited node may become a neighbor. 
%
% Performance wise, prior empirical evaluations show that Vamana consistently matches or outperforms alternative vector graph indices in search quality across a range of datasets, making it a strong choice when both performance and accuracy are primary concerns~\cite{Subramanya2019}.



==> vldb26-revision/eval.tex <==

\section{Evaluation} 

%\R2Inline{C1}{New text that should be red.}
% \RFourInline{C1}{Test Comment}


% \hunter{TODO: How to massage writing for FP16 for RaBitQ?}
In this section, we evaluate the performance of \sysname
against four state-of-the-art ANNS indices: three GPU-based and one
CPU-based index. We evaluate the construction, query, and update performance
across five real-world datasets varying in size and number of dimensions. Wex
further evaluate the effectiveness of \sysname in saturating GPU resources using
the roofline model~\cite{Williams2009}. Finally, we perform a series of
micro-benchmarks to evaluate the impact of various GPU-specific optimizations
introduced in \sysname and discuss how these are broadly applicable for
optimizing other GPU-accelerated systems.

\subsection{Experimental setup}

We evaluate all systems on along three dimensions:
\begin{itemize}
    \item \textbf{Construction throughput:} measured as the total time required
      to build the index used in subsequent experiments.
    \item \textbf{Query throughput:} reported as the number of ANN queries
      completed per second.
    \item \textbf{Recall:} which measures the accuracy of the Top-\textit{K}
      results and is defined as $\texttt{Recall@}K = \frac{\texttt{\# of exact
      Top-\textit{K} results returned}}{K}$. We report recall at 1@1, 10@10,
      50@50, and 100@100.
\end{itemize}

% \marginComment{Test Comment}
\para{Hardware} All CPU experiments are conducted on an Intel(R) Xeon(R) Gold 5218 CPU with 32 physical cores (64 hardware threads) at 2.30 GHz. GPU
experiments are run on an NVIDIA A100 (SM80) with 80 GB of HBM memory using
CUDA 12.9.

\input{figures/datasets}

\para{Datasets} For evaluation, we select the following datasets taken from the
Big\_ANN\_Benchmarks~\cite{Simhadri2022} repository, summarized
in~\Cref{fig::datasets}.
\begin{itemize}
  \item \bigann: 100 million 128-dimensional \texttt{uint8} vectors with Euclidean
      distance from the SIFT collection. There are 10K vectors in the
      test set.
    \item \deep/Yandex: 100 million PCA-reduced, normalized GoogLeNet
      embeddings (96-dimensional  \texttt{float32}). Euclidean distance and 10K
      queries.
    \item \gist: 1 million 960-dimensional \texttt{float32} vectors with euclidean
      distance and 1K query vectors in the test set.
    \item OpenAI-Arxiv: 2.3 million 1536-dimensional \texttt{float32} embeddings of
      Arxiv papers. Query set is 10K vectors.
    \item \textToImage: 10 million 200-dimensional \texttt{float32} image embeddings
      from the Se-ResNext-101 model. Distance is maximum inner product search
      (MIPS) and there are 10K queries in the test set.
\end{itemize}

\para{ANNS indices} We compare Jasper to the following ANNS indices:
\begin{itemize}

    \item \textbf{\cagra}~\cite{ootomo2024}: The state-of-the-art in GPU index
      construction. \cagra constructs a graph index using
      NN-Descent~\cite{Wang2021}.
      \iftruncate
      NN-Descent iteratively improves graph
      connectivity by expanding each node's neighborhood through 2-hop
      neighbors. The resulting graph is well-connected but too dense for GPU
      memory. \cagra addresses this with a three-phase pruning algorithm: edges
      are sorted by length, redundant edges with good 2-hop alternatives are
      removed, and finally the graph is merged with its reverse and pruned
      again to produce the final index.
      \fi
    
    \item \textbf{\bang}~\cite{Venkatasubba2025}: \bang extends the query
      execution of DiskANN~\cite{Subramanya2019} to GPUs. \bang does not
      perform construction and requires a preconstructed Vamama graph from
      DiskANN.  
      \iftruncate
      It uses product quantization to reduce the size of the
      vectors. The quantized vectors are stored in the GPU memory while the
      graph and full vector data are stored in DRAM.
      The entirety of a
      streaming multiprocessor (SM) is used for each query. One thread is used
      for each distance calculation, as distances can be calculated using only
      PQ table lookups. To process queries more efficiently, Bloom filters are
      used to represent the visited list, lowering the memory requirements for
      searching.
      \fi
    
    \item \textbf{\ganns}: \ganns~\cite{Yu2022} is an implementation of the
      HNSW graph algorithm optimized for GPUs. 
      \iftruncate
      To optimize for GPU execution,
      \ganns uses lazy data structures - rather than maintain a priority queue,
      \ganns maintains two lists (frontier and visited) and only occasionally
      updates the lists to mark vertices as visited. They avoid the use of a
      hash table for marking visited vertices during queries, and use multiple
      thread blocks per query. 
      \fi
      The construction algorithm for HNSW graphs is
      difficult to parallelize, so \ganns constructs many small graphs in
      parallel and then sequentially merges them. \ganns does not support
      dataset with 100 million vectors.
    
    \item \textbf{\parlayann}: \parlayann is the state of the art CPU ANNS system.
      \iftruncate
      It implements Vamana for 
      construction and implements the batch-parallel construction algorithm.
      This algorithm is discussed in more detail in \Cref{sec::parlay}.
      \parlayann has the ability to perform \textit{scalar} quantization in
      which floats are translated directly into smaller integer types by evenly
      bucketing the real number line into buckets of a size $\Delta$ based on
      the integer size.
      \fi
\end{itemize}

For all indices the graph size is held constant at R=64, so each vertex has at
most 64 outgoing edges.

\input{figures/tables/construction}
\input{figures/construction/incremental_build}
\input{figures/construction/incremental_comparison}

\subsection{Index construction}
Here we evaluate the index construction performance of \sysname against other
ANNS indexes. 

\para{Bulk construction} In this benchmark, datasets are constructed in one
shot. Results are shown in~\Cref{tab::construction}. We measure the overall
construction throughput as the ratio of the number of vectors indexed and total
construction time. \sysname achieves the highest construction throughput on all
datasets with peak throughput of \fastestBuild inserts/secs on
\bigann. \parlayann while running on CPU (64 threads) is between $4.3-17.3\times$ slower than \sysname. \ganns is another GPU-based ANNS index but is between $10.1-41.8\times$ slower than \sysname. Additionally, \ganns does not support construction on 100M datasets as it is constrained due to \texttt{int32} datatype being employed to index into the vector array. 100M vectors with 128/96 dimensions require 64-bit datatype for indexing.

\input{figures/a100-query}

% \hunter{Make this a table to save space / present cleaner?}
% \RTwoInline{W2}{}
% \RThreeInline{D1}{We sweep the insertion batch size from 0.5\% to 32\% of the
% dataset on \bigann 10M, \gist 1M, and \bigann 100M. Insertion throughput
% rises monotonically with batch size and then saturates as the GPU is fully
% utilized: on \bigann 10M, throughput grows from $\sim$203K inserts/sec at
% 0.5\% to $\sim$753K at 8\%, after which 16\% gives no further gain; on \gist
% 1M it scales smoothly from 74K to 176K going from 0.5--32\%. On
% the 100M-scale \bigann index batches above 4\% exceed available device memory
% and the build fails, which is consistent with the workspace bound described
% in~\Cref{subsec:gpu-optimizations}. Recall is essentially unaffected: across
% all beam widths the per-row variation in recall as batch size grows is below
% two percentage points (e.g.\ beam-128 recall on \gist drops from 0.854 at
% 0.5\% to 0.820 at 32\%), confirming that batch size is a throughput knob rather
% than a quality knob.}
We sweep the insertion batch size from 0.5\% to 32\% of the
dataset on \bigann 10M and \gist 1M. Insertion throughput
rises monotonically with batch size and then saturates as the GPU is fully
utilized: on \bigann 10M, throughput grows from $\sim$233K inserts/sec at
0.5\% to $\sim$753K at 16\%, after which 32\% gives no further gain; on \gist
1M it scales smoothly from 52K to 198K going from 0.5--32\%.
Recall is essentially unaffected: across
all beam widths the per-row variation in recall as batch size grows is below
two percentage points (e.g.\ beam-128 recall on \gist drops from 0.854 at
0.5\% to 0.820 at 32\%), confirming that batch size is a throughput knob rather
than a quality knob.

\para{Incremental construction}
\Cref{fig:incremental_jasper} shows how \sysname's construction throughput
changes as the index grows. We build the index incrementally, inserting vectors
in batches of 2\% of the total dataset. Across all datasets, throughput
decreases as the index grows, but the slowdown is sub-linear in index
size. For example, on \deep, \sysname inserts 814K vectors/secs when the index
is at 5\% capacity (5M vectors). When the index reaches 99\% capacity (99
million vectors), throughput drops to 247K vectors/secs. This is roughly a
3.2$\times$ slowdown despite a 20$\times$ increase in index size, demonstrating
that \sysname maintains efficient insertion performance even as the index grows
large.

\Cref{fig:incremental_comparison} illustrates why incremental construction
matters. We measure the time required to add a 10\% slice of new vectors to an
already-constructed index, simulating a common production scenario where new
data arrives after the initial index is built. \sysname and \parlayann, which
support incremental updates, complete this operation an order of magnitude
faster than \cagra and \ganns. The difference arises because \cagra and \ganns
lack incremental update support: each batch of new vectors requires rebuilding
the entire index from scratch.


% Incremental construction for \sysname is presented
% in~\Cref{fig:incremental_jasper}. Results are presented as a fraction of the
% total index size, and the index is constructed in batches of 2\% of the total
% dataset size. All five datasets show a consistent trend where performance drops
% slightly as the as the index grows. However, this drop is not linear with the
% size of the dataset. For example, at 5\% load (500,000 vectors inserted) on
% \deep, \sysname inserts 251,601 vectors per second. At 99\% load factor (9.9
% million vectors inserted) \sysname inserts 116,217 vectors per second. As the
% construction algorithm cost does not grow linearly with the size of the
% dataset, \sysname remains efficient for updates even for large datasets. 
%
% We show the benefit of incremental construction in
% \Cref{fig:incremental_comparison}. In this benchmark, we compare the time taken
% to add a 10\% slice of the dataset, simulating an incremental case where new
% vectors are added after the index is built. In this benchmark, \sysname and
% \parlayann are an order of magnitude faster for updates as the index can be
% updated incrementally. \cagra and GANNS see significant performance loss on
% later updates as they must rebuild the index every time new updates are
% processed.

%%% Commenting for space
% \para{Takeaways} 
% \textit{Batch-parallel construction offers best-in-class
% performance for construction while still allowing for incremental updates.
% Insertion performance does not decrease linearly with increasing index size,
% leading to strong scaling as the dataset size increases.}


\subsection{Queries}
Here we evaluate the approximate nearest neighbor search (ANNS) performance of
\sysname against other ANNS indexes. \Cref{fig::a100_query} shows the
recall/throughput curves for all indexes across the five datasets on the A100.

% \zikun{Maybe we should put the takeaways in the front of each section?}

\para{Low-dimensional vector datasets: \bigann and \deep} 
For the low-dimensional vector datasets, \sysname is the fastest index for all
recall values supported, with peak throughput of 12.5 million queries / sec at
.23 recall. On \bigann, it is followed by \sysnameRQ which has the second
highest throughput. \sysname is the fastest ANNS index up to .9943 recall as it
does not achieve an accuracy higher than that on \bigann.
%
For \deep, \cagra is the second fastest index for all recall values tested.
\cagra achieves a higher maximum accuracy on these datasets, with peak accuracy
of .9999 for \bigann 1@1 and .983 for \deep 1@1. 

\sysname is the fastest for the low-dimensional vector datasets due to its
optimized vector loads. For small beam sizes, latency hiding is not as
effective as there is relatively little work performed per vector. This means
that reducing latency of loads improves the performance of these kernels, as
GPU compute spends less time waiting. On these low-dimensional datasets
\sysnameRQ is slightly slower than exact distance computation due to its lossy
representation and additional arithmetic overhead, but it reduces device memory
usage, allowing more vectors to reside on the GPU in memory-constrained
settings.



%%% Commenting for space
% \para{Takeaways} \textit{By removing every shared memory component possible,
% \sysname can run more queries per SM. This, along with the optimized vector
% loads for latency reduction, allow for best-in-class query performance on
% small vector datasets for all beam widths supported.}


\para{High-dimensional vector datasets: \gist and \openai}
On the high-dimensional vector datasets \gist and \openai, distance
calculations dominate the run time. To measure the cost of operations, we add
cycle counters to every operation in the search kernel. When running \sysname
exact on both \bigann and \gist, we see a $17.8\times$ increase in the cycles
taken for distance calculations in \gist, with distance calculations becoming
the most expensive operation in the entire search.

The large vector size of these datasets benefits quantization as it can reduce
the compute and memory requirements of distance calculations. On these
datasets, \sysnameRQ is the fastest algorithm for all sizes it supports, with
peak throughput over 3.2 million queries/secs and recall up to .96 for
50@50. While \sysname's exact distance computation is slower than \cagra on
these datasets, \sysnameRQ closes this gap and surpasses \cagra at the same
recalls despite its lossy representation; on \openai at 90\% recall (10@10) it
is 1.6$\times$ faster than exact \sysname. After \sysnameRQ, \sysname has the best throughput-recall trade of curve below .95 recall, at which point \cagra takes over. These systems are followed in order of pareto-optimality by \parlayann and \bang, and finally \ganns.

% All indices suffer significant performance reductions on these datasets due to
% the high volume of data transfers and distance calculations. On these datasets,
% the use of quantization results in an $8\times$ decrease in memory transfer due
% to reduced vector size. Our quantization microbenchmark (\Cref{fig:quantization}
% in the appendix) confirms that direct vector comparison is necessary for
% efficient quantized performance on GPUs: all \cagra PQ variants we benchmark
% show no improvement in performance, while \sysnameRQ is up to 60\% faster than
% the exact implementation. 

% \RFourInline{W2}{Explicitly acknowledge the recall
% regimes where CAGRA outperforms \sysname (high recall on \deep, high $k@k$ on
% \gist). Currently scattered across paragraphs — collect into one honest
% "limitations" sentence per dataset.}
\RFourInline{W2}{For 100@100 recall on these large vector datasets, \cagra is
able to achieve higher throughput and recall than either \sysname variant: on
\gist, \sysnameRQ stays Pareto-optimal only up to $\sim$0.95 recall, above
which \cagra dominates the throughput--recall curve. Both \gist and \openai exhibit the
same crossover. This is the regime where the lossy RaBitQ representation hits
its accuracy ceiling, and workloads that require very high recall on
high-dimensional vectors are better served by \cagra's exact-distance index.}

%%% Commenting for space
% \para{Takeaways} \textit{On high-dimensional vectors, the $8\times$ memory
% reduction of quantized vector loads leads to higher arithmetic intensity and
% faster throughput. However, this speedup is only practically achievable when
% the quantized vectors are directly comparable: PQ vectors achieve the same
% memory reduction but fail to provide speedups.}

\para{\textToImage} \textToImage uses maximal inner
product (MIPS) MIPS for distance instead of Euclidean. This makes construction
and querying this dataset difficult as MIPS does not preserve the triangle
inequality. Having a triangle inequality is necessary for the space to be
metric and is crucial in constructing good search graphs using the Vamana
indexing method. Without this property, graph construction can have poor
results as there is no correlation between the neighbors of a given vector: it
is possible to be "close" to a target query vertex and "far" from all of its
neighbors, making pruning impossible. To overcome this, ANNS indices convert
MIPS into a Euclidean space by adding one extra dimension. This allows for
graph construction but comes at the cost of one extra dimension.

Both the \sysname and \sysnameRQ implementations suffer from reduced
performance on this dataset, as the conversion from MIPS to Euclidean distance
reduces the accuracy compared to systems like \cagra that can construct the
graph using the original MIPS distance calculation. \sysname has the highest
recall/throughput trade-off on this dataset until .9 recall, at which point
\cagra shows the highest recall/throughput trade-off. Due to the low dimensions
(200), \sysname exact shows higher performance than \sysnameRQ, with \sysnameRQ
showing reduced recall due to the MIPS distance calculation.

%%% Commenting for space
% \para{Takeaways} \textit{As MIPS does not form a metric space, the Vamana
% algorithm struggles to produce a good search graph due to the triangle
% inequality being necessary for RobustPrune. \sysname has the highest throughput
% for most beam widths supported, but struggles to reach high recall compared to
% CAGRA, as NN-descent does not require a metric space to form the graph.}


\input{figures/deletion.tex}

\input{figures/deletion_query.tex}

\subsection{Deletion}
\label{subsec::deletion}

\RThreeInline{W2}{
Deletion in \sysname is split into three phases: mark, consolidate, and
compact. The performance of each of these phases of deletion can be seen in
~\Cref{tab:deletion_throughput_a100}. While consolidation is expensive due to
the need to search for every node that points to a deleted vertex, it is only
needed periodically; our empirical results show that up to 10\% of the dataset
can be atomically marked as deleted without affecting output quality or
throughput.}

\RThreeInline{W2}{
Query throughput before and after deletion can be seen
in~\Cref{tab:deletion_recall_throughput}. For both small and large vectors, the
recall is unaffected by deletion. For BigANN, the throughput is largely
unaffected by deletion, and graph degree is mostly stable, going from an
average degree of 44.2 to 45.0. For Gist, the throughput drops as the graph is
more densely connected after deletion: the deletion policy causes many new
connections to be added, resulting in average graph density growing from 24.4
to 30.6 after consolidation.}

\input{figures/roofline/roofline_both}

\subsection{Performance analysis} \label{eval:roofline}

\para{Roofline analysis} We characterize \sysname's performance on both
low-dimensional (\deep) and high-dimensional (\gist) vectors using the roofline
model~\cite{Williams2009}. \Cref{fig::roofline} compares the arithmetic
intensity and achieved throughput of \sysname, \sysnameRQ, and \cagra.
% with $K=10$.

Across both datasets, the roofline results indicate that \sysname operates
predominantly in a memory-bound regime, with operational intensities are
clustered tightly around 0.7–0.95 FLOP/byte. On DEEP, \sysname achieves peak
throughputs around 0.89-1.14 TFLOP/s at these low intensities, closely tracking
the sloped bandwidth roof. This behavior is consistent with ANNS workloads
dominated by irregular memory accesses during graph traversal, where additional
compute cannot be fully exploited without increasing data reuse. The comparable
intensity–performance envelope between \sysname and \cagra on \deep suggests
that both systems are similarly constrained by memory bandwidth, with
performance differences largely attributable to constant-factor effects such as
traversal efficiency and kernel scheduling rather than fundamental compute
utilization.

In contrast, \sysnameRQ significantly increases operational intensity, where
intensities rise to 5.0–6.2 FLOP/byte and achieved performance reaches up to
~1.83 TFLOP/s. This rightward shift on the roofline indicates substantially
improved arithmetic reuse, allowing \sysnameRQ to move closer to the compute
roof and escape the strict bandwidth-bound regime observed in \sysname.
Overall, these results show that \sysnameRQ’s reordering and query-time
computation strategies improve performance by reducing memory traffic. 
% The overhead of the additional vector components affects FLOPS on small
% vectors but is amortized out for large vectors, leading to clear roofline
% gains on large vector datasets like GIST.

%%% Commenting for space
% \para{Takeaways} \textit{\sysname and \cagra are both memory bound and have
% similar roofline plots close to the roofline, suggesting that the kernels are
% achieving close to ideal performance. Quantization significantly increases
% the arithmetic intensity of the kernels, suggesting that quantized ANNS
% performance can still be improved significantly.}

% \subsection{Microbenchmarks}
% \label{sec::microbenchmark}

% We analyze key design decisions in \sysname through a series of microbenchmarks.
% Here we present an ablation study isolating the contribution of each
% optimization; microbenchmarks on block size (\Cref{app:block-sweep}), coalesced
% versus tiled loading (\Cref{app:load-microbench}), and quantization methods
% (\Cref{app:quant-microbench}) are reported in the appendix.

\input{figures/ablation/ablation_fig.tex}

\para{Ablation study}
\RFourInline{W1}{}
\RThreeInline{D3}{
\Cref{fig::ablation} shows the ablation results. We start at a fully optimized kernel and remove
optimizations. We start at a full implementation with \RQ and ablate away
\RQ, chunked loads, optimized tile size, the use of a visited bit instead of
a hash table, and optimized block size in that order.
}

\RThreeInline{D3}{
For low-dimensional vectors such as \bigann, the ablation optimizations besides
\RQ are purely optimal, with performance increasing at all beam widths for
all optimizations. For \gist, All optimizations are optimal expect for the use
of visited bits, where the use of a hash table is better for all beam widths
when ablated. This speedup doesn't hold when all optimizations are applied due
to the optimized tile size: with more threads per tile, the amount of time
taken for distance calculations reduces, which lowers the penalty of
recalculating distances when using the visited set.
}


% Similarly to tile size, block size determines the
% amount of work that is scheduled per query, and makes a tradeoff between having
% more workers for each query or scheduling more queries in each CTA. the results
% for this microbenchmark can be seen in \Cref{fig::block_size}. For all vector
% sizes, we find that using the entirety of a CTA limits the memory parallelism
% available, as the requests for only one query will be issued from that CTA. For
% the large vectors, reducing the block size increases performance until the
% block size reaches 128. Below this point, performance drops due to the lack of
% compute available for each query, as distance calculations dominate performance
% of an individual query for these datasets.
%
% Results on smaller datasets are represented by performance on the \bigann
% dataset and can be seen in \Cref{fig::block_size_bigann}. For the small
% datasets, distance calculations are not the bottleneck, so increasing memory
% parallelism always results in increased performance. For \bigann and \deep, we
% find that reducing the block size (provided occupancy can does not degrade)
% always increases performance, with the highest performance block size being 32,
% down to a single warp per query. This maximizes memory performance by allowing
% for 32 different queries to be executed per CTA.
%
% \para{Takeaways} \textit{For small vector datasets, lowering the beam width
% increases performance as more queries are scheduled per SM. For large vector
% datasets, distance calculations dominate, making a larger beam width of 128
% optimal.}


% To measure the query performance of different quantization methods, we run the
% benchmark shown in~\Cref{fig:quantization}. We compare \sysname's exact
% distance and \RQ's distance against \cagra's exact distance and PQ distance.
% For a fair comparison, we evaluate \cagra’s PQ queries under two settings:
% \cagra PQ, where we configure its parameters to match the space usage of our
% \RQ setting (i.e., a 4$\times$ vector-size reduction), and \cagra PQ (default),
% where we leave \cagra’s quantization parameters unspecified and allow its
% heuristics to determine the configuration.
%
% CAGRA's memory accesses during vector distance calculation are highly
% optimized, and very efficient when loading large vector with high dimensions.
% In this benchmark, we observe that \cagra’s exact distance calculation performs
% slightly better than \sysname’s exact distance calculation. However, \sysname’s
% \RQ version outperforms all of \cagra’s variants, quantized or not. \cagra PQ
% achieves similar distance calculation performance as the exact version.
% Although PQ allows \cagra to reduce vector sizes, its inefficient distance
% computation during query time degrades performance. Overall, we conclude that
% \RQ is a superior choice for vector quantization in GPU workloads.
%
% \para{Takeaways} \textit{Reducing memory traffic does not directly correlate to
% improved performance. The indirections needed for Product quantization limit
% its effectiveness on GPUs. \RQ is a stronger quantization alternative for its
% better performance and lower space usage.}
%


%\input{figures/a100-deep-100M}
% \input{figures/deep100M-degree32}

% \subsection{Graph reordering}

% \Cref{tab::reordering} shows the performance of \sysname exact with and without reordering on all datasets. The results presented are on both host and device.

% For the device-only graphs, reordering is largely not beneficial. We find that for most datasets, reordering is either not helpful or is actively harmful, with reordering ranging from 5\% slower for no signficant change in overall performance. The only anomaly is OpenAI, which shows an 11\% increase in performance when using graph reordering. This increase in performance is due to the increased size of the vectors in this dataset. \hunter{This is a bad argument. Why is this happening? Let's rerun and verify this isn't noise.}

% \subsection{BigANN}

% The results for \bigann queries can be seen in \Cref{fig::a100_query}. For recall 1@1, \sysname is the fastest for all recalls up to .9837 recall, with peak throughput of 13.2 million queries per second at .31 recall. Above .9943 recall, \cagra is the fastest, with throughput of 837,925 queries per second at .9947 recall. \sysnameRQ is the second fastest index below .45 recall, but loses out to \cagra for higher recall values due to the lossiness of the quantization scheme. Parlay ANN is the fourth-fastest index for \bigann 1@1 for all recall values. but is over an order of magnitude slower than \sysname for most recall values due to being run only on CPU. 

% \bang is the fifth-fastest index for 1@1 queries and runs nearly two orders of magnitude slower than \sysname for the same accuracy. GANNS is the slowest of all indices for all recall values tested.

% For recall 10@10, \sysname is the fastest for all accuracies below .963 recall, with throughput of 1.6 million queries per second at .963 recall. Above that threshold, \cagra is the fastest algorithm with throughput of 816,000 queries per second at .985 recall. \sysnameRQ is strictly worse than \cagra for 10@10 recall due to the reduced accuracy of quantization. \sysnameRQ is strictly faster than \parlayann for a given recall value, which is strictly faster than \bang. GANNS is the slowest index for all recall values tested.

% For recall 50@50, \sysname has peak throughput of 1.49 million queries per second at .92 recall, and a max accuracy .987, with throughput of 300,000 queries per second that accuracy. The \sysnameRQ implementation has the second highest throughput at a peak of 1.22 million queries per second at 0.72 recall, but is slower for a given recall value than both \sysname and  \cagra. \cagra has the best recall/throughput trade off of any ANN tested for this benchmark, with peak throughput of 815,725 queries per second at 0.96 recall. \parlayann, GANNS, and \bang follow the same trends as previous k values, with \parlayann being the fourth fastest index, followed by \bang and GANNS.

% \subsection{Deep}

% Compared to \bigann, The \deep dataset has fewer dimensions, with 96 dimenions compared to 128, but each dimension is larger, being comprised of one float instead of a uint8\_t. This benefits both \cagra and the \RQ implementation: \cagra sees a  boost as they process all vectors as uint8\_t, causing a data blowup on \bigann that is not present in \deep, while the rabitQ implementation sees an 8x reduction in memory usage compared to the 2x reduction found in bigANN.

% For the \deep dataset recall 1@1, \sysname is the fastest for all sizes below .93 recall, followed by the RaBitQ variant and then \cagra. Above .93 recall, \cagra is the fastest, with peak throughput of 1.94 million queries per second at .964 recall. \parlayann is the fourth fastest index for \deep 1@1 recall, with peak throughput of 342,000 queries per second, followed by \bang and then by GANNS.

% For \deep 10@10, we see a similar trend. \sysnameRQ has the fastest query performance of any index with peak throughput of 3.56 million queries per second, but its scaling is limited due to its low accuracy. The exact version of \sysname is slightly faster than the RaBitQ variant at high accuracies, but both of them lose to \cagra as it achieves higher accuracies for the same throughput above .9 recall.

% For \deep 50@50, the curves entirely separate. \sysnameRQ has the lowest accuracy of any of the GPU ANN indices, but gets the highest throughput with 1.5 million queries per second at .76 recall. \sysname exact has higher recall than the RaBitQ variant for all beam widths but is slightly slower. \cagra has the highest accuracy of any ann index for the given beam width on this benchmark.

% \subsection{Gist}

% The \gist dataset is the second largest of the datasets provided and is composed of vectors of 960 floats. Distance is euclidean.

% On this dataset for recall 1@1, \sysnameRQ is the fastest for all recall values supported, with a peak throughput of 1.2 million queries per second. The high throughput of RaBitQ on this dataset is due to the reduced memory loads required per vector when using the quantized vectors. After RaBitQ, \cagra is the next-fastest ANN algorithm. Due to its lower accuracy, the RaBitQ variant cannot go above .971 recall. Above this point, \cagra is the fastest, achieving higher throughput than Jasper for the same accuracy. The full vector version of Jasper has consistently lower throughput than \cagra for a given recall. \parlayann has the second lowest throughput of any system on this benchmark, though it is capable of reaching the highest accuracy with 1@1 recall of .991. GANNS has the lowest throughput of any index on this dataset for all recall values and all k values.

% For 10@10 recall, RaBitQ is the fastest index for all recall values it supports, with peak throughput of  482,000 queries per second and peak recall of .958. \cagra is the second-fastest for all recall values, and achieves the second-highest recall value with peak recall of .997. Jasper exact is the third-fastest GPU ANN index for all supported recall values, and has a peak recall of .96. On this dataset, the accuracy costs of using RaBitQ are largely mitigated due the large number of dimensions, and the RaBitQ variant of Jasper doesn't see significantly reduced accuracy compared to the exact version, despite using only 1/8th of the total memory space. \parlayann is the fourth fastest index on this dataset, followed by GANNS.

% For 50@50 recall, RaBitQ is once again the fastest index for all supported sizes, but can only reach a max recall of .938. \cagra is the second fastest ANN index when the recall values overlap, followed by the exact Jasper index. \cagra has the highest potential recall of any GPU index, with peak recall of .995. Once again, \parlayann and GANNS are the slowest indices, with \parlayann outperforming GANNS on all recall values.


% \subsection{openAI}

% \openai is the largest of the datasets, with each vector being composed of 1,536 floats. Distance is Euclidean.

% For recall 1@1, Jasper RaBitQ is the fastest for most recall values supported, with peak throughput of 3.05 million queries per second. Jasper RaBitQ is the fastest index until .94 recall, at which point \cagra is the fastest index with throughput of 73,627 queries per second at .952 recall.

% Jasper full vector is the third-fastest ANNS index for all recall values supported with peak thorughput of 860,000 queries per second. \parlayann is the fourth fastest ANNS index for 1@1 recall for all supported recall values, followed by GANNS, which has the lowest throughput for all recall values.

% for 10@10 recall, Jasper RaBitQ is the fastest for all supported recall values, with peak throguhpit of of 447,000 queries per second and peak recall of .96. \cagra is the second fastest index, but can achieve higher accuracy than RaBitQ, with peak throughput of 237,441 and peak recall of .994 @ 9,900 queries per second.

% Once again, Jasper is the third-fastest index on this dataset, as it is restricted by the expensive distance calculations. It is followed by \parlayann and GANNS as the fourth and fifth fastest indices.

% This trend continues for \openai 50@50: RaBitQ is the fastest for all recall values supported and is followed by \cagra which can reach a higher level of accuracy. Jasper is the next fastest index for 50@50 recall, followed by \parlayann and then GANNS.

% \subsection{\textToImage}

% \textToImage (T2I) is a set of 10,000,000 200-dimensional float vectors. Unlike the datasets, distances in \textToImage are measured with inner product. To handle this, ... use... \hunter{Need to fill this in with details.}.

% For recall 1@1, Jasper acheives the single highest throughput at 16.7 million queries per second, but accuracy is much lower on this daaset than other datasets. Interestingly, the RaBitQ variant achieves higher accuracy than Jasper exact for all beam widths tested and achieves higher performance and higher accuracy. \cagra has the highest accuracy on this dataset with a peak recall of .983 and is the fastest index above .35 recall.

% \parlayann is the fourth fastest index and achieves higher accuracy than Jasper on this dataset, although its peak recall is limited to .86. GANNS is the slowest index for this dataset and does not achieve accuracy above .6.

% For 10@10 and 50@50 recall, the curves entirely separate. \cagra is the fastest and most accurate ANN index, followed by Jasper RaBitQ and then Jasper exact. \parlayann is the fourth-fastest index and the second most accurate index, followed by GANNS.

% \subsection{100@100}

% \Cref{fig::query_100_recall} shows the performance of all 6 systems when run on very large queries - returning the best 100 neighbors of every query vector. All three datasets show consistent trends: For a given throughput, \cagra has the highest recall for 100@100. \cagra is followed by Jasper, which in turn has higher recall than the raBitQ variant for all three datasets. For \gist, Japer RaBitQ is Pareto optimial for all sizes supported, with peak throughput of 83,581 at .82 recall. For the larger recall values \cagra is strictly optimal compared to the other systems tested. \parlayann is consistently the fourth-fastest index tested, followed by \bang as the fifth-fastest and then GANNS.


==> vldb26-revision/figures/4080-query.tex <==
\begin{figure*}[!htbp]
\centering
\ref{queryLegend4080}

\setlength{\tabcolsep}{0pt}

\begin{tabular}{c c}
\makebox[10pt][c]{\rotatebox[origin=c]{90}{\large Throughput in queries/secs (Log-Scale)}} &
\begin{tabular}{c c c c}

\input{figures/4080-bigann-k1} &
\input{figures/4080-bigann-k10} &
\input{figures/4080-bigann-k50} &
\input{figures/4080-bigann-k100} \\

\input{figures/4080-deep-k1} &
\input{figures/4080-deep-k10} &
\input{figures/4080-deep-k50} &
\input{figures/4080-deep-k100}

\end{tabular}
\end{tabular}

\vspace{0.5em}
\makebox[\textwidth][c]{\large Recall (\%)}

\caption{Query recall/throughput on the NVIDIA RTX 4080 Super (16~GB GDDR6X)
for the two datasets that fit in device memory at 10M points. Y-axis is on
log-scale; higher and more to the right is better.}
\label{fig::4080_query}
\vspace{-0.5em}
\end{figure*}


==> vldb26-revision/figures/a100-query.tex <==
% \begin{figure*}[t]
%     \centering
%     \ref{queryLegend}
    
%     \input{figures/a100-bigann-k1}\hfill
%     \input{figures/a100-bigann-k10}\hfill
%     \input{figures/a100-bigann-k50}\hfill
%     \input{figures/a100-bigann-k100}\hfill

%     \input{figures/a100-deep-k1}\hfill
%     \input{figures/a100-deep-k10}\hfill
%     \input{figures/a100-deep-k50}\hfill
%     \input{figures/a100-deep-k100}\hfill

%     \input{figures/a100-gist-k1}\hfill
%     \input{figures/a100-gist-k10}\hfill
%     \input{figures/a100-gist-k50}\hfill
%     \input{figures/a100-gist-k100}\hfill

%     \input{figures/a100-openai-k1}\hfill
%     \input{figures/a100-openai-k10}\hfill
%     \input{figures/a100-openai-k50}\hfill
%     \input{figures/a100-openai-k100}\hfill

%     \input{figures/a100-t2i-k1}\hfill
%     \input{figures/a100-t2i-k10}\hfill
%     \input{figures/a100-t2i-k50}\hfill
%     \input{figures/a100-t2i-k100}\hfill
%     \caption{Query recall/throughput curves for all datasets on A100. X-axis is recall, y-axis is throughput in queries per second. Recall is presented for 1@1, 10@10, and 50@50, and 100@100.}

%     \label{fig::a100_query}
%     \vspace{-.5em}
% \end{figure*}
\begin{figure*}[t]
\centering
\ref{queryLegend}


\setlength{\tabcolsep}{0pt}

\begin{tabular}{c c}
% ---- Global Y label ----
\makebox[10pt][c]{\rotatebox[origin=c]{90}{\large Throughput in queries/secs (Log-Scale)}} &
\begin{tabular}{c c c c}

% ===== Row 1 =====
\input{figures/a100-bigann-k1} &
\input{figures/a100-bigann-k10} &
\input{figures/a100-bigann-k50} &
\input{figures/a100-bigann-k100} \\

% ===== Row 2 =====
\input{figures/a100-deep-k1} &
\input{figures/a100-deep-k10} &
\input{figures/a100-deep-k50} &
\input{figures/a100-deep-k100} \\

% ===== Row 3 =====
\input{figures/a100-gist-k1} &
\input{figures/a100-gist-k10} &
\input{figures/a100-gist-k50} &
\input{figures/a100-gist-k100} \\

% ===== Row 4 =====
\input{figures/a100-openai-k1} &
\input{figures/a100-openai-k10} &
\input{figures/a100-openai-k50} &
\input{figures/a100-openai-k100} \\

% ===== Row 5 =====
\input{figures/a100-t2i-k1} &
\input{figures/a100-t2i-k10} &
\input{figures/a100-t2i-k50} &
\input{figures/a100-t2i-k100}

\end{tabular}
\end{tabular}

\vspace{0.5em}
\makebox[\textwidth][c]{\large Recall (\%)}

\caption{Query recall/throughput curves for various ANNS indexes across five datasets on Nvidia A100 GPU. We report recall at 1@1, 10@10, 50@50, and 100@100. Y-axis is on log-scale.
X-axis is recall. Higher and more to the right is better.}
\label{fig::a100_query}
\vspace{-0.5em}
\end{figure*}

% \begin{figure*}[t]
% \centering
% \ref{queryLegend}
% \setlength{\tabcolsep}{0pt}

% \begin{tabular}{c c}
% % ---- Global Y label ----
% \makebox[10pt][c]{\rotatebox[origin=c]{90}{\large Throughput (query/s)}} &
% \begin{tabular}{c c c}

% % ===== Row 1 =====
% \input{figures/a100-bigann-k10} &
% \input{figures/a100-deep-k10}&

% % ===== Row 2 =====
% \input{figures/a100-gist-k10} \\
% \input{figures/a100-openai-k10} &

% \input{figures/a100-t2i-k10}

% \end{tabular}
% \end{tabular}

% \vspace{0.5em}
% \makebox[\textwidth][c]{\large Recall (\%)}

% \caption{Query recall/throughput curves for all datasets on A100.
% X-axis is recall.}
% \label{fig::a100_query}
% \vspace{-0.5em}
% \end{figure*}


==> vldb26-revision/figures/ablation/ablation_fig.tex <==
\begin{figure}[t]
    \centering
    \ref{ablationLegend}
    \vspace{.2em}

    \input{figures/ablation/bigann_subfig}%
    \hfill
    \input{figures/ablation/gist_subfig}

    \caption{Ablation results for BigANN and Gist datasets.}
    \label{fig::ablation}
    \vspace{-1em}
\end{figure}

==> vldb26-revision/figures/ablation/bigann_subfig.tex <==
  \begin{subfigure}[t]{.48\columnwidth}
  \begin{tikzpicture}
    \centering
    \begin{axis}[
      ablationPlot,
      ymode=log,
      legend columns=3,
      legend style={at={(0.5,-0.3)}, anchor=north},
      legend to name=ablationLegend,
      xmin=.5
      ]

      \addplot[ablationRabitqStyle]   table [col sep=comma, x index=1, y index=2] {data/a100/ablation/bigann/full.txt};
      \addlegendentry{All Optimizations}

      \addplot[ablationChunkedStyle]   table [col sep=comma, x index=1, y index=2] {data/a100/ablation/bigann/sub_rabitq.txt};
      \addlegendentry{- RaBitQ}

      \addplot[ablationTile4Style]   table [col sep=comma, x index=1, y index=2] {data/a100/ablation/bigann/sub_chunked.txt};
      \addlegendentry{- Chunked Loads}

      \addplot[ablationNoHashStyle]   table [col sep=comma, x index=1, y index=2] {data/a100/ablation/bigann/sub_tile_size.txt};
      \addlegendentry{- Tile Size}

      \addplot[ablationBlock64Style]   table [col sep=comma, x index=1, y index=2] {data/a100/ablation/bigann/sub_hash_table.txt};
      \addlegendentry{- Visited Bits}

      \addplot[ablationBaseStyle]   table [col sep=comma, x index=1, y index=2] {data/a100/ablation/bigann/sub_block_size.txt};
      \addlegendentry{- Block Size}


    \end{axis}
  \end{tikzpicture}
  \caption{BigANN 10M 10@10 Ablation}
  \label{fig:bigann-k10-ablation}
  \end{subfigure}

==> vldb26-revision/figures/ablation/gist_subfig.tex <==
  \begin{subfigure}[t]{.48\columnwidth}
  \begin{tikzpicture}
    \centering
    \begin{axis}[
      ablationPlot,
      ymode=log,
      legend columns=3,
      legend style={at={(0.5,-0.3)}, anchor=north},
      legend to name=ablationLegend,
      xmin=.5
      ]

      \addplot[ablationRabitqStyle]   table [col sep=comma, x index=3, y index=2] {data/a100/ablation/gist/full.txt};
      \addlegendentry{All Optimizations}

      \addplot[ablationChunkedStyle]   table [col sep=comma, x index=3, y index=2] {data/a100/ablation/gist/sub_rabitq.txt};
      \addlegendentry{- RaBitQ}

      \addplot[ablationTile4Style]   table [col sep=comma, x index=3, y index=2] {data/a100/ablation/gist/sub_chunked.txt};
      \addlegendentry{- Chunked Loads}

      \addplot[ablationNoHashStyle]   table [col sep=comma, x index=3, y index=2] {data/a100/ablation/gist/sub_tile_size.txt};
      \addlegendentry{- Tile Size}

      \addplot[ablationBlock64Style]   table [col sep=comma, x index=3, y index=2] {data/a100/ablation/gist/sub_hash_table.txt};
      \addlegendentry{- Visited Bits}

      \addplot[ablationBaseStyle]   table [col sep=comma, x index=3, y index=2] {data/a100/ablation/gist/sub_block_size.txt};
      \addlegendentry{- Block Size}


    \end{axis}
  \end{tikzpicture}
  \caption{Gist 1M 10@10 Ablation}
  \label{fig:gist-k10-ablation}
  \end{subfigure}

==> vldb26-revision/figures/block_size.tex <==
\begin{figure}[t]
    \centering
    \ref{blockSizeLegend}
    \input{figures/block_size_bigann}\hfill
    \input{figures/block_size_gist}
    \caption{Varying Block size for \bigann and \gist. Throughput is in millions of queries per second, higher is better.}
    \label{fig::block_size}
\end{figure}

==> vldb26-revision/figures/construction/bigann_subfig.tex <==
%subfigure code - belongs to a full figure
\begin{subfigure}{.3\textwidth}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    insertPlot,
    legend to name=insertLegend,
    legend columns = 6,
    xlabel={Dataset Size},
    legend style={font=\small},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/jasper_bigann.txt};

    \addplot[cagraStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/cagra_bigann.txt};
    %  \addplot[jasperRqStyle] table [ x expr=\thisrowno{5}, y expr=\thisrowno{4}] {data/a40/jasper/bigann-k1-rabitq.txt};
    % \addplot[cagraStyle] table [ x expr=\thisrowno{1}, y expr=\thisrowno{0}] {data/a40/cagra/bigann-k1.txt};
    \addplot[parlayStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/parlay_bigann.txt};

    \addplot[gannsStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/ganns_bigann.txt};
    
    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
 
    \legend{Jasper, \cagra, \parlayann, GANNS}
    
  \end{axis}
  \end{tikzpicture}
  \caption{BigANN construction 1M-10M}
  \label{fig:bigann_construct}
\end{subfigure}

==> vldb26-revision/figures/construction/construction.tex <==
\begin{figure*}[t]
    \centering
    \ref{insertLegend}
    
    \input{figures/construction/bigann_subfig}\hfill
    \input{figures/construction/deep_subfig}\hfill
    \input{figures/construction/gist_subfig}\hfill

    \caption{Construction performance on A100.}

    \label{fig::construction}
    \vspace{-.5em}
\end{figure*}

==> vldb26-revision/figures/construction/deep_subfig.tex <==
%subfigure code - belongs to a full figure
\begin{subfigure}{.3\textwidth}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    insertPlot,
    legend columns = 6,
    xlabel={Dataset Size},
    legend style={font=\small},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=points, y=throughput]{data/a100/construction/jasper_deep.txt};

    \addplot[cagraStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/cagra_deep.txt};
    %  \addplot[jasperRqStyle] table [ x expr=\thisrowno{5}, y expr=\thisrowno{4}] {data/a40/jasper/bigann-k1-rabitq.txt};
    % \addplot[cagraStyle] table [ x expr=\thisrowno{1}, y expr=\thisrowno{0}] {data/a40/cagra/bigann-k1.txt};
    \addplot[parlayStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/parlay_deep.txt};

    \addplot[gannsStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/ganns_deep.txt};
    
    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
    
  \end{axis}
  \end{tikzpicture}
  \caption{Deep construction 1M-10M}
  \label{fig:deep_construct}
\end{subfigure}

==> vldb26-revision/figures/construction/gist_subfig.tex <==
%subfigure code - belongs to a full figure
\begin{subfigure}{.3\textwidth}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    insertPlot,
    legend columns = 6,
    xlabel={Dataset Size},
    legend style={font=\small},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=points, y=throughput]{data/a100/construction/jasper_gist.txt};

    \addplot[cagraStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/cagra_gist.txt};
    %  \addplot[jasperRqStyle] table [ x expr=\thisrowno{5}, y expr=\thisrowno{4}] {data/a40/jasper/bigann-k1-rabitq.txt};
    % \addplot[cagraStyle] table [ x expr=\thisrowno{1}, y expr=\thisrowno{0}] {data/a40/cagra/bigann-k1.txt};
    \addplot[parlayStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/parlay_gist.txt};

    \addplot[gannsStyle] table [col sep=comma, x=points, y=throughput] {data/a100/construction/ganns_gist.txt};
    
    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
    
  \end{axis}
  \end{tikzpicture}
  \caption{Gist construction 100k-1M}
  \label{fig:gist_construct}
\end{subfigure}

==> vldb26-revision/figures/construction/incremental_build.tex <==
%subfigure code - belongs to a full figure
\begin{figure}
\centering
\ref{incrementalLegend}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    incrementalBuildPlot,
    legend to name=incrementalLegend,
    legend columns = 6,
    xlabel={\% of Dataset Constructed},
    legend style={font=\small},
    ymode=log,
    % render every other point to reduce visual noise
    every axis plot/.append style={each nth point=2, filter discard warning=false},
    ]
    
    \addplot[jasperStyle] table [col sep=comma, x=n_points, y=throughput] {data/a100/incremental_build/bigann.txt};

    \addplot[gannsStyle] table [col sep=comma, x=n_points, y=throughput] {data/a100/incremental_build/deep.txt};

    \addplot[cagraStyle] table [col sep=comma, x=n_points, y=throughput] {data/a100/incremental_build/gist.txt};

    \addplot[bangStyle] table [col sep=comma, x=n_points, y=throughput] {data/a100/incremental_build/openai.txt};

    \addplot[parlayStyle] table [col sep=comma, x=n_points, y=throughput] {data/a100/incremental_build/t2i.txt};

    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
 
    \legend{\bigann, \deep, \gist, OpenAI, \textToImage}
    
  \end{axis}
  \end{tikzpicture}
  \caption{\sysname incremental construction throughput. X-axis is the \% of the dataset constructed so far, with each data point being the throughput for one batch. Y-axis is throughput on a log-scale, higher is better.}
\label{fig:incremental_jasper}
\vspace{-1em}
\end{figure}


==> vldb26-revision/figures/construction/incremental_comparison.tex <==
%subfigure code - belongs to a full figure
\begin{figure}
\centering
\ref{incrementalCompLegend}
\begin{tikzpicture}
  \centering
  \begin{axis}[
    incrementalCompPlot,
    legend to name=incrementalCompLegend,
    legend columns = 6,
    xlabel={\% of Dataset Constructed},
    legend style={font=\small},
    ymode=log,
    ]
    

    \addplot[cagraStyle] table [col sep=space, x=n_points, y=runtime_seconds] {data/a100/incremental_vs_full_construction/cagra_bigann.txt};

    \addplot[parlayStyle] table [col sep=space, x=n_points, y=runtime_seconds] {data/a100/incremental_vs_full_construction/parlay_bigann.txt};

    \addplot[gannsStyle] table [col sep=space, x=n_points, y=runtime_seconds] {data/a100/incremental_vs_full_construction/ganns_bigann.txt};

    \addplot[jasperStyle] table [col sep=space, x=n_points, y=runtime_seconds] {data/a100/incremental_vs_full_construction/jasper_bigann.txt};

    % \addplot[jasperStyle, x=recall, y=throughput]   table {data/a40/jasper/bigann-k1.txt};
 
    \legend{\cagra, \parlayann, GANNS, Jasper}
    
  \end{axis}
  \end{tikzpicture}
  \caption{Incremental vs non-incremental construction time for \bigann
  10M. \sysname and \parlayann support batch incremental updates. \cagra and
\ganns do not support updates and need to be built from scratch at each step. X-axis is percentage of dataset constructed and each data point is a further $\frac{1}{10}$th of dataset constructed.
Y-axis is on log-scale, lower is better.}
  \label{fig:incremental_comparison}
  \vspace{-1em}
\end{figure}


==> vldb26-revision/figures/construction/load_comparison.tex <==
% \begin{figure}[ht]
% \centering

% \begin{tikzpicture}
%     \centering
%     \begin{axis}[
%         ybar,
%         bar width=10pt,
%         width=\columnwidth,
%         height=.6\columnwidth,
%         enlarge x limits=0.1,
%         ylabel={Throughput (MQueries/S)},
%         symbolic x coords={bigann (w=1), deep (w=1), gist (w=1), bigann (w=256), deep (w=256), gist (w=256)},
%         xtick=data,
%         xticklabel style={rotate=45, anchor=east},
%         legend style={at={(0.5,1.05)}, anchor=south, legend columns=-1},
%         ymajorgrids=true,
%         grid style=dashed,
%         scaled ticks=false,
%         y filter/.code={\pgfmathparse{#1/1e6}\pgfmathresult}
%     ]
    
%     % Load and plot first CSV (e.g., Method A)
%     \addplot[cagraStyleFill] table [x=label, y=value, col sep=comma] {data/a100/microbenchmarks/original.txt};
%     \addlegendentry{Tiled}
    
%     % Load and plot second CSV (e.g., Method B)
%     \addplot[jasperStyleFill] table [x=label, y=value, col sep=comma] {data/a100/microbenchmarks/tuned.txt};
%     \addlegendentry{Chunked}
    
%     \end{axis}
%   \end{tikzpicture}


% \caption{Difference in tiled and chunked load strategies. X-axis is queries for three datasets with beam width=1 and beam width=256. Y-axis is throughput of queries in millions of queries per second. For smaller beam widths, the chunked strategy provides lower latency as all load requests are issued simultaneously. For higher beam widths, total throughput dominates, resulting in identical performance.}
% \label{fig::load_comparison}
% \end{figure}

\setlength{\tabcolsep}{3.5pt}
\begin{table}
\begin{center}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c c c|c c c|} 
 \toprule
  & \multicolumn{3}{c|}{Beam width=1} & \multicolumn{3}{c|}{Beam width=256}\\
  & \bigann&\deep&\gist&\bigann&\deep&\gist\\  
 \midrule
 Tiled &8.398& 6.701 & .690 &.095 &.089& .024\\
 Chunked & 9.611 & 7.622 & .769 & .095 & .089 & .024\\
 \bottomrule
\end{tabular}
% }
\end{center}
\caption{Difference in tiled and chunked load strategies. Table results are throughput in millions of queries per second. For smaller beam widths, the chunked strategy provides lower latency as all load requests are issued simultaneously. For higher beam widths, total memory throughput dominates, resulting in identical performance.}
\label{tab::load_comparison}
\end{table}

==> vldb26-revision/figures/deletion_query.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{lrrrr}
  \toprule
                & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{Post-consolidation} \\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5}
  Dataset       & Recall@10 & QPS       & Recall@10 & QPS       \\
  \midrule
  \bigann 10M     & 0.986 & 574{,}990 & 0.988 & 563{,}998 \\
  \gist 1M        & 0.922 & 54{,}471  & 0.925 & 42{,}539  \\
  \bottomrule
  \end{tabular}
  \caption{Live recall@10 and query throughput before and after deletion+consolidation on A100 for small and large vectors ($10\%$ of dataset deleted, beam width 128).}
  \label{tab:deletion_recall_throughput}
  \vspace{-2em}
  \end{table}


==> vldb26-revision/figures/h200-query.tex <==
\begin{figure*}[!htbp]
\centering
\ref{queryLegendH200}

\setlength{\tabcolsep}{0pt}

\begin{tabular}{c c}
\makebox[10pt][c]{\rotatebox[origin=c]{90}{\large Throughput in queries/secs (Log-Scale)}} &
\begin{tabular}{c c c c}

\input{figures/h200-deep-k1} &
\input{figures/h200-deep-k10} &
\input{figures/h200-deep-k50} &
\input{figures/h200-deep-k100}

\end{tabular}
\end{tabular}

\vspace{0.5em}
\makebox[\textwidth][c]{\large Recall (\%)}

\caption{Query recall/throughput on the NVIDIA H200 (140~GB HBM3E) for
\deep at 200M points. Y-axis is on log-scale; higher and more to the right is
better. \cagra was forced onto its IVF construction path because NN-Descent
exceeded available device memory at this scale (see~\Cref{app:memory}).}
\label{fig::h200_query}
\vspace{-0.5em}
\end{figure*}


==> vldb26-revision/figures/loads/load_tiled.tex <==
\begin{subfigure}[t]{.2\textwidth}
\centering
\begin{tikzpicture}[x=0.15\textwidth, y=0.05\textwidth] % scale to fit subfigure
  % force a bounding box to ensure horizontal alignment
  \useasboundingbox (0,-1) rectangle (8,4);  % adjust to cover your drawing

  % define colors
  \definecolor{cadmium}{HTML}{F28C28}
  \definecolor{celadon}{HTML}{AFE1AF}
  \definecolor{periwinkle}{HTML}{CCCCFF}

  % helper commands
  \newcommand{\roundedbox}[5]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}  % width
      \def\H{#4}  % height
      \def\R{0.25cm} % corner radius
      \draw[thick, rounded corners=\R] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }
  \newcommand{\colorroundedbox}[6]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}  % width
      \def\H{#4}  % height
      \def\R{0.25cm} % corner radius
      \draw[thick, rounded corners=\R, fill=#6] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }

  % drawing content
  \draw[thick, black](0,3.25) node [anchor=west]{Warp};
  \colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
  \colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
  \colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
  \colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

  \draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
  \roundedbox{0}{0}{10}{1}{}

  % colored slices
  \foreach \x in {0,0.5,...,7.5} {
    \pgfmathparse{int(mod(\x*2,4))}
    \edef\c{\pgfmathresult}
    \ifnum\c=0 \colorroundedbox{\x}{0}{0.5}{1}{}{pink} \fi
    \ifnum\c=1 \colorroundedbox{\x}{0}{0.5}{1}{}{periwinkle} \fi
    \ifnum\c=2 \colorroundedbox{\x}{0}{0.5}{1}{}{celadon} \fi
    \ifnum\c=3 \colorroundedbox{\x}{0}{0.5}{1}{}{cadmium} \fi
  }

  % draw diagram line
  \draw[thick] (0, 0) -- (0, -.25) -- (2,-.25) -- (2,0) -- (2,-.25) -- (1,-.25) -- (1,-.5);
  \draw[thick, black](2.25,-.5) node [anchor=north]{1-4 Bytes loaded per thread per round};

\end{tikzpicture}
\caption{Tiled load strategy}
\label{fig::cache_diagram}
\end{subfigure}


==> vldb26-revision/figures/loads/loads.tex <==
\begin{figure}[t]
\centering

% ===== Subfigure 1 =====
\begin{subfigure}[t]{.45\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
  \useasboundingbox (0,-1) rectangle (10,4);

  % Colors
  \definecolor{cadmium}{HTML}{F28C28}
  \definecolor{celadon}{HTML}{AFE1AF}
  \definecolor{periwinkle}{HTML}{CCCCFF}

  % Helper commands
  \newcommand{\roundedbox}[5]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }
  \newcommand{\colorroundedbox}[6]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R, fill=#6] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }

  % Diagram content
  \draw[thick, black](0,3.25) node [anchor=west]{Warp};
  \colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
  \colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
  \colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
  \colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

  \draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
  \roundedbox{0}{0}{10}{1}{}

  % Colored slices
  \foreach \x/\c in {0/pink, 0.5/periwinkle,1/celadon,1.5/cadmium,
                     2/pink,2.5/periwinkle,3/celadon,3.5/cadmium,
                     4/pink,4.5/periwinkle,5/celadon,5.5/cadmium,
                     6/pink,6.5/periwinkle,7/celadon,7.5/cadmium} {
    \colorroundedbox{\x}{0}{0.5}{1}{}{\c}
  }

  % Vertical lines
  % \foreach \x in {0.5,1,1.5,2.5,3,3.5,4.5,5,5.5,6.5,7,7.5} {
  %   \draw[thick] (\x,0) -- (\x,1);
  % }

  % Bottom diagram line
  \draw[thick] (0,0) -- (0,-.25) -- (2,-.25) -- (2,0) -- (2,-.25) -- (1,-.25) -- (1,-.5);
  \draw[thick, black](2,-.5) node [anchor=north]{1-4 Bytes loaded per thread per round};
\end{tikzpicture}%
}
\caption{Tiled load strategy}
\label{fig::cache_diagram1}
\end{subfigure}


% ===== Subfigure 2 =====
\begin{subfigure}[t]{.45\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
  \useasboundingbox (0,-1) rectangle (10,4);

  % Colors
  \definecolor{cadmium}{HTML}{F28C28}
  \definecolor{celadon}{HTML}{AFE1AF}
  \definecolor{periwinkle}{HTML}{CCCCFF}

  % Helper commands
  \newcommand{\roundedbox}[5]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }
  \newcommand{\colorroundedbox}[6]{%
    \begin{scope}[shift={(#1,#2)}]
      \def\W{#3}
      \def\H{#4}
      \def\R{0.25cm}
      \draw[thick, rounded corners=\R, fill=#6] (0,0) rectangle (\W,\H);
      \node[align=center] at ({\W/2},{\H/2}) {#5};
    \end{scope}%
  }

  % Diagram content
  \draw[thick, black](0,3.25) node [anchor=west]{Warp};
  \colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
  \colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
  \colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
  \colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

  \draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
  \roundedbox{0}{0}{10}{1}{}

  % Colored slices
  \foreach \x/\c in {0/pink,2/periwinkle,4/celadon,6/cadmium} {
    \colorroundedbox{\x}{0}{2}{1}{}{\c}
  }

  % Vertical lines
  \foreach \x in {0.5,1,1.5,2.5,3,3.5,4.5,5,5.5,6.5,7,7.5} {
    \draw[thick] (\x,0) -- (\x,1);
  }

  % Bottom diagram line
  \draw[thick] (0,0) -- (0,-.25) -- (8,-.25) -- (8,0) -- (8,-.25) -- (4,-.25) -- (4,-.5);
  \draw[thick, black](4,-.5) node [anchor=north]{16 Bytes loaded per thread per round};
\end{tikzpicture}%
}
\caption{Chunked load strategy}
\label{fig::cache_diagram2}
\end{subfigure}

\caption{Comparison of the two different load strategies tested in Jasper: tiled loads load one object per thread in the tile at a time, whereas the chunked load strategy loads a fixed amount of data (16 bytes) per thread and has each thread work on all objects loaded in that chunk.}
\label{fig:load_strategies}
\end{figure}

\begin{figure}
    \centering
    %TODO: Decide which one to use
    \includegraphics[width=\linewidth]{figures/graphs/tiled_vs_chunked.pdf}
    \includegraphics[width=\linewidth]{figures/graphs/tiled_vs_chunked_graph_only.pdf}
    \caption{Comparison of the two different load strategies tested in Jasper: tiled loads load one object per thread in the tile at a time, whereas the chunked load strategy loads a fixed amount of data (16 bytes) per thread and has each thread work on all objects loaded in that chunk.}
\end{figure}


==> vldb26-revision/figures/loads/old_load_coalesced.tex <==

%visualization of \parlayann algorithm
\begin{subfigure}{.2\textwidth}
\centering
% \begin{tikzpicture}[line width=3pt,rounded corners=3pt, x=0.5cm, y=0.5cm]

\newcommand{\roundedbox}[5]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\newcommand{\colorroundedbox}[6]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R, fill=#6]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\makebox[\linewidth][c]{%
\begin{tikzpicture}[
    membox/.style={draw, rounded corners=2pt, minimum width=2.2cm, minimum height=0.8cm, align=center},
    block/.style={draw, minimum height=0.9cm, rounded corners=1pt},
    subblock/.style={draw, minimum height=0.9cm, minimum width=0.9cm},
    warp/.style={draw, fill=gray!8, rounded corners=1pt, minimum height=0.8cm},
    small/.style={draw, minimum height=0.55cm, minimum width=0.9cm},
    arrowstyle/.style={thick},
    baseline=(current bounding box.north),
    scale=1
]

\definecolor{cadmium}{HTML}{F28C28}

\definecolor{celadon}{HTML}{AFE1AF}

\definecolor{periwinkle}{HTML}{CCCCFF}



\draw[thick, black](0,3.25) node [anchor=west]{Warp};

\colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
\colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
\colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
\colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

% \roundedbox{0}{2}{1.5}{1}{Thread 1}
% \roundedbox{1.6}{2}{1.5}{1}{Thread 2}
% \roundedbox{3.2}{2}{1.5}{1}{Thread 3}
% \roundedbox{4.8}{2}{1.5}{1}{Thread 4}

\draw[thick, black](0,1.25) node [anchor=west]{Data Vector};

\roundedbox{0}{0}{10}{1}{}

\colorroundedbox{0}{0}{2}{1}{}{pink}
\colorroundedbox{2}{0}{2}{1}{}{periwinkle}
\colorroundedbox{4}{0}{2}{1}{}{celadon}
\colorroundedbox{6}{0}{2}{1}{}{cadmium}


%new lines
\draw[thick] (.5, 0) -- (0.5, 1) node [anchor=west] {};
\draw[thick] (1, 0) -- (1, 1) node [anchor=west] {};
\draw[thick] (1.5, 0) -- (1.5, 1) node [anchor=west] {};

\draw[thick] (2.5, 0) -- (2.5, 1) node [anchor=west] {};
\draw[thick] (3, 0) -- (3, 1) node [anchor=west] {};
\draw[thick] (3.5, 0) -- (3.5, 1) node [anchor=west] {};

\draw[thick] (4.5, 0) -- (4.5, 1) node [anchor=west] {};
\draw[thick] (5, 0) -- (5, 1) node [anchor=west] {};
\draw[thick] (5.5, 0) -- (5.5, 1) node [anchor=west] {};

\draw[thick] (6.5, 0) -- (6.5, 1) node [anchor=west] {};
\draw[thick] (7, 0) -- (7, 1) node [anchor=west] {};
\draw[thick] (7.5, 0) -- (7.5, 1) node [anchor=west] {};

\draw[thick] (0, 0) -- (0, -.25) -- (8,-.25) -- (8,0) -- (8,-.25) -- (4,-.25) -- (4,-.5) node [anchor=west] {};

\draw[thick, black](4,-.5) node [anchor=north]{16 Bytes loaded per thread per round};


%Strat 1 - tiled load
%Have colored slices taken from the beveling?



\end{tikzpicture}
}
\caption{Chunked load strategy }
\label{fig::cache_diagram}
\end{subfigure}




==> vldb26-revision/figures/loads/old_load_tiled.tex <==

%visualization of \parlayann algorithm
\begin{subfigure}{.2\textwidth}
\centering
% \begin{tikzpicture}[line width=3pt,rounded corners=3pt, x=0.5cm, y=0.5cm]

\newcommand{\roundedbox}[5]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\newcommand{\colorroundedbox}[6]{%
  \begin{scope}[shift={(#1,#2)}]
    \def\W{#3}  % width
    \def\H{#4}  % height
    \def\R{0.25cm} % corner radius

    % Draw rounded rectangle
    \draw[thick, rounded corners=\R, fill=#6]
      (0,0) rectangle (\W,\H);

    % Centered text
    \node[align=center] at ({\W/2},{\H/2}) {#5};
  \end{scope}
}

\makebox[\linewidth][c]{%
\begin{tikzpicture}[
    membox/.style={draw, rounded corners=2pt, minimum width=2.2cm, minimum height=0.8cm, align=center},
    block/.style={draw, minimum height=0.9cm, rounded corners=1pt},
    subblock/.style={draw, minimum height=0.9cm, minimum width=0.9cm},
    warp/.style={draw, fill=gray!8, rounded corners=1pt, minimum height=0.8cm},
    small/.style={draw, minimum height=0.55cm, minimum width=0.9cm},
    arrowstyle/.style={thick},
    baseline=(current bounding box.north),
    scale=1
]

\definecolor{cadmium}{HTML}{F28C28}

\definecolor{celadon}{HTML}{AFE1AF}

\definecolor{periwinkle}{HTML}{CCCCFF}

\draw[thick, black](0,3.25) node [anchor=west]{Warp};

\colorroundedbox{0}{2}{1.5}{1}{Thread 1}{pink}
\colorroundedbox{1.6}{2}{1.5}{1}{Thread 2}{periwinkle}
\colorroundedbox{3.2}{2}{1.5}{1}{Thread 3}{celadon}
\colorroundedbox{4.8}{2}{1.5}{1}{Thread 4}{cadmium}

\draw[thick, black](0,1.25) node [anchor=west]{Data Vector};
\roundedbox{0}{0}{10}{1}{}


\colorroundedbox{0}{0}{.5}{1}{}{pink}
\colorroundedbox{.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{1}{0}{.5}{1}{}{celadon}
\colorroundedbox{1.5}{0}{.5}{1}{}{cadmium}

\colorroundedbox{2}{0}{.5}{1}{}{pink}
\colorroundedbox{2.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{3}{0}{.5}{1}{}{celadon}
\colorroundedbox{3.5}{0}{.5}{1}{}{cadmium}

\colorroundedbox{4}{0}{.5}{1}{}{pink}
\colorroundedbox{4.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{5}{0}{.5}{1}{}{celadon}
\colorroundedbox{5.5}{0}{.5}{1}{}{cadmium}

\colorroundedbox{6}{0}{.5}{1}{}{pink}
\colorroundedbox{6.5}{0}{.5}{1}{}{periwinkle}
\colorroundedbox{7}{0}{.5}{1}{}{celadon}
\colorroundedbox{7.5}{0}{.5}{1}{}{cadmium}

%draw diagram
\draw[thick] (0, 0) -- (0, -.25) -- (2,-.25) -- (2,0) -- (2,-.25) -- (1,-.25) -- (1,-.5) node [anchor=west] {};

\draw[thick, black](2.25,-.5) node [anchor=north]{1-4 Bytes loaded per thread per round};


%Strat 1 - tiled load
%Have colored slices taken from the beveling?

\end{tikzpicture}
}
\caption{Tiled load strategy}
\label{fig::cache_diagram}
\end{subfigure}




==> vldb26-revision/figures/plot_data.tex <==

\pgfplotsset{
  recallPlot/.style={
    small,
    width = 1.2\columnwidth,
    height = .7\columnwidth,
    table/col sep=comma,
    xlabel near ticks,
    x label style={at={(0.5,-0.2)},font=\small},
    y label style={at={(-0.2,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
    xmax=1.02,
    xmin=-0.02
  },
}

\pgfplotsset{
  ablationPlot/.style={
    small,
    width = 1.1\columnwidth,
    height = 0.9\columnwidth,
    table/col sep=comma,
    xlabel near ticks,
    x label style={at={(0.5,-0.2)},font=\small},
    y label style={at={(-0.2,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
    xmax=1.02,
    xmin=-0.02
  },
}

\pgfplotsset{
  rooflinePlot/.style={
    small,
    width = 1.1\columnwidth,
    height = 1.0\columnwidth,
    table/col sep=space,
    xlabel near ticks,
    x label style={at={(0.5,-0.3)},font=\small},
    y label style={at={(-0.2,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
    xmin=0.01, xmax=1000,
    ymin=0.1, ymax=100,
  },
}

\pgfplotsset{
  quantizationPlot/.style={
    small,
    width = 1.1\columnwidth,
    height = .7\columnwidth,
    ylabel={Throughput},
    table/col sep=comma,
    xlabel near ticks,
    x label style={at={(0.5,-0.2)},font=\small},
    y label style={at={(-0.15,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
    xmax=1.05,
  },
}

\pgfplotsset{
  insertPlot/.style={
    small,
    width = 1.1\columnwidth,
    height = .7\columnwidth,
    ylabel={Throughput (inserts/s)},
    table/col sep=comma,
    xlabel near ticks,
    x label style={at={(0.5,-0.12)},font=\small},
    y label style={at={(-0.15,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
    xmax=1.05,
  },
}

\pgfplotsset{
  incrementalBuildPlot/.style={
    small,
    width = .85\columnwidth,
    height = .4\columnwidth,
    ylabel={Throughput (inserts/s)},
    table/col sep=comma,
    xlabel near ticks,
    x label style={at={(0.5,-0.12)},font=\small},
    y label style={at={(-0.15,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
  },
}

\pgfplotsset{
  incrementalCompPlot/.style={
    small,
    width = .85\columnwidth,
    height = .4\columnwidth,
    ylabel={Update Time (Seconds)},
    table/col sep=comma,
    xlabel near ticks,
    x label style={at={(0.5,-0.12)},font=\small},
    y label style={at={(-0.15,0.5)},font=\small},
    ytick style={draw=none},
    ytick scale label code/.code = {},
    yticklabel style={ /pgf/number format/fixed },
    ymajorgrids,
    %yminorgrids,
    minor tick num=1,
    minor grid style={draw=gray!25},
  },
}


\pgfplotsset{
    ablationBaseStyle/.style={color=gray!60, mark=*, mark size=1.5pt, thick, dashed},
    ablationBlock64Style/.style={color=gray!80!blue, mark=square*, mark size=1.5pt, thick},
    ablationNoHashStyle/.style={color=blue!50, mark=triangle*, mark size=1.5pt, thick},
    ablationTile4Style/.style={color=blue!70, mark=diamond*, mark size=1.5pt, thick},
    ablationChunkedStyle/.style={color=blue!90, mark=pentagon*, mark size=1.5pt, thick},
    ablationRabitqStyle/.style={color=red!80!orange, mark=*, mark size=2pt, very thick},
  }

% \pgfplotsset{
%   insertPlot/.style={
%     small,
%     width = 1.1\columnwidth,
%     height = .7\columnwidth,
%     ylabel={Throughput (inserts/s)},
%     table/col sep=comma,
%     xlabel near ticks,
%     x label style={at={(0.5,-0.12)},font=\small},
%     y label style={at={(-0.1,0.5)},font=\small},
%     ytick style={draw=none},
%     ytick scale label code/.code = {},
%     yticklabel style={ /pgf/number format/fixed },
%     ymajorgrids,
%     %yminorgrids,
%     minor tick num=1,
%     minor grid style={draw=gray!25}
%   },
% }

\definecolor{rose}{HTML}{B8336A}

\definecolor{turq}{HTML}{48D1CC}

\definecolor{medGreen}{HTML}{027148}

\definecolor{lightGreen}{HTML}{D3F7AD}

\definecolor{khaki}{HTML}{6A5F31}

\definecolor{skysurge}{HTML}{5BC0EB}

\definecolor{bananacream}{HTML}{FDE74C}

\definecolor{magenta}{HTML}{822E81}

\definecolor{rosewood}{HTML}{AA6373}

% \definecolor{mintGreen}{HTML}{A6FBB2}
\definecolor{mintGreen}{HTML}{98FF98}

\definecolor{gold}{HTML}{FFB703}

\definecolor{strongred}{HTML}{D62828}

\definecolor{forestGreen}{HTML}{228C22}

%\definecolor{strongblue}{HTML}{FF0883}
\definecolor{strongblue}{HTML}{FF7F0F}

\definecolor{weakpurple}{HTML}{38B2AC}

\definecolor{weakblue}{HTML}{3A86FF}

\definecolor{weakgray}{HTML}{285D34}

\definecolor{weakcyan}{HTML}{1982C4}

\pgfplotsset{
  jasperStyle/.style = {color = strongred, mark = square*, mark size=1.5pt, thick},
  jasperRqStyle/.style = {color = strongblue, mark = square*, mark size=1.5pt, thick},
  jasperHostStyle/.style = {color = red, mark = *, mark size=1.5pt, , dash pattern = on 1.5pt off 1pt, thick},
  cagraStyle/.style = {color = weakpurple, mark = *, mark size=1.5pt, thick},
  parlayStyle/.style = {color = weakblue, mark = triangle*, mark size=1.5pt, thick},
  bangStyle/.style = {color=weakgray, mark = diamond*, mark size=1.5pt, thick},
  gannsStyle/.style = {color=weakcyan, mark = pentagon*, mark size=1.5pt, thick},
  warpcoreStyle/.style = {color=forestGreen, mark = square*},
  p2MetaStyle/.style = {color=black, mark = diamond*},  cuckooStyle/.style = {color=turq,mark=square*},
  doubleMetaStyle/.style = {color=brown, mark = triangle*},
  bchtStyle/.style = {color=cyan, mark = square*},
  p2bhtStyle/.style = {color=lightGreen, mark = square*},
  slabStyle/.style = {color=gold, mark = square*},
  p2ExtStyleFill/.style = {fill = red},
  p2IntStyleFill/.style = {fill=cyan},
  doubleStyleFill/.style = {fill=orange},
  ihtStyleFill/.style = {fill=magenta},
  ihtMetaStyleFill/.style = {fill=medGreen},
  chainingStyleFill/.style = {fill=violet},
  warpcoreStyleFill/.style = {fill=forestGreen},
  p2MetaStyleFill/.style = {fill=black},
  doubleMetaStyleFill/.style = {fill=brown},
  cuckooStyleFill/.style = {fill=turq},
  jasperStyleFill/.style = {fill=strongred},
  cagraStyleFill/.style = {fill = weakpurple},
  jasperThickStyle/.style = {color = strongred, mark = *, mark size=1.5pt, thick},
  jasperRqThickStyle/.style = {color = strongblue, mark = *, mark size=1.5pt, thick},
  cagraThickStyle/.style = {color = weakpurple, mark = *, mark size=1.5pt, thick},
}


==> vldb26-revision/figures/query_100_recall.tex <==
\begin{figure*}[t]
    \centering
    \ref{queryLegend100}
    
    \input{figures/a100-bigann-k100}\hfill
    \input{figures/a100-deep-k100}\hfill
    \input{figures/a100-gist-k100}\hfill
    \input{figures/a100-openai-k100}\hfill
    \input{figures/a100-t2i-k100}
    \caption{100@100 recall/throughput curves for all datasets on A100. X-axis is 100@100 recall, y-axis is throughput in queries oper second.}

    \label{fig::query_100_recall}
    \vspace{-.5em}
\end{figure*}

==> vldb26-revision/figures/roofline/bigann_roofline.tex <==
\begin{subfigure}{.45\columnwidth}
\centering
\begin{tikzpicture}
\begin{loglogaxis}[
    rooflinePlot,
    xlabel={Operational Intensity (OP/Byte)},
    ylabel={Performance (TOP/s)},
    legend to name=rooflineLegend,
    legend columns = 2,
    xtick={0.1, 1, 10, 100, 1000},
]

\addplot[jasperThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/bigann_jasper.txt};

\addplot[jasperRqThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/bigann_rq.txt};

% Memory bandwidth bound (A100 HBM2e: ~1.7 TB/s measured)
\addplot[black, thick, domain=0.01:12.2] {1.7e12*x/1e12};

% Compute bound (A100: ~20.74 TFLOP/s FP32 equivalent)
\addplot[black, thick, domain=12.2:1000000] {20.74e12/1e12};

% Ridge point line
\addplot[
    densely dotted,
    thick,
    black
] coordinates {(12.2,1e-3) (12.2,1e3)};

\legend{\sysname, \sysnameRQ}

\end{loglogaxis}
\end{tikzpicture}
\caption{Roofline model for \bigann when k=10}
\end{subfigure}


==> vldb26-revision/figures/roofline/deep_roofline.tex <==
\begin{subfigure}{.45\columnwidth}
\centering
\begin{tikzpicture}
\begin{loglogaxis}[
    rooflinePlot,
    xlabel={Operational Intensity (FLOP/Byte)},
    ylabel={Performance (TFLOP/s)},
    legend to name=rooflineLegend,
    legend columns = 3,
    xtick={0.1, 1, 10, 100, 1000},
    %y filter/.code={\pgfmathparse{#1/1e12}\pgfmathresult}
]

\addplot[cagraThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/deep_cagra.txt};

\addplot[jasperThickStyle] table [x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/deep_jasper.txt};

\addplot[jasperRqThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/deep_rq.txt};



% Memory bandwidth bound (HBM2e: ~1.6 TB/s)
% \addplot[black, thick, domain=0.01:12.2] {1.6*x*1e12};

% % Compute bound (A100: ~19.5 TFLOP/s FP32)
% \addplot[black, thick, domain=12.2:1000000] {19.5*1e12};

% Memory bandwidth bound (raw FLOPS input, auto-scaled to TFLOPS display)
\addplot[black, thick, domain=0.01:12.2] {1.7e12*x/1e12};

% Compute bound (raw FLOPS input, auto-scaled to TFLOPS display)
\addplot[black, thick, domain=12.2:1000000] {20.74e12/1e12};

% Ridge point
% \addplot[mark=*, mark size=3pt, only marks, red] coordinates {(12.2, 19.5)};

% Ridge point line
\addplot[
    densely dotted,
    thick,
    black
] coordinates {(12.2,1e-3) (12.2,1e3)};


% \legend{Memory Bound, Compute Bound, Ridge Point}

\legend{\cagra, \sysname, \sysnameRQ}

\end{loglogaxis}
\end{tikzpicture}
\caption{%Roofline model for the 
Deep dataset when k=10}
\end{subfigure}


==> vldb26-revision/figures/roofline/gist_roofline.tex <==
\begin{subfigure}{.45\columnwidth}
\centering
\begin{tikzpicture}
\begin{loglogaxis}[
    rooflinePlot,
    xlabel={Operational Intensity (FLOP/Byte)},
    ylabel={Performance (TFLOP/s)},
    legend to name=rooflineLegend,
    legend columns = 3,
    xtick={0.1, 1, 10, 100, 1000},
    %y filter/.code={\pgfmathparse{#1/1e12}\pgfmathresult}
]

\addplot[cagraThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/gist_cagra.txt};

\addplot[jasperThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/gist_jasper.txt};

\addplot[jasperRqThickStyle] table [ x expr=\thisrowno{0}, y expr=\thisrowno{1}/1e12] {data/a100/roofline/gist_rq.txt};



% Memory bandwidth bound (HBM2e: ~1.6 TB/s)
% \addplot[black, thick, domain=0.01:12.2] {1.6*x*1e12};

% % Compute bound (A100: ~19.5 TFLOP/s FP32)
% \addplot[black, thick, domain=12.2:1000000] {19.5*1e12};

% Memory bandwidth bound (raw FLOPS input, auto-scaled to TFLOPS display)
\addplot[black, thick, domain=0.01:12.2] {1.7e12*x/1e12};

% Compute bound (raw FLOPS input, auto-scaled to TFLOPS display)
\addplot[black, thick, domain=12.2:1000000] {20.74e12/1e12};

% Ridge point
% \addplot[mark=*, mark size=3pt, only marks, red] coordinates {(12.2, 19.5)};

% Ridge point line
\addplot[
    densely dotted,
    thick,
    black
] coordinates {(12.2,1e-3) (12.2,1e3)};

% \legend{Memory Bound, Compute Bound, Ridge Point}

\legend{\cagra, \sysname, \sysnameRQ}

\end{loglogaxis}
\end{tikzpicture}
\caption{%Roofline model for 
\gist when k=10}
\end{subfigure}


==> vldb26-revision/figures/roofline/roofline_both.tex <==
\begin{figure}[t]
    \centering
    \ref{rooflineLegend}
    \input{figures/roofline/deep_roofline}\hfill
    \input{figures/roofline/gist_roofline}
    \caption{Roofline analysis of the \deep and \gist search kernels for \sysname, \sysnameRQ, and \cagra. Y-axis is on log-scale, higher is better.}
    \label{fig::roofline}
    \vspace{-1.5em}
\end{figure}


==> vldb26-revision/figures/tables/construction.tex <==
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c c c c|c|} 
 \toprule
 \multirow{2}{*}{Dataset} & \multirow{2}{*}{\sysname} & \multirow{2}{*}{\cagra} & \multirow{2}{*}{\parlayann} & \multirow{2}{*}{\ganns} & \sysname Speedup \\
 & & & & & over \cagra \\
 \midrule
 \bigann & \textbf{327.7} & 1323.3 & 1418.2 & - & 4.04$\times$ \\
 \deep & \textbf{296.2} & 825.6 & 4336.9 & - & 2.79$\times$ \\
 \gist & \textbf{12.2} & 14.1 & 210.6 & 151.9 & 1.16$\times$ \\
 \openai & \textbf{89.0} & 127.8 & 1379.4 & 899.2 & 1.44$\times$ \\
 \textToImage & \textbf{24.3}& 619.2 & 184.0 & 1017.4 & 25.48$\times$ \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{Index construction time in seconds for various ANNS indexes. \parlayann is constructed on CPU. \ganns could not finish construction on \bigann and \deep 100M datasets.}
\label{tab::construction}
\end{table}


% \setlength{\tabcolsep}{3.5pt}
% \begin{table}
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c c c c c|} 
%  \toprule
%  Index & \bigann & \deep & \gist & \openai & \textToImage \\  
%  \midrule
%  \sysname & 679.8 & 785.0 & 14.8 & 120.1 & 88.7 \\
%  \cagra & 1323.3 & 825.6 & 14.1 & 127.8 & 619.2  \\
%  \parlayann & 2797.5 & 7818.3 & 450.7 & 4043.1 & 433.6 \\
%  \ganns & - & - & 151.9 & 899.2 & 1017.4\\
%  \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{Index construction time in seconds for various ANNS indexes. \parlayann is constructred on CPU. \ganns could not finish construction on \bigann and \deep 100M datasets.}
% \label{tab::construction}
% \end{table}


==> vldb26-revision/figures/tables/memory_breakdown.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c c c|c|}
 \toprule
 Component & \sysname & \cagra (NN-Descent) & \cagra (IVF) & Notes \\
 \midrule
 Raw vectors                & 38.5\,GB & 38.5\,GB & 38.5\,GB & Same input \\
 Graph index                & 25.6\,GB & 25.6\,GB & 25.6\,GB & R=64 \\
 Construction workspace     &  8.0\,GB & $\approx$\,90\,GB & 8.0\,GB & PRELIM --- pending collaborator confirm \\
 \midrule
 \textbf{Peak device memory}& \textbf{72.1\,GB} & $\approx$\,150\,GB & 72.1\,GB & A100 has 80\,GB; H200 has 140\,GB \\
 Fits on A100 (80\,GB)?     & yes      & no  & yes  & \\
 Fits on H200 (140\,GB)?    & yes      & no  & yes  & at 200M points \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{Construction memory footprint at \deep 100M. \sysname keeps the full
construction pipeline inside device memory; \cagra's NN-Descent pass exceeds
the device budget and falls back to its IVF construction path, sacrificing
graph quality. \emph{Numbers marked PRELIM are pending collaborator
confirmation.}}
\label{tab::memory_breakdown}
\end{table*}


==> vldb26-revision/figures/tables/reordering.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{| c | r r r r | r |} 
 \toprule
 Dataset & Jasper & Jasper (R) & Jasper Host & Jasper Host (R) & Vector Size (bytes)\\  
 \midrule
 \bigann & 1,492,730 & 1,427,520 & 14,098 & 17,212 & 128 \\
 \deep & 1,185,880 & 1,149,740 & 7,781 & 7,161 & 384 \\
 \gist & 96,881 & 96,741 & 864 & 800 & 3,840\\
 \openai & 62,883 & 69,413 & 421 & 416 & 6,144 \\
 \textToImage & 473,087 & 472,540 & 3,561 & 3,708 & 800 \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{Query throughput for the original vs reordered graph when beam width = 64 and K=50. Results presented are Kiloqueries per second.}
\label{tab::reordering}
\end{table}


==> vldb26-revision/figures/tile_size.tex <==
\begin{figure}[t]
    \centering
    \ref{tileSizeLegend}
    \input{figures/tile_size_bigann}\hfill
    \input{figures/tile_size_gist}
    \caption{Varying Tile size for \bigann and \gist. Throughput is in millions of queries per second, higher is better.}
    \label{fig::tile_size}
\end{figure}

==> vldb26-revision/implementation.tex <==
\section{\sysname: A GPU native ANNS system}
\label{subsec:gpu-optimizations}


\RFourInline{W1}{\sysname's design targets four GPU characteristics to achieve
  high performance. The
  central challenge in GPU-based ANNS is sustaining high hardware (compute and
  memory) utilization for an irregular, data-dependent, and memory-intensive
  workload. Existing systems trade off compute efficiency for memory bandwidth,
  or vice versa. \sysname achieves both simultaneously by re-architecting
  greedy beam search and its associated data structures around GPU execution
  constraints. The four characteristics addressed by \sysname are: }

  \begin{itemize}
    \item \RFourInline{W1}{\emph{Shared memory:} per-query state (frontier,
      candidate buffer, distances) lives in shared memory, and \sysname
      aggressively optimizes to reduce shared memory usage and increase occupancy. The
      removal of the visited hash table employed in \parlayann and \cagra helps more queries
      fit per SM.}
    \item \RFourInline{W1}{\emph{Warp divergence:} the irregular phases of beam
      search are confined to a single warp to minimize control-flow divergence.}
    \item \RFourInline{W1}{\emph{Register pressure:} distance computation is
      tiled into 16-byte chunks (\Cref{fig::load_comparison}), bounding the
      per-thread accumulator state to the register budget needed for peak
      occupancy at 32 threads/block.}
    \item \RFourInline{W1}{\emph{Memory access pattern:} our GPU \RQ implementation
      uses sequential global-memory loads, avoiding the random
      codebook lookups and read amplification incurred by PQ
      (\Cref{sec::quant}). For high-dimensional datasets, we
      widen the block to trade memory-level parallelism for per-query compute.}
  \end{itemize}

% TODO[app:gpu-chars]: Once Nsight Compute counters are collected, restore
% the extended GPU-characteristic appendix and add a forward reference here.


% We first describe how we navigate and overcome the trade-off between compute
% and memory utilization, new GPU-native optimizations to the \parlayann design,
% GPU kernel design in \sysname, and how we design batch-parallel construction. 

 % - approximately 80\% on our target hardware—which is essential for fully
 %   exploiting GPU parallelism in ANN workloads.
 % \prashant{This claim needs to be updated.}

% \para{Background} \zikun{We can delete this paragraph, duplicated
% information.} Our starting point is the DiskANN algorithm, originally
% designed for CPU execution. DiskANN performs a beam search starting from the
% graph medoid, maintaining a frontier of the $K$ closest candidates to the
% query. In each iteration, the closest unvisited node is expanded, its
% neighbors are evaluated, and the frontier is updated and pruned to size $K$.
% Search terminates once all candidates in the frontier have been visited.
% During index construction, DiskANN runs beam search for each inserted vector
% and adds both forward and reverse edges between the new vector and the
% visited nodes. To bound graph degree, a pruning procedure
% (\texttt{RobustPrune}) is invoked when necessary.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/graphs/jasper_query_sync.pdf}
    \caption{ANNS query pipeline in \sysname.}
    \label{fig:query-gpu}
\end{figure}


\subsection{Block-per-query execution model}

A central design decision in \sysname is to assign one CUDA thread block to
each query or inserted vector. This block-per-query model allows threads to
cooperatively execute search while keeping all per-query state (frontier,
candidates, distances) in shared memory, reducing global memory traffic and
enabling data reuse. Computing distances between vectors is embarrassingly
parallel and occupies the full block, while irregular phases such as candidate
expansion and graph traversal are partially serialized to reduce control-flow
divergence.

The full query pipeline can be seen in \Cref{fig:query-gpu}. 
The size of the thread block controls a trade-off between per-query compute
throughput and the number of memory requests issued. Larger blocks increase
arithmetic throughput, instruction-level parallelism, and shared-memory
capacity per query, while smaller blocks allow more concurrent queries in each
SM (streaming multiprocessor), allowing for higher memory utilization. The
optimal trade-off choice depends on the compute and memory balance of the
distance kernel. For low-dimensional datasets such as \bigann, where
performance is memory-bound, smaller blocks maximize throughput. For
high-dimensional datasets such as \gist, where distance computation dominates
(17.6$\times$ higher cost than \bigann), larger blocks that maximize per-query
parallelism achieve higher throughput. \RTwoInline{D3}{Block size is chosen as
32 for vectors with up to 128 dimensions, and as 64 threads per block for all
larger vectors. For the small vectors, we additionally double the block size at
beam widths of 512 and above as it provides a 38\% performance boost for these
large beam widths.} In summary, \emph{smaller vectors favor
higher query concurrency; larger vectors require greater per-query compute
resources.} 
% \RTwoInline{D3}{TODO: State explicitly that block size is chosen
% per-dataset (a function of vector dimension), not fixed across all
% configurations. Reviewer asked whether this is implemented or hypothetical.}


% \prashant{This paragraph is too long.} \zikun{This paragraph can be deleted.
% It is talking about the same thing as two previous paragraphs.} In our
% experiments on the NVIDIA A40 GPU, we do not use a single block size across
% all phases of the algorithm, but instead tailor the block size to the
% computational characteristics of each kernel. For beam search on
% low-dimensional datasets such as \bigann (128-byte vectors), we use a block
% size of 64 threads, as distance computation is inexpensive relative to global
% memory latency and smaller blocks increase memory-level parallelism (MLP) by
% allowing more concurrent queries per SM, improving latency hiding. For beam
% search on high-dimensional datasets such as \gist, we increase the block size
% to 128 threads to provide greater per-query parallelism, which improves
% arithmetic throughput, register reuse, and instruction-level parallelism in
% this compute-bound regime while maintaining sufficient occupancy. Finally,
% for the \texttt{RobustPrune} kernel, which is dominated by large batches of
% distance computations over candidate edge lists, we use a block size of 512
% threads to maximize per-task compute throughput and efficiently exploit
% shared memory. These choices reflect a deliberate trade-off between per-query
% compute parallelism and MLP, allowing \sysname to achieve high utilization
% across both memory-bound and compute-bound phases without enforcing a single,
% suboptimal execution configuration.

\subsection{Divergence from \parlayann construction} \label{subsec:divergence}

Our version of \search diverges from \parlayann's \search due to the
difference between CPU and GPU parallelism. We are limited by the computing
model and resources when running \search on GPU. 
% This section discusses the trade-offs we employ for GPUs. 
The \search algorithm in \parlayann is serial for each query, as there are many
more queries than CPU threads. On the GPU, we have an order of magnitude more
threads. To fully saturate the GPU compute and achieve high performance, we must
parallelize the internal components of \search. 
% This leads to divergent behavior from the original \parlayann algorithm,
% which we discuss below.

% Mapping the \parlayann construction algorithm to GPUs requires fundamental
% changes due to differences in the parallel execution model. On CPUs,
% \parlayann assigns a single thread per task, relying on a relatively small
% number of hardware threads to process large batches of work. For example,
% even our smallest dataset contains 10M vectors, yielding batch sizes on the
% order of 200K vectors processed by at most $\sim$1K CPU threads. This
% imbalance allows efficient single-thread-per-task execution with limited
% divergence.

% GPUs, by contrast, expose orders of magnitude more parallelism, with over
% 100K threads potentially active concurrently. In this regime, assigning one
% thread per task leads to poor load balance and underutilization, particularly
% for the irregular control flow of graph-based ANN construction. Moreover,
% individual GPU threads are significantly weaker than CPU cores, making such
% fine-grained tasks inefficient. We therefore assign multiple threads to
% cooperatively process each vector, which substantially improves beam search
% efficiency and query throughput, at the cost of increased divergence and
% shared-memory pressure.

% \RTwoInline{D4/D5}{State unambiguously that the hash
% table is REMOVED in all \sysname configurations (not optional / not toggled
% per dataset). Then in pseudocode (Alg. 2 + Alg. 3 merge step), show the
% replacement check explicitly.}
\para{Different hash table choices} A major source of divergence arises from
\parlayann’s use of a lossy hash table during beam search. The original
algorithm employs a fixed-size (512-slot) hash table with direct replacement to
track previously visited vertices and prune duplicates. On CPUs, this structure
is accessed sequentially within a single thread, yielding deterministic
behavior. On GPUs, preserving this access pattern would require serializing
hash table operations across cooperating threads, severely limiting throughput.
Parallelizing these operations improves performance but introduces
non-determinism. We find that this hash table does not
significantly affect accuracy or search throughput on the GPU,
\RTwoInline{D4}{and remove the hash table in all \sysname configurations,
instead opting to use a visited bit for each item in the frontier.}
\RTwoInline{D5}{Removing the
hash table reduces shared memory pressure and allows \sysname to
schedule more queries per block, as shared memory is the limiting occupancy
factor when running with 32 threads per block.}

\para{Different merge order} \sysname employs a different candidate merge order
during beam search. \parlayann implements a deferred-merge optimization, which
postpones sorting and merging when candidate lists are smaller than a fixed
fraction of the beam width. The size of the candidate set depends on the
results of the hash table lookup: with non-deterministic hash tables, we cannot
guarantee this mechanism produces the same candidate list order each time.
Empirically, we find that removing the hash table and deferred merging
materially affects neither index quality or query accuracy. Consequently,
\sysname removes both features. This simplifies control flow, preserves
determinism, and eliminates a major source of thread divergence.

% \para{Limited shared memory on GPU} Finally, divergence is further amplified by
% shared memory constraints. Cooperative execution requires per-query shared data
% structures, which limits occupancy and reduces the GPU’s ability to hide memory
% latency. We deliberately accept this trade-off: tighter shared-memory budgets
% and higher intra-warp divergence enable greater locality and reuse, which are
% critical for irregular ANNS workloads. As shown in our roofline analysis
% in~\Cref{eval:roofline}, this design remains competitive and when combined with
% query reordering in \sysnameRQ, can significantly increase operational
% intensity.
% \hunter{I don't understand what this paragraph is trying to say.}
% \hunter{I don't like the end of this paragraph - need a punchier takeaway}

\subsection{Diverging from \parlayann's search}
\RTwoInline{W1}{\sysname inherits the two-phase batch-parallel structure above
  but tunes the inner \search and the batch-pruning prologue for GPU execution.
\Cref{alg:jasperbeam} shows \sysname's \search; it can be read against
\Cref{alg:beamsearch} to see the changes directly. The visited-tracking hash
table that \parlayann uses to filter neighbors at gather time is removed
entirely: each frontier entry instead carries a visited flag, gather pulls in
\emph{all} neighbors of $u$ without filtering, and any already-visited
duplicates are absorbed by the subsequent sort. This trades a small number of
recomputed distances for $\sim$512 bytes of shared memory per query (the
fixed-size hash table in \parlayann), which raises the number of concurrent
queries per SM. \parlayann's deferred-merge optimization is also removed:
every round, \sysname \emph{gathers}, \emph{computes distances} in parallel
across the block's tiles, \emph{sorts and merges} into $F$, and \emph{prunes}
$F$ back to $K$.
A third change touches the batch pruning prologue (\apxref{alg:parlayann}{Appendix~A},
Step 3): the per-batch \textsc{Semisort} is replaced by a full Thrust
\textsc{Sort} keyed on \emph{(target vertex, distance)}, which both groups edges
per vertex and pre-orders each group for \prune. This single sort yields
better load balance on the GPU than a semisort followed by per-vertex thread
sorts.
}
% The rationale and empirical justification for each replacement are discussed
% alongside the kernel design in~\Cref{subsec:divergence}.}

\subsection{Vector load optimization}

\begin{figure}[!t]
    \centering
    % \includegraphics[width=\linewidth]{figures/graphs/tiled_vs_chunked.pdf}
    \includegraphics[width=\linewidth]{figures/graphs/tiled_vs_chunked_graph_only.pdf}
    \caption{Comparison of the two different load strategies tested in
    \sysname: tiled loads load one object per thread in the tile at a time,
  whereas the chunked load strategy loads a fixed amount of data (16 bytes) per
thread and has each thread work on all objects loaded in that chunk.}
    \label{fig::load_comparison}
    \vspace{-0.5em}
\end{figure}
Efficient distance computation is limited not only by arithmetic throughput but
also by the memory load latency. By default, when a warp accesses
a large object, the compiler emits a sequence of 16-byte loads issued by a
single thread, which limits latency hiding. Element-wise loads distribute
requests across threads but reduce effective bandwidth, as each element is no
more than 4 bytes large.

We adopt a \emph{chunked loading scheme} that partitions each vector into 16-byte
segments and assigns one segment to each thread. Threads load query and
candidate chunks in parallel, compute partial distances locally, and iterate
until the full vector is processed. A block-wide reduction then produces the
final distance. This approach issues many coalesced 16-byte loads
simultaneously to achieve near-peak memory bandwidth.

\Cref{fig::load_comparison} shows the difference between tiled and chunked loading. Chunked loading improves performance for
latency-sensitive workloads: for small beam widths, where search is memory
latency bound, it yields up to a 14\% speedup. For large beam widths, where
compute throughput dominates, optimized loads match baseline performance
without loss.

% In
% ~\Cref{subsec::rabitq}, we explains in detail how RaBitQ works along side with
% optimized loads.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/graphs/jasper_batch_construct.pdf}
    \caption{Batch graph construction pipeline in \sysname.}
    \label{fig:batch-construction}
\end{figure}

\subsection{Batch construction on GPUs}

% \RThreeInline{W3}{Clarify here that batches are not a
% limitation of the algorithm but a consequence of GPU launch model: per-vector
% insertion is supported but batching is required to saturate the device. Also
% note inserts and queries cannot run concurrently (already in R2-D1 margin).}
To support high-throughput index construction, \sysname adopts the bulk
construction algorithm \RThreeInline{W3}{as this matches the structure of the original algorithm and is highly amenable to the GPU launch model}. \parlayann relies on fork--join parallelism (via
ParlayLib~\cite{Blelloch2020}) and a semisort to group edges before insertion,
enabling lock-free parallel updates. Fork--join dynamically decomposes large
tasks (e.g., sorting and grouping edges) into smaller subtasks that are
scheduled across CPU threads.

\parlayann's execution model does not map directly to GPUs: kernel launches
require a fixed thread configuration, dynamic task spawning is not supported
within a kernel, and excessive kernel launches incur substantial overhead. We
therefore fuse \emph{search}, \emph{grouping}, and \emph{pruning} into a small
number of self-contained GPU kernels with fixed parallel structure. 
This fused pipeline is illustrated in~\Cref{fig:batch-construction}.
Although this removes some scheduling flexibility, it preserves the scalability of batch-parallel
search and pruning while conforming to the GPU execution model and
minimizing launch overhead.
\RTwoInline{W3,D1}{We employ the batch-parallel design and fuse the build steps
into a fixed kernel pipeline to achieve high performance. Therefore,
insertions and queries are run in phases: a batch of inserts must complete
before queries resume, and vice versa. Inserts are still incremental in the
sense that each batch extends a live index without rebuilding it.} 

% \hunter{Could mention we could stage a buffer similar to NEOS to allow for true incremental?}

\para{GPU-efficient pruning}
We implement a hybrid pruning strategy for \prune. Outgoing edges produced by
beam search are accumulated together with existing edges that require pruning
and are stored in a unified buffer. This buffer is fully sorted by vertex ID and
distance using the CUDA Thrust library. While \parlayann performs a
semisort followed by per-vertex distance sorting using a single thread, we find that on
GPUs a full parallel sort provides better load balance. as individual threads
are relatively weak and uneven work distribution is costly.

After sorting, each vertex’s edge list is pruned by assigning an entire SM
(1024 threads) to the operation. \prune is dominated by distance
computations and therefore benefits from high intra-vertex parallelism.

\subsection{Deletion}

\RThreeInline{W2}{Along with batch insertions, \sysname implements batch deletions using the algorithm from FreshDiskANN~\cite{Singh2021}. In this algorithm, vertices are first logically marked as deleted. This is a lightweight, in-place operation that prevents vertices from appearing in the output but does not remove them from the graph. A bulk remove operation \texttt{compact} is then called once a large percentage of the graph has been deleted (10\%). This culls nodes from the graph without sacrificing recall by using a bulk prune strategy: each vertex that pointed to a deleted vertex is pointed to every directed neighbor of that vertex, and robust prune is called to ensure only high-quality neighbors are kept. This preserves recall and allows the vertex to be entirely removed from the graph. Performance of these phases can be seen in \Cref{subsec::deletion}.}

\subsection{Scalability with batch size for updates}

% \setlength{\tabcolsep}{2pt}
% \begin{table}
% \begin{center}
% \begin{tabular}{|c|c|c|c|} 
%  \toprule
%  Dataset & Index Size & Construct Budget & Batch Size \\  
%  \midrule
%  \bigann 100M & $38.5GB$ & $41.5GB$ & 1M\\ 
%  \deep 100M & $64.1GB$ & $15.9GB$ & 400K\\
%  \bottomrule
% \end{tabular}
% \end{center}
% \caption{Batch size to achieve maximum throughput during updates in \sysname. \zikun{We can get rid of this table}}
% \label{fig::construct_config}
% \end{table}

% \RTwoInline{W2}{TODO: Insert memory-usage strength paragraph here:
% \sysname stays within device memory at 100M scale where CAGRA NN-Descent
% overflows and falls back to IVF. Forward-ref \Cref{app:memory} for the full
% breakdown and \Cref{app:h200} for 200M results.}
Index construction in \sysname is performed entirely on the GPU:
\RTwoInline{W2}{both the dataset vectors and the evolving graph reside in
device memory}, eliminating PCIe transfers and using the remaining memory as
workspace for batch processing. The achievable batch size is therefore
constrained by the available device memory after storing the index and directly
determines the degree of parallelism and throughput of the construction
pipeline.

On an NVIDIA A100 with 80 GB of memory, the BigANN-100M dataset and its graph
occupy 38.5 GB, leaving 41.5 GB for construction buffers; this supports an
optimal batch size of approximately 1M vectors. 

% For Deep-100M, the index
% occupies 64.1 GB, leaving 15.9 GB of workspace and an optimal batch size of
% approximately 400K vectors. These batch sizes maximize construction throughput
% by fully utilizing available device memory while keeping all computation and
% data movement on the GPU.

\RTwoInline{W2}{
 For Deep 100M datset, during Jasper construction we spend 38.5GB to store the
 raw vectors, 25.6GB to store the graph index, and an additional 8GB for the
 construction workspace. In total, \sysname uses 72GB of device memory during
 construction, which is very close to the 80GB limit by Nvidia A100 GPU. In
 contrast, \cagra's NN-descent construction requires around 150GB of device
 memory for the same dataset, almost double the available memory. In our
 experiments, \cagra failed to allocate sufficient memory for NN-descent and had
 to fall back to the IVF method to build the index trading off construction
 performance and accuracy.
}

\RTwoInline{W2}{
 Overall, \sysname's construction method scales better compared to NN-descent
 when the GPU memory is the bottleneck for large datasets. We calculate the
 full memory usage breakdown in \apxref{app:memory}{Appendix~D}. We also shown in
 \apxref{app:h200}{Appendix~C.2} we can support 200M vector dataset using GPU with larger
 memory.
}

% \subsection{Optimizing Loads}
% \label{subsec:opt-loads}
% \subsection{Optimizing Block Size}

% Block size introduces a fundamental trade-off between per-query compute throughput and memory-level parallelism (MLP). Larger blocks assign more threads to each query, improving arithmetic throughput and register reuse. Smaller blocks allow more queries to execute concurrently, increasing outstanding memory requests and improving latency hiding.

% For low-dimensional datasets, memory latency dominates. In this regime, reduced per-query parallelism has minimal impact, while increased MLP yields higher throughput. Conversely, for high-dimensional datasets such as GIST, distance computation dominates: we measure a 17.6$\times$ higher compute cost relative to memory operations. In this compute-bound regime, reducing block size directly degrades performance by limiting per-query compute resources. Thus, the optimal block size is dataset-dependent and closely tied to the compute–memory balance of the distance kernel.

% \subsection{Optimizing Distance Calculations}




% In this section, we describe the GPU-specific optimizations required to efficiently execute the Vamana algorithm on modern GPU hardware. The core challenge is to balance computational throughput and memory bandwidth in order to maximize performance. Our approach carefully redesigns the beam search algorithm and associated data structures so that the GPU kernels achieve approximately 80\% simultaneous utilization of both compute units and memory bandwidth. This high level of utilization is essential for fully exploiting the parallelism of GPUs when executing the complex search operations required by approximate nearest neighbor (ANN) algorithms.

% Our starting point is the original DiskANN algorithm, which is designed for CPU execution. The pseudocode for beam search can be seen in \cref{alg:beamsearch}. The baseline algorithm performs a beam search beginning at the medoid of the graph, and maintains a list of the $K$ closest vectors to the query. In each iteration, the neighbors of the closest unvisited vector are loaded. Their distances to the query vector are calculated and they are merged into the frontier and sorted by distance. If the size of the frontier exceeds K, the furthest vectors are discarded. This continues until all nodes all vectors in the frontier have been visited. 

% To add a vector to the graph, DiskANN runs the beam search on that node before adding two sets of edges, one set running from the visited nodes to the new vector, and a reverse set running from the new vector to the visited nodes. To keep the degree of the graph small, DiskANN runs a procedure called RobustPrune whenever the degree of a vertex is too high.

% To make the construction algorithm more suitable for GPU execution, we use the bulk construction from \parlayann~\cite{Manohar2024}, a parallel ANN framework originally designed for multi-core CPUs. \parlayann uses parlayLib~\cite{Blelloch2020}, a library for efficient CPU fork-join parallelism. \parlayann utilizes the beam search from the original paper but implements the pruning phase using a batch-parallel algorithm. In this algorithm, the new edges are \textbf{semisorted} to efficiently group them. This allows for edge insertions to be performed in parallel without the use of locks, significantly improving the scalability of construction. We adapted this batch parallel construction for use in CUDA. As there does not exist an efficient way to implement fork-join parallelism in CUDA, we adapt the batch construction as one self-contained kernel.


% A key decision in our design is to assign a full cooperative thread array (CTA) to each query. Our kernel needs to be able to handle the maximum fanout for each vector. To do this efficiently, we directly control the number of threads working on each step of the beam search to maintain maximum throughout, with certain steps executed in parallel across the batch and others performed sequentially within each query. This redesign is a critical step in making the algorithm GPU-friendly.


% % Fork-join parallelism presents unique challenges on GPUs because thread creation is not dynamic within a single kernel. Unlike on CPUs, where threads can be spawned and synchronized on demand, GPU kernels must pre-allocate a fixed number of threads. To address this limitation, we allocate the maximum span of threads required in advance and reuse them throughout the computation. This approach allows us to approximate the flexibility of fork-join parallelism while conforming to the GPU execution model. By carefully tuning the problem parameters and thread layout, we are able to achieve a structure that behaves similarly to fork-join execution in practice.

% Distance computations, such as distance computation between the query and a set of candidate vectors, are embarrassingly parallel and can be mapped efficiently across all threads in a block. By dedicating an entire CTA to a single query, we ensure that all threads are utilized during these phases, maximizing throughput. This approach also simplifies the implementation by isolating per-query state to a single block, which allows for the major data structures to be stored in shared memory. For the NVIDIA A40 GPU used in our experiments, the block size was chosen as 512 to fully occupy the available hardware resources, though the exact size may vary depending on the target architecture.

% Within each CTA, we must ensure that every stage of the beam search is optimized for GPU execution. The beam search consists of three main phases. The first phase is distance computation, where tiles of vector data are loaded into shared memory and distances are computed in parallel. The second phase is candidate sorting, which we implement using CUB's full thread block sorting primitives to achieve high performance. The third phase is edge expansion, where the neighbors of each candidate are retrieved and evaluated. For this final phase, we use a single warp to process edges, minimizing control flow divergence and improving efficiency.

% We utilize a hybrid approach to perform the robustPrune efficiently. The outgoing edges from the beamSearch are accumulated into a thrust vector, along with existing edges from nodes that need to have robustPrune run. This vector is then fully sorted on both node ID and distance to the query vector. Using a thrust sort allows us to not only group the edges as is done in the \parlayann semisort, but it also locally reorders the new edges into the correct order for comparison in the prune. Due to the relatively low throughput of individual threads in the GPU, performing a full sort instead of a semisort allows for more even work distribution and thus higher throughput than performing the sort locally with one CTA. The prune kernel assigns an entire CTA to each edge list being modified, as this phase is dominated by distance computations.



% % \subsection{Optimizing for GDDR}
% % In ANNS, memory bandwidth is the dominant performance bottleneck in our GPU implementation, as each dimension in a loaded vector is used only once before being discarded. To maximize memory throughput, we focus on two complementary strategies: reducing the total volume of data loaded from memory, and improving the speed at which the necessary data is transferred.

% \input{figures/loads/loads}
% % \input{figures/loads/load_tiled}
% % \input{figures/loads/load_coalesced}

% \subsection{Algorithm Divergence}

% Efficiently mapping the construction algorithm from ParlayANN to GPUs requires several algorithmic changes, the most significant of which stems from differences in the parallel execution model. ParlayANN targets CPUs, where parallelism is limited by a relatively small number of hardware threads compared to the amount of work per batch. In our setting, even the smallest dataset contains 10M vectors, yielding batch sizes on the order of 200K vectors that are processed by at most ~1K CPU threads. This imbalance allows ParlayANN to assign a single thread per task without incurring significant load imbalance or control-flow inefficiency.

% GPUs, by contrast, support orders of magnitude more parallelism, with over 100K active threads potentially executing concurrently. Under this regime, a one-thread-per-task mapping leads to poor work distribution and underutilization, particularly given the irregular and data-dependent nature of graph-based ANN construction. Moreover, individual GPU threads are substantially weaker than CPU cores, making per-thread workloads too fine-grained to efficiently hide memory latency. Empirically, we find that assigning multiple GPU threads to cooperatively process a single vector—rather than mapping vectors to individual threads—substantially improves beam search efficiency and overall query performance. This cooperative strategy better matches GPU hardware characteristics, albeit at the cost of increased divergence and shared-memory pressure, which we explicitly manage in \sysname and \sysnameRQ.

% Assigning multiple GPU threads to each inserted vector introduces additional sources of divergence relative to the CPU-oriented design of ParlayANN, most notably around its use of a lossy hash table during beam search. ParlayANN employs a fixed-size (512-slot) hash table with direct replacement to track previously visited vectors and prune duplicate candidates during expansion. Because ParlayANN executes one beam search per CPU thread, hash table queries and updates occur sequentially, yielding deterministic behavior and well-defined pruning semantics. Replicating this behavior on a GPU would require serializing hash table accesses across the threads assigned to a single vector, which would substantially limit throughput and negate the benefits of cooperative parallelism.

% While the hash table is not required for correctness of either construction or query, it is used in ParlayANN to enforce specific pruning decisions that influence whether candidate lists are merged in the current round or deferred. This interaction is further complicated by ParlayANN’s batching mechanism, which allows the sort and merge of the candidates to be deferred when the current candidate lists is smaller than a set fraction of the beam width (< beamwidth / 8). Parallelizing hash table operations across threads improves performance but introduces nondeterminism, which in turn interacts poorly with deferred merging. In our experiments, we find that neither the lossy hash table nor delayed merging materially affects index quality or query accuracy. Consequently, to maximize GPU throughput while preserving deterministic behavior, \sysname removes these features from beam search, simplifying control flow and avoiding a major source of divergence without sacrificing empirical performance.

% % Issuing multiple threads per inserted vector leads to some divergence issues with \parlay, mainly surrounding the lossy hash table. In beamSearch, \parlay uses a 512 slot hash table with direct replacement to manage previously seen vectors. This hash table is used during candidate selection to filter out previously seen candidates. As \parlay issues one thread for each beam search, the hash table is queried and updated sequentially. To match the behavior of \parlay, \sysname would have to query this table sequentially as well, which would significantly limit the throughput of this checking phase.

% % The hash table is not necessary for construction and query correctness, but it is required to match the \parlay construction algorithm exactly, as the hash table prunes candidates which determines if the current set of candidates will be merged in this round or deferred. Processing operations in the hash table in parallel provides a speedup but makes this algorithm nondeterministic.

% % \begin{itemize}
% %     \item there is also batching - parlayANN allows candidate lists with a small number of candidates (< beamwidth/8) to be deferred to the next round
% %     \item this presents an issue with the hash table as our parallel operations are nondeterministic.
% %     \item We find that the hash table + delayed merge don't affect accuracy.
% %     \item Therefore, in order to maximize performance and maintain deterministic behavior, we clip this features from the beamsearch in \sysname.
% % \end{itemize}

% Our divergence from the original \parlay construction algorithm is further amplified by shared memory pressure, which is a fundamental constraint on GPUs but largely absent in the original ParlayANN setting. Cooperative thread groups require shared data structures (e.g., candidate lists, visited sets, intermediate distances), increasing shared memory usage per task and limiting occupancy. Lower occupancy reduces the GPU’s ability to hide memory latency, making divergence more visible in performance. Nevertheless, this design reflects a deliberate trade-off: by tolerating higher intra-warp divergence and tighter shared memory budgets, \sysname and \sysnameRQ gain improved locality and reuse across threads, which is essential for irregular ANNS workloads. The roofline results show that, despite these divergence costs, the approach remains competitive and—when combined with query reordering in \sysnameRQ—can shift execution toward higher operational intensity, partially offsetting the control-flow inefficiencies inherent to GPU-based graph search.

% \subsection{Optimizing loads}
% \label{subsec:opt-loads}

% While quantization can cut down on the amount of memory transferred, we must also look at optimizing how data is loaded in order to achieve maximum performance.

% % \subsubsection{Graph reordering}
% % Our first improvement tested is a novel graph reordering technique. By reordering the nodes of the graph so that vectors which are close in the metric space are stored adjacent to each other in memory, we increase the likelihood that memory accesses will be sequential. In theory, sequential accesses are more efficient on modern GPUs, as they reduce cache misses and enable coalesced global memory operations. This reordering step can therefore improve the overall throughput of the distance computation phase. 

% % In practice, we find that graph reordering is not helpful for graphs which are stored entirely in GPU memory. For the main vectors, graph reordering is between 5\% slower to 11\% faster, with the majority of datasets showing no improvement or negative performance. However, when we scale out of device memory into host graph reording shows significant improvements, with performance increasing by XX\%\hunter{How much?}. The increased performance on host is due to the coalescing of PCIE transfers: two or more adjacent vectors can be grouped together, reducing the overhead of the transfer and increasing the PCIE throughput.

% We carefully optimize the loads themselves to maximize throughput. By default, when a warp accesses a large object, the NVIDIA compiler issues the load of the object as a series of 16-byte loads issued by one thread in the warp. This maximizes memory bandwidth for that thread but introduces additional latency as one thread issues all requests. If the object is accessed directly as an array, the compiler instead issues element-wise loads across the warp, with each thread in the warp loading exactly one element at a time. This results in a larger number of smaller requests, reducing effective bandwidth. To avoid this problem, we partition each vector into 16-byte chunks. Each thread is responsible for loading one chunk from both the query vector and the candidate vector in parallel. The thread computes a partial distance for all elements in the chunk locally, and this process repeats until the entire vector is processed. After all chunks are processed, a reduction across threads produces the final distance value. This scheme ensures that multiple 16-byte loads are issued simultaneously at the maximum stride, achieving near-peak memory throughput. 

% \input{figures/construction/load_comparison}

% This approach improves the latency of loads without sacrificing throughput. The benefit of this approach can be seen in \Cref{fig::load_comparison}. When the beam width is small, the search operation is latency bound as there are not enough loads to properly latency hide. This results in a 14\% boost to the query speed as all loads are issued simultaneously. However, when the beam width is large, there is enough work to properly hide latency, and throughput dominates. In this scenario, the optimized loads have the same throughput as other load strategies - no throughput is lost;

% Our optimized loading scheme applies equally to both original floating-point vectors and quantized vectors produced by RaBitQ. When combined with RaBitQ’s compression, this approach yields substantial gains. RaBitQ reduces the total data transferred by up to 50\% in the worst case, and the optimized loading pattern improves the speed of these transfers. Combining it with RaBitQ leads to a ...\% overall increase in beam search performance compared to the unoptimized GPU baseline.

% Through the combination of RaBitQ-based compression and optimized vector loading, we achieve a highly efficient GPU implementation of DiskANN. These optimizations enable our kernels to operate near the theoretical limits of the hardware, with approximately 80\% utilization of both compute and memory resources. This balance is essential for scaling ANN search to the large datasets and high query volumes required in modern applications.

% \subsection{Optimizing block size}
% Previous work placing ANNS on GPUs suggests that using the entirety of a CTA is beneficial due to the increased parallelism and extra scratch space available in shared memory. Adding more threads improves the parallelism available to an individual query. However, reducing the block size increases the number of queries that can be processed concurrently within each CTA. This elevates the amount of memory traffic and raises memory-level parallelism (MLP), improving the ability of the GPU to hide global-memory latency.
% We find that this behavior represents a fundamental trade-off between memory parallelism and per-query compute tradeoff.  Using a smaller block size increases the number of outstanding memory loads per CTA, but it also reduces the number of threads assigned to each query. This lowers the arithmetic throughput available for computing distances, since less per-query parallelism and register reuse are available.

% For low-dimensional vectors, the memory-parallelism benefit dominates. When vector dimensions are small, the cost of the distance computation is minor relative to memory latency. In this regime, reduced per-query compute resources have little negative impact, while the increased MLP yields a net throughput gain. Consequently, processing twice as many queries per CTA outweighs the modest increase in compute time per query. This counteracts the commonly supported knowledge - for smaller vectors, small beam sizes perform much better. For \bigann, where vectors are only 128 bytes, we find that smaller beamsize is strictly beneficial up to the maximum occupancy of 32 blocks per CTA.


% For high-dimensional vectors (e.g., GIST), the compute cost dominates and reverses the trade-off. In our measurements, distance computations in \gist consume 17.6× more cycles than memory operations. Because the dot-product computation is the dominant bottleneck, reducing block size directly slows down the central operation—each query receives fewer threads, less instruction-level parallelism, and diminished register reuse. In this compute-bound regime, increased MLP provides negligible benefit, so smaller block sizes reduce overall performance.
% Thus, the optimal block size is dataset-dependent and correlates closely with the compute/memory balance of the distance kernel. Memory-bound datasets benefit from high memory parallelism; compute-bound datasets require maximal per-query compute throughput.


% \subsection{Optimizing distance calculations}
% In our testing, the square root operation took over 40\% of the walltime of the distance calculation, even after optimizing for tile sizes. As square root is monotonic over the positive reals, we elide the square root operation from Euclidean distance calculations. This improves the performance for the vast majority of distance calculations without sacrificing correctness, as all relative distances are preserved.


% % \section{Implementation}
% % In this section, we discuss the design of our algorithm and the GPU optimizations necessary to achieve high performance.

% % \input{pseudocode/parlayANN}

% % Our approach is based off of the batch parallel vamana algorithm used in \parlayann~\cite{Manohar2024}. This algorithm inserts vectors into the index in batches, using a lock-free algorithm.

% % The pseudocode for insertion can be seen in \Cref{pseudo::parlayANN}. In each iteration, a batch of new nodes are appended to the existing graph. For each node in the batch, greedySearch is executed on the main graph, and the list of updates to be applied to the main graph are generated. Instead of applying updates directly, the set of new edges for all nodes in the batch is collected in a list. This list is then organized using a \textit{semisort}, a variation of sort which groups identical keys together but does not order the keys. This groups all edges connected to a vertex together in the list. A vertex-parallel kernel is then executed to apply the edge updates. Since each vertex has a collected list of updates, they can be safely updated in parallel. Once the new edges have been added, robustPrune is executed on all nodes that were modified.

% % \subsection{Porting to GPU}
% % The main challenge when porting the algorithm to GPUs is how to properly express parallelism. In the original \parlayann implementation, parallelizing across the incoming vertices in beamSearch and robustPrune is sufficient, as there are a relatively low number of threads compared to the number of vertices. The increased number of threads on a GPU makes parallelizing across just the vertices work-inefficient, and the differing compute-memory complexity of each phase of execution means that significant speedups can be achieved through better work distribution.

% % \subsubsection{Thrust}
% % To parallelize across a batch, we use the Thrust vector library. This library provides on-device vectors which can be accessed and resized from host. In the beam search, we group the individual visited list, frontier list, and unvisited list of each vector in the batch together into one large thrust vector. This allows for the set difference and sort calls to be processed for all vectors in the batch in one call to thrust.

% % One of the main advantages of using thrust is the ability to specify the level of parallelism needed for a given function. In \parlayann, all operations are performed with a single thread, as there are a limited number of CPU threads. On the GPU, the parallelism we can express per-operation can vary drastically depending on the operation.
 
% % For example, during the beam search, many operations are memory bound - To find the next set of candidates, we must read the neighbors of every node in the live frontier. This requires no compute, so we can schedule this operation per-thread and maximize the memory throughput of the GPU. However, for the distance calculation, compute is the new bound, so we assign teams of threads to cooperatively perform the distance calculations. Finally, in robustPrune, the compute density is much higher, as each iteration must perform L different distance calculations per round of pruning. For this scenario, the ideal amount of parallelism is a thread block, as we must maximize the available parallelism when performing the per-round distance calculations.

% % \input{pseudocode/cudaBeam}

% % \subsection{Beam search}
% % In the beam search, the graph is greedily traversed to find the nearest neighbors of a target query vector Q. This search returns two vectors: a set of the nearest neighbors called the \textbf{frontier}, and a set of all nodes traversed, called \textbf{visited}.

% %  In each iteration, the closest unvisited node in the frontier is gathered, and the neighbors of that node are loaded from the graph. The distance between Q and each neighbor is calculated, and the neighbors are merged into the frontier. If the size of the frontier ever exceeds the cap $L$, the frontier is clipped to contain the $L$ best vectors.  The frontier contains a second variable, the beam width, which determines how many unvisited nodes are loaded in each iteration.

% % The pseudocode for the CUDA beam search can be seen in \Cref{pseudo::cudaBeam}. In every iteration of the beam search, we pop the first $w$ unvisited nodes in the unvisited frontier from every vertex. These form the \textbf{live frontier} whose neighbors will form the next candidate set. For every node in the live frontier, we load its neighbor list in the graph and populate the candidate vector with the new pairs {Q->neighbor}. A second kernel is launched to perform the distance calculation for all pairs in parallel. The candidates are then sorted first by Q, then by distance. This set is then merged with the current frontier. If the frontier size of any individual vector exceeds the cap $L$, that section of the frontier is clipped to conatin the $L$ best vectors. Finally, the live frontier is merged with the visited list, and the unvisited frontier is regenerated by taking the set difference between the frontier and visited lists. This process continues until all items in the frontier have been visited, and returns the frontier and visited vectors.

% % Compared to the original \parlayann implementation, the beam search is not run per-thread. Instead, the beam search is run for all vectors in a batch is run simultaneously using Thrust. The frontier, candidates, live frontier, and visited sets are all maintained as thrust vectors of edges. The frontier for all vectors is initialized simultaneously as one thrust vector, holding one copy of the medoid for each vector in the batch. To differentiate the edges in the frontier from each other, we pass the id of the query vector along with each new edge gathered. This allows for a thrust sort to group the objects by ID while also sorting each frontier by distance. For example, if the batch contained vectors 4 and 5 with a medoid of 2, we would construct a starting frontier of {4->2, 5->2}.

% % \subsubsection{Optimizing sort} An additional optimization that we apply is improving the performance of beam search is to improve over the sorts used in Thrust. In order to perform set difference and merge operations, thrust requires that both arrays be sorted.

% % To maintain the candidates efficiently, we store objects in the candidate set as a source->sink edge, which guarantees that all edges in the candidates (and therefore, the frontier) belonging to a particular vertex will be contiguous. 

% % candidates are added to the candidate set in a semisorted fashion, i.e. all candidates for a given vertex will be contiguous in the candidate set, but are not guaranteed to be sorted internally. This implies that sorting the entire frontier via one call to sort is wasteful - at most, an object will move R*width slots in the candidate vector, as the candidates for a given vertex are already in the correct position in the vector. 

% % We can therefore reduce the computational complexity of the sort and increase throughput by chunking the sort into smaller sections and running each sort independently. To perform this efficiently, we use 8 cudaStreams and submit 8 sort requests, each for 1/8th of the total vector size. This results in a [get the number]\% decrease in time required for sorting.

% % \subsection{RobustPrune} In \parlayann, robustPrune is a function that is executed serially per-thread. It cleans the neighbor list of a given node by removing unnecessary edges. RobustPrune is run when adding a new node to the graph or whenever the neighbors of a node grow too large. RobustPrune takes in the set of edges, sorts them by distance to the target node, then adds edges one at a time, discarding any edges in the rest of the list that fail a quality check. This check compares the distance between the newly-added node and remaining nodes in the list, clipping remaining nodes if a good-enough two hop route exists.

% % \subsection{GPU robustPrune} In analysis, we find that robustPrune is compute bound, with the lion's share of the execution time dedicated to distance calculations which are too expensive to calculate with one warp. Therefore, to execute robustPrune efficiently on the GPU, we run the robustPrune with one thread block per vertex. This allows us to compute the distance comparisons between every point remaining in the list simultaneously. The pseudocode for this can be seen in \cref{TODO}. In every iteration, the first live vertex is added as an outgoing edge in shared memory. Distances are then computed as parallel as possible, with a shared memory bit-array being used to calculate which nodes are dead in the sequence. 

% % \subsubsection{Distance calculation improvements} One of the most critical and most frequently-run operations in diskANN is the distance calculation between two vertices. As the sizes of the vectors increase, performing this operation serially becomes the bottleneck in all kernels.

% % To improve the performance of the distance calculations, we perform two optimizations. Firstly, we use tiles instead of individual threads to calculate distances, increasing the amount of parallelism available for distance calculations.

% % Secondly, we elide the square root operation from Eucldiean distance calculations. In our testing, the square root operation took over 40\% of the walltime of the distance calculation, even after optimizing for tile sizes. As on optimization, we remove the square root only when the distance sum before the square root is greater than one. This improves the performance for the vast majority of distance calculations without sacrificing correctness, as all relative distances are preserved.


% % \section{optimizations}

% % \begin{itemize}
% %     \item Single CTA beam search: For beam search, we use one single kernel call. Inside the kernel, each query vector is getting assigned to one thread block, with each block containing 512 threads. Inside each thread block, we can fully utilize the shared memory during querying without constant loads and stores to the device memory.
% %     \item Load optimizations: During distance calculations, the entire vector must be brought into memory to be compared and accumulated. The original implementation issued a load from the warp to bring the vector into the stack automatically. This is much more efficient than treating the vector as an array of uint8\_t to be loaded automatically, but leaves performance on the table. We now have every thread in the tile issue a 16 byte load using the \texttt{ld.vec4.uint32\_t} instruction. The individual threads then accumulate all 16 dimensions individually before accumulating the group results via \texttt{cg.reduce}. This improves performance of the beam search by ~25\% over the previous implementation.
% %     \item Hash table optimizations: The previous hash table design allowed all threads to compete for the insert of a single key, issuing 512 atomic instructions for a single insert (albeit in shared memory). As we own the entire thread block, we can have a single thread issue one non-atomic load. This improves performance ~10\% over the previous beam search. We can further improve the hash table by using multiple threads to cooperatively perform the singular insert and multiple threads per query to prevent bank conflicts.
% %     \item Tiling: We enumerate all possible tile sizes for the beam search and find the fastest tile size to be 4.
% %     \item: 
% % \end{itemize}

 
% % In order to account for all of these phases efficiently, we maintain counts of the number of objects needed in each phases, e.g. the size of the frontier, the number of objects per frontier, th

% \subsection{New Implementation}

% \subsubsection{DRAFTING LAYOUT}
% \begin{itemize}
%     \item layout - in this section, we discuss the GPU-specific optimizations necessary to efficiently run diskANN on GPUs. With our optimizations, we achieve kernels that run at 80\% of both compute and memory utilization simultaneously.
%     \item Our implementation forks from DiskANN - setup the original algorithm with beam search and prune (pseudocode?)
%     \item The algorithm is extended from \parlayann - showcase modifications to the pipeline via fork-join parallelism and batch-parallel algorithm. (add pseudocode).
%     \item Our algorithm optimizations 1: Fork join parallelism isn't possible on GPUs, but with the problem parameters set we can use the maximum span possible.
%     \item we use a full CTA per query as some phases (like distance calculations) are embarrassingly parallel. Using an entire CTA maximizes performance for distance calculation. (can we get an exact number?)
%     \item With a full CTA, we need to maximize performance in each phase of the beam search
%     \item Distance - tiles loads / dists of vectors
%     \item sort - full thread block sort using CUB
%     \item edge load - one warp.
%     \item subsection - optimizing memory loads. Memory loads dominate performance in the beam search. We group our optimizations into two categories - 1. cutting down the amount of memory loads necessary and 2. loading as quickly as possible.
%     \item RaBitQ - I need Zikun's help to write this as he understands RaBitQ better. We use 4-bit RaBitQ optimize the memory loads. This provides a 2x reduction in memory use for 8-bit vector types and a 8x memory reduction for uint32\_t and float vector types. 
%     \item RaBitQ for construction?
%     \item advantage of RaBitQ: Previous diskANN algorithms use product quantization to perform lookups. Product quantization requires a large lookup table to perform the quantized loads efficiently.
%     \item Due to bank conflicts and limited shared memory, this actually results in slowdowns on the GPU - get number from Zikun.
%     \item We need a quantization method that does not require indirection as this will *always* cause read amplifications.
%     \item ... explanation of RaBitQ here - explain the setup method and inputs required, space savings, and accuracy of metric calculations in the space. If we can add the math here for it that would be great - is there worst case error?
%     \item Using RaBitQ cuts down the amount of data loaded by 50\% in the worst case. We can also improve performance by optimizing the loads. 
%     \item The first optimization we add is a novel graph reordering that improves load throughput by placing close vectors adjacent to each other in the graph, improving the sequential access throughput.
%     \item We also improve individual load throughput by issuing all loads simultaneously at the largest stride possible.
%     \item By default, the compiler will issue 16-byte loads (the largest granularity on our A40) from one thread if the warp accesses the vector exactly. If we treat the vector as an array of elements, the loads are performed in parallel with the entire warp, but at the granularity of individual elements. This improves the speed of the load requests but adds many more requests as they are at a smaller granularity. The optimal throughput comes when load 16 bytes per thread with as many loads issued simultaneously as possible.
%     \item To achieve this, we block the vectors into 16-byte chunks. Each thread loads one chunk from both input vectors and then performs a local aggregation for all of the loaded dimensions. This occurs until the entire vector has been processed, and then all threads reduce to aggregate the final result.
%     \item Both the original vectors and PQ vectors can be loaded with this modified load scheme. This improves the performance of the beam search by 14\%.
% \end{itemize}




==> vldb26-revision/includes.tex <==
\usepackage{graphicx} % Required for inserting images
\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{algorithmic}
% \usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{svg}
% \usepackage{amssymb}

%not today satan
\usepackage[subtle]{savetrees}

%currently disabled as it causes problems with the "proof"
% definition
%\usepackage{ltexpprt}

\usepackage[textsize=tiny]{todonotes} % package for cool todonotes in the margin
\usepackage[normalem]{ulem} % package that allows text to be striked out

\usepackage{graphicx} % Required for inserting images
\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amstext}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary {shapes.geometric}
\usetikzlibrary{calc}
\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.3}
\usepackage{url}
\usepackage{xspace}
\usepackage{siunitx}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\setitemize{leftmargin=*}
\usetikzlibrary{external}
\usepackage{graphicx}
\usepackage{svg}
\usepackage{balance}
\usepackage{placeins}  % provides \FloatBarrier so appendix figures stay with their text
\usepackage{footmisc}
% \usepackage{showframe}
% \renewcommand\ShowFrameLinethickness{0.15pt}
% \renewcommand*\ShowFrameColor{\color{red}}
\usepackage[normalem]{ulem}
\usepackage{cancel}
\usepackage{array}


==> vldb26-revision/intro.tex <==
\section{Introduction}

Nearest neighbor search is a fundamental problem in machine learning and
information retrieval. The problem involves finding the $k$ closest points to a
query in a high-dimensional space. In this paradigm, complex data such as
images, documents, or user profiles are embedded as vectors in a \emph{metric
space} (such as Euclidean, Manhattan, Hamming) that enables similarity to be
measured through geometric distance. Applications span recommendation
systems~\cite{Roy2022, Singh2021}, image
retrieval~\cite{Rahman2024OptimizingDI, Belahyane2020}, anomaly
detection~\cite{Schubert2015, Okkels2024, Gu2019}, and increasingly,
retrieval-augmented generation (RAG) for large language models~\cite{Quinn2025,
Wang2024, Wang2025}, where relevant context must be retrieved from massive
corpora in real time.

Traditional indexing structures such as $k-d$ trees~\cite{Bentley1975} and quad
trees~\cite{Finkel1974} provide efficient exact nearest neighbor search in low
dimensions, but scale poorly as dimensionality increases. \iftruncate The
\emph{curse of dimensionality}~\cite{Minsky2017} causes distances between
points to concentrate, with the ratio between nearest and farthest neighbors
approaching one. This phenomenon undermines the spatial pruning heuristics
that traditional indices rely upon, causing query complexity to degrade
toward exhaustive linear scans. Modern embedding models routinely produce
vectors with hundreds to thousands of dimensions, limiting the practicality
of exact methods. \fi

Approximate nearest neighbor search (ANNS) addresses this challenge by relaxing
the exactness constraint.  \RFourInline{D1}{Instead of guaranteeing the true
nearest neighbors, ANNS returns approximate results whose accuracy can be
tuned against query cost. This trade-off makes it possible to scale
efficiently to high-dimensional datasets.} The three dominant paradigms for
ANNS are: inverted file indices (IVF)~\cite{Babenko2015, Xia2013, Sivic2003,
Jgou2011}, locality-sensitive hashing (LSH)~\cite{Indyk1998, Datar2004,
Motwani2008}, and graph-based indices~\cite{Malkov2020, Malkov2014, Dong2011,
Subramanya2019,Gollapudi2023, Manohar2024, ootomo2024, FAISS}.
\RFourInline{D1}{To improve performance further, these techniques can be
combined with vector quantization, which reduces vector size while preserving
relative distances.}

Graph-based indices achieve the best recall-throughput trade-offs among these
paradigms. Recent empirical studies have consistently demonstrated this
advantage~\cite{Subramanya2019}. Graph-based indices construct a
\emph{navigable search graph}~\cite{Malkov2014} where vertices correspond to
vectors and edges encode neighborhood relationships. Nearest neighbor queries
proceed via greedy traversal also known as \emph{beam search}: starting from a
designated entry point, the search iteratively expands the closest unvisited
vertex until convergence, maintaining a frontier of the best (top $k$)
candidates encountered.

\para{Modern applications require updatable ANNS indexes} Real-world ANNS
applications operate at massive scale and require continuous updates due to
evolving datasets. Web-scale retrieval systems index billions of vectors:
Facebook's similarity search infrastructure handles over 200 billion
embeddings~\cite{FAISS}, while Microsoft's Bing uses DiskANN to search over a
billion document vectors~\cite{adams2025distributedann}. These systems must
support both millions of queries per second and continuously index updates as
new content arrives~\cite{Singh2021}. Music streaming, product recommendation,
and RAG systems depend on scalable and updatable similarity
search~\cite{Singh2021a}.

% often implemented using approximate nearest neighbor indices that trade perfect accuracy for speed and scalability. Modern ANN indices such as HNSW provide efficient search over large embedding collections with logarithmic latency even in high dimensions\cite{Fu2019}. Real-time dynamic variants like FreshDiskANN support thousands of concurrent insertions and queries without expensive rebuilds, making them suitable for continuously growing datasets \cite{Singh2021}. Furthermore, dynamic range-filtering ANN research demonstrates how ANN indices can handle mixed streaming of data arrivals and queries, which is essential for services with high-velocity updates\cite{Peng2025}.

% Music streaming services add roughly
% 100,000 new tracks daily~\cite{Marconette_2023}, e-commerce catalogs update
% product embeddings in real time~\cite{Aslanyan2020}, and RAG systems must
% incorporate fresh documents to remain
% current~\cite{Ouyang2025}. \prashant{These
% citations are not appropriate.}

\para{The case for GPU acceleration} GPUs offer massive parallelism that
promises to accelerate ANNS to achieve high throughput and low latency. Both
index construction and search are well-suited to leverage this parallelism
because the core operations (pair-wise distance computations) are independent
and can execute concurrently across candidates. 
% Both index construction and search are dominated by distance computations,
% which can be performed in parallel across candidates. 
As dataset size and vector dimensionality grow, so does the available parallel
work that GPUs can exploit.

% Graph-based ANNS is compute-intensive and implicitly parallel, making it
% well-suited for GPU acceleration. Index construction requires computing vast
% numbers of pairwise distances and repeatedly refining graph connectivity. Query
% processing must traverse the graph and compute distances at each hop. Both
% operations scale with dataset size and vector dimensionality. Importantly,
% distance computations across candidate vectors are independent, allowing them
% to execute in parallel.
%
Furthermore, GPUs are already widely deployed in settings where ANNS is most
needed. Modern machine learning infrastructure runs on GPU clusters. Using GPUs
for ANNS allows organizations to leverage existing hardware rather than
provisioning separate CPU-based retrieval infrastructure. This co-location also
reduces data movement: embeddings generated on GPU can be indexed and queried
without costly transfers to CPU memory.

\para{Challenges in exploiting GPU parallelism for ANNS} Modern GPUs offer
thousands of execution units and memory bandwidth exceeding 2
TB/s~\cite{a100specs}, yet achieving peak performance for ANNS indexing and
queries remains difficult. We identify three key challenges in exploiting the
massive GPU parallelism. 

1) \textit{ANNS workloads need updatability.} Most current GPU indices require
a rebuild from scratch in order to process new updates. 
However, real-world applications such as anomaly detection~\cite{Gu2019} and
RAG~\cite{Quinn2025, Wang2024, Wang2025} require the ability to modify the
index to incorporate new information in search results.

2) \textit{Greedy graph traversal creates irregular memory access patterns.}
Unlike dense matrix operations where access patterns are known ahead of time,
graph search follows data-dependent paths that vary per query. When different
threads in a warp access non-contiguous memory locations, the GPU must issue
multiple memory transactions, wasting memory bandwidth. This problem is made
worse by the pointer-chasing nature of graph traversal, where each hop depends
on the previous result.

3) \emph{ANNS workloads are memory-bound rather than compute-bound.} Each
vector dimension is read once, used for a single multiply-add in the distance
computation, then discarded. With no data reuse, performance is limited by how
fast data can be fetched from memory rather than how fast arithmetic can be
performed. For a 128-dimensional float32 vector, the GPU performs 256
floating-point operations but must load 512 bytes of data, a ratio far below
what modern GPUs can sustain at peak compute utilization. In our analysis
in~\Cref{eval:roofline}, we find that the state-of-the-art ANNS search kernels
are very close to the peak memory capacity. \RFourInline{D1}{To further improve performance, we need to reduce the data transfer and avoid incurring random memory accesses. Efficient vector quantization techniques can help us achieve both targets.}

% \prashant{Not sure if this para is needed anymore. Commenting for now.}
% The control flow of graph search maps poorly to the GPU execution model. Beam
% search requires maintaining priority queues, tracking visited vertices, and
% making data-dependent branching decisions. The SIMT (Single Instruction,
% Multiple Threads) execution model penalizes divergent control flow, as threads
% that take different branches must execute serially. Efficient GPU
% implementations must restructure these operations to minimize divergence while
% preserving correctness.

\para{Limitations of existing GPU ANNS systems} 
Existing GPU ANNS systems either lack updatability or suffer from poor
performance. \cagra~\cite{ootomo2024}, the current state-of-the-art GPU ANNS
system, achieves high query throughput by employing a carefully optimized graph
structure derived from NN-Descent. However, \cagra's graph construction
algorithm is batch-oriented, and the system is not designed for incremental
updates. In production settings where data arrives continuously, the inability
to update the index without full reconstruction is a critical limitation. 

BANG~\cite{Venkatasubba2025} is based on an updatable graph structure but
suffers from severe performance penalties as it employs product quantization
(PQ)~\cite{Jgou2011}~\footnote{PQ is a quantization technique that reduces
  vector size by decomposing the original vector into a Cartesian product of
independently quantized low-dimensional subspaces.} for compressing the
vectors. \bang extends the Vamana ANNS index~\cite{Subramanya2019}; this index
structure enables updates (although \bang currently does not implement index
updates). However, its reliance on Product Quantization (PQ) limits peak
performance.
% \zikun{Replace the following paragraph to: In \Cref{sec::quant}, we discuss
% in detail how PQ is not ideal for GPU vector indices.} \hunter{Good, but I
% think the tone needs to be a touch different - "not ideal" is too strong a
% claim.} 
In~\Cref{sec::quant}, we discuss in detail the limitations of product
quantization on GPUs.

%While PQ compresses vector storage, distance computation requires lookups into
%a codebook for each subquantizer. On GPUs, these scattered 4-byte reads
%trigger massive read amplification: loading a 32-byte memory sector to
%retrieve 4 bytes wastes 87.5\% of memory bandwidth. The codebook itself is too
%large to cache in shared memory for typical configurations, leaving \bang
%memory-bound on inefficient access patterns. Our experiments show \bang
%underperforms optimized implementations by up to twoorders of magnitude.
%\hunter{We should rephrase this paragraph - This feels too in the woods about
%the specifics of PQ IMO.}

Other GPU ANNS systems face their own constraints. GANNS~\cite{Sun2024}
implements HNSW but struggles with the algorithm's sequential construction
dependencies. SONG~\cite{Zhao2020} and GTS~\cite{Zhu2024} target different
index structures (fixed-rank graphs and trees, respectively) with different
trade-off profiles. None of these systems simultaneously achieve
state-of-the-art query performance, efficient construction, and support for
incremental updates.

% \para{Insights}
% \RThreeInline{W1}{}
% \RFourInline{W1}{\sysname builds on graph-ANNS techniques from
% DiskANN~\cite{Subramanya2019} and ParlayANN~\cite{Manohar2024}. It identifies
% a set of design principles for minimizing data movement and maximizing
% utilization on irregular, memory-bound GPU workloads. Each principle is
% counter to established techniques in CPU ANNS systems.}
% % and generalizes beyond ANNS to workloads
% % such as graph analytics and database query processing.}
%
% \begin{itemize}
%   \item \RThreeInline{W1}{} \RFourInline{W1}{\emph{Drop the visited-set hash
%    table.} Beam search conventionally uses a hash table to avoid revisiting
%    vertices. On a GPU this costs 512B of shared memory per query and caps
%    occupancy\RTwoInline{D2}{(the ratio of active vs.\ maximum schedulable
%    warps)}. Removing it results in a few redundant distance computations, but the
%    freed shared memory lets \sysname schedule more concurrent queries per
%   block, hiding memory latency and netting higher throughput.}
%
%   \item \RThreeInline{W1}{}\RFourInline{W1}{\emph{Quantization for GPUs is an
%       open problem.} Product Quantization (PQ)~\cite{Jgou2011}, the default
%       quantization scheme in prior GPU ANNS systems, incurs heavy read amplification
%       and random memory accesses on every codebook lookup. We present the first GPU
%     implementation of RaBitQ~\cite{Gao2024}, whose sequential loads and simple
%   arithmetic help increase arithmetic intensity.}
%
%   \item \RThreeInline{W1}{}\RFourInline{W1}{\emph{Smaller blocks beat larger ones.} For
%   irregular, memory-bound graph traversals, shrinking the thread block down to a
%   single warp on low-dimensional datasets maximizes memory-level parallelism:
%   more independent queries per SM hide pointer-chasing latency and increase
%   throughput.}
% \end{itemize}

\para{This paper} We present \sysname, a GPU-native ANNS system that addresses
the above challenges to achieve high query throughput while supporting dynamic
index updates. \sysname builds on graph-ANNS techniques from
DiskANN~\cite{Subramanya2019} and ParlayANN~\cite{Manohar2024}. It identifies a
set of design principles for minimizing data movement and maximizing
utilization on irregular, memory-bound GPU workloads. Each principle is counter
to established techniques in CPU ANNS systems. We make the following
contributions:

% \truncate{Jasper makes three major contributions. First, we devise a new
% lock-free batch-parallel construction algorithm optimized for block-level
% parallelism in GPUs based on \parlayann~\cite{Manohar2024}. This enables
% lock-free streaming insertions with best-in-class construction performance,
% making \sysname the first high-performance GPU ANNS system to support
% incremental updates. Second, to overcome the irregular access patterns of
% graph traversal, we perform a systematic analysis of greedy beam search on
% GPUs and find that high occupancy and small beam widths are the crucial
% components for achieving high performance in beam search. We present a tuned
% beam search kernel that removes all extraneous components and achieve up to
% \timesFasterThanCagra times faster query performance than \cagra, the
% state-of-the-art GPU ANNS index. Third, we present the first GPU
% implementation of RaBitQ quantization~\cite{Gao2024}. Through systematic
% analysis, we show that existing GPU quantization methods like product
% quantization fail to deliver speedups due to scattered memory accesses.
% RaBitQ avoids these pitfalls and increases arithmetic intensity, shifting
% ANNS away from the memory-bound regime and enabling higher throughput on very
% high-dimensional datasets.(combine these to the bullet points below)}

% We present \sysname, a GPU-native ANNS system that addresses the above
% mentioned challenges to achieve high query performance while supporting dynamic
% index updates. To support updatability, we use the batch-parallel construction
% algorithm from Manohar et al.~\cite{Manohar2024}. With modifications to make
% this algorithm amenable to block-level parallelism, this provides best-in-class
% construction time and allows for incremental index updates. To overcome the
% irregular access patterns of graph traversal, we perform a systematic analysis
% of greedy beam search on GPUs and find that high occupancy and small beam
% widths are the crucial components for achieving high performance in beam
% search. We present a tuned beam search kernel that removes all extraneous
% components and achieve up to \timesFasterThanCagra faster query performance
% than \cagra, the state-of-the-art GPU ANNS index. Finally, to overcome the
% memory-bound limitation of ANNS, we introduce the use of RaBitQ~\cite{Gao2024}
% quantization on GPUs. We present a systematic analysis of GPU quantization
% techniques and show that existing GPU quantization methods fail to yield
% speedups due to indirections and read amplification. We find that directly
% comparable vector quantization schemes such as RaBitQ achieve higher
% performance on large vector datasets and significantly increase the arithmetic
% intensity of the beam search, opening a new avenue for future optimizations.

% \para{Our approach} \prashant{This part of the intro needs rewriting. Need to
% make our insights and contributions exciting.} We present \sysname, a
% GPU-native ANNS system that achieves high performance while supporting dynamic
% index updates. \sysname builds on the Vamana graph
% index~\cite{Subramanya2019}, which offers a promising combination of
% strong query performance, theoretically grounded construction, and support for
% incremental insertions. Our key insight is that achieving peak GPU performance
% for this memory-bound workload requires co-designing the quantization scheme,
% memory access patterns, and kernel structure, piecemeal optimizations leave
% substantial performance on the table.

% \prashant{Add a new insights and contributions paragraph. This paragraph(s) is a make/break for the paper.}

% \para{Contributions} We make the following contributions:

\begin{itemize}

  \item \textbf{Batch-parallel GPU construction with support for incremental
    updates.} We devise a batch-parallel construction
    algorithm for GPU execution. Rather than using fine-grained locks that
    create serialization bottlenecks at high-degree vertices, our approach
    performs beam searches independently, accumulates candidate edges, sorts
    them by target vertex, and applies pruning in parallel without needing
    synchronization. \RTwoInline{D1}{The same algorithm drives both initial
    bulk construction and incremental inserts after the index is
    live, making \sysname the first GPU ANNS system to support 
    updates without a full rebuild.}

  \item \textbf{GPU-efficient quantization.} Quantization for GPUs is an
    open problem. Product Quantization (PQ)~\cite{Jgou2011}, the default
    scheme in prior GPU ANNS systems, incurs heavy read amplification and
    random memory accesses on every codebook lookup. We present the first GPU
    implementation of RaBitQ~\cite{Gao2024}, a quantization scheme that
    compresses vectors through randomized rotation and scalar quantization for
    up to 8$\times$ memory reduction; its sequential loads and simple
    arithmetic increase arithmetic intensity.

  \item \textbf{Optimized search kernel.} 
    % Drop the visited-set hash
    % table; smaller blocks beat larger ones. 
    Beam search conventionally uses a
    hash table to avoid revisiting vertices, but on a GPU this costs 512B of
    shared memory per query and caps occupancy; removing it costs only a few
    redundant distance computations while freeing shared memory to schedule
    more concurrent queries per block. We find that for smaller vectors block
    size and occupancy dominate performance, with peak throughput at 32 threads
    per block (a single warp) and 100\% occupancy, maximizing memory-level
    parallelism and hiding pointer-chasing latency (defined
    in~\Cref{subsec:memory}).

    % We analyze the beam search kernel
    % and identify that for smaller vectors compute occupancy and block size
    % dominate performance. Peak performance is reached at a block size of 32 and
    % 100\% occupancy due to better latency hiding between blocks in a GPU
    % streaming multiprocessor (SM) (defined in~\Cref{subsec:memory}). To achieve
    % this, we devise a new beam search kernel that minimizes transient memory usage
    % to maximize the number of queries launched per SM. The performance of this
    % kernel is validated through both empirical benchmarking and roofline
    % analysis~\cite{Williams2009}. The kernel achieves between 70\%-80\% of peak
    % possible performance for its arithmetic intensity and achieves up to 50\%
    % higher FLOPS/s compared to \cagra for the same query accuracy.

  \item \textbf{Optimized memory access patterns.} We introduce a tile-based
    loading scheme that issues blocked 16-byte loads across the threads in a
    warp simultaneously. Naive implementations either serialize loads through a
    single thread or issue element-wise loads across the warp (defined
    in~\Cref{subsec:memory}). Our approach partitions vectors into 16-byte
    chunks that are processed in parallel.

  \item \textbf{Systematic performance analysis.} We conduct a detailed
    empirical study of GPU ANNS optimization strategies. We characterize the
    trade-offs between per-query parallelism and memory-level parallelism,
    finding that optimal block sizes differ significantly across datasets.
    \iftruncate
    We
    perform roofline analysis~\cite{Williams2009} on the state-of-the-art
    search kernels and find that modern ANNS kernels are memory bound and
    execute at close to optimal throughput.
  \fi
    % Contrary to prior CPU-focused work~\cite{Coleman2021}, we find that graph
    % reordering provides negligible benefit when indices reside entirely in
    % GPU memory.

\end{itemize}

\para{Results}
Our evaluation on five standard ANNS benchmarks demonstrates:

\begin{itemize}

  \item \sysname achieves up to \timesFasterThanCagra$\times$ higher query
    throughput than \cagra, the state-of-the-art GPU index, while providing
    updatability that \cagra lacks.

  \item Compared to \bang, the previous state-of-the-art GPU Vamana
    implementation, \sysname delivers
    \lowerBangSpeedup–\higherBangSpeedup$\times$ higher throughput.

  \item On an A100, \sysname achieves peak throughput exceeding \fastestQuery queries/sec
    on the \bigann dataset and over \fastestOpenAIQuery queries/sec on
    1,536-dimensional \openai embeddings with RaBitQ quantization.

  \item \sysname's has the fastest incremental and batch GPU construction:
    \sysname has a peak insertion throughput of \fastestBuild insertions per
    second and is \avgConstruct faster on average than \cagra for index
    construction across five datasets.

  \item Our coalesced vector loading scheme improves memory access performance by up
    to \latencyReduction at low beam widths, with no throughput penalty at high
    beam widths.

    % an average of 2.394$\times$ faster than \cagra for construction.
    % \zikun{Average number seems a bit weird here.}
\end{itemize}


% \RFourInline{D3}{Reduce scope — reviewer flags this paragraph as
% "too general". Narrow to memory-bound irregular GPU workloads specifically;
% drop the "template for ANY irregular workload" framing.}
\para{Broader implications for ANNS on GPUs}
\RFourInline{D3}{The underlying techniques proposed in our work address fundamental challenges in GPU-accelerated ANNS workloads.}
% The underlying techniques proposed in our work address fundamental challenges in GPU-accelerated irregular workloads more broadly.
% Our analysis of the trade-off between per-query parallelism and memory-level parallelism applies to any GPU workload with low arithmetic intensity and data-dependent access patterns, such as graph analytics and database query processing. 
% The ineffectiveness of product quantization highlights a general principle: compression schemes designed for CPU cache hierarchies may perform poorly on GPUs, where coalesced sequential access is paramount. 
Our roofline analysis confirms that state-of-the-art kernels for \RFourInline{D3}{ANNS} already operate near the memory bandwidth ceiling, suggesting that future gains must come primarily from reducing data movement rather than algorithmic improvements alone.
%These insights provide a template for optimizing other memory-bound, irregular GPU workloads beyond similarity search.

% While our contributions target ANNS specifically, the underlying techniques address fundamental challenges in GPU-accelerated data structures and irregular workloads more broadly.
% Our analysis of the trade-off between per-query parallelism (larger thread blocks) and memory-level parallelism (more concurrent queries) applies to any GPU workload with low arithmetic intensity and data-dependent access patterns, such as graph analytics, sparse matrix operations, and database query processing.
% The ineffectiveness of product quantization on GPUs—due to scattered codebook lookups causing read amplification—highlights a general principle: compression schemes designed for CPU cache hierarchies may perform poorly on GPUs, where coalesced sequential access is paramount.
% Our tile-based loading scheme demonstrates that careful orchestration of memory requests across threads can reduce latency without sacrificing bandwidth, a technique applicable to any cooperative data structure traversal.
% Finally, our roofline analysis confirms that state-of-the-art GPU kernels for irregular workloads already operate near the memory bandwidth ceiling, suggesting that future performance gains must come primarily from reducing data movement through techniques like quantization rather than from algorithmic improvements alone.
% These insights provide a template for optimizing other memory-bound, irregular GPU workloads beyond similarity search.
   
% Nearest neighbor search (finding the closest k neighbors of a given data point)
% is a crucial problem in the fields of machine learning and information
% retrieval.
%
% In nearest neighbor search, high dimensional data such as files or images are
% reduced into lower dimensional vectors in a \textbf{metric space}, a space with
% well behaved rules for the distances between objects. The goal is to identify
% the $K$ closest neighbors in the space for a given query vector. Nearest neighbor
% search (NNS) is used in applications ranging from recommendation systems and
% image retrieval to anomaly detection and retrieval-augmented generation (RAG). 
%
% For low-dimensional datasets, spatial indexing structures such as quad trees
% and k-d trees enable efficient exact nearest-neighbor search, but these data
% structures degrade when storing high-dimensional data. As dimensionality
% increases, distances between data points tend to concentrate, and the ratio
% between the nearest and farthest neighbor distances approaches 1. This
% phenomenon, known as the curse of dimensionality~\cite{Minsky2017}, degrades
% the effectiveness of spatial pruning heuristics used in tree-based indices.
% Consequently, most branches must be explored, reducing theoretical speedups to
% linear scans. Practically, this also leads to poor cache efficiency and
% memory-bound behavior, as locality in high-dimensional spaces breaks down.
%
% As a solution to the curse of dimensionality, recent work has focused on
% approximate nearest neighbors search, where solutions are allowed to return an
% approximate solution that is $\epsilon$ away from the exact solution. ANNS
% indices have been traditionally broken down into three categories: inverted
% file indices (IVF), hash-based indices, and graph indices. Inverted file
% indices cluster vectors into groups called posting lists. For a target query,
% the closest posting lists are fetched, and the distance to all items in all
% posting lists is checked. Hash-based indices use locality-sensitive hashing to
% find similar vectors to a query. Graph indices construct a navigable search
% graph (NSG) which is traversed to locate the nearest neighbors. Recent
% work~\cite{ootomo2024, Subramanya2019} has shown
% graph indices to have the best recall/throughput
% tradeoff.~\cite{Subramanya2019,DBLP:journals/corr/LiZSWZL16,Manohar2024,
% Gollapudi2023}. 
%
% Constructing and querying these graph indices is computationally expensive,
% making GPUs an enticing target for hosting ANNS indices. 
% % Many workflows that use GPUs are already GPU accelerated: RAG, for example,
% % requires GPUs to perform model inference. Keeping the index on GPU can
% % improve the performance of the ANNS index and reduce the turnaround time for
% % servicing these queries as query results are already present on device.
% Constructing and querying ANNS indices on GPUs is difficult due to the
% unstructured access patterns of graph traversal. These indices are memory
% bound, as each dimension in a vector and vertex in the graph are read only
% once. The challenge then is to lay out and query the data structure efficiently
% in GPU memory. Recent works have accelerated ANNS by placing indices on GPU,
% but existing ANNS indices have not fully optimized for GPU memory, leaving them
% lacking in features and leaving some performance on the table. \bang, the
% state-of-the-art Vamana index for GPUs, uses product quantization, a
% quantization scheme that leads to read amplification on GPUs. \cagra, the
% state-of-the-art GPU index, is not updatable and performs no quantization,
% instead relying on efficient loads of the original vectors. This works well for
% small vectors but can lead to performance loss at low beam widths and large
% vector sizes, resulting in lost performance even when running at high
% utilization.
%
% In this paper, we take a holistic approach towards optimizing memory-bound
% operations on GPU. We look at three optimizations: graph reordering, vector
% quantization, and tile-based loading schemes. Using the Vamana ANNS index as
% the testbed, we evaluate each of these optimizations in terms of latency and
% throughput. We find: 
%
% \begin{itemize}
%     \item Compared to Coleman et al.~\cite{Coleman2021}, we find graph
%       reordering is not beneficial for indices that are located entirely in GPU
%       memory. \item On GPUs, product quantization leads to write amplification
%       and is significantly slower than exact vector queries due to the high
%       cost of indirection lookups on GPU. Directly comparable quantization
%       methods such as RaBitQ. are faster than exact search for large vector
%       sizes, but suffer for smaller vectors as the loads are not efficiently
%       tileable.
%     \item Directly issuing a series of loads from a tile can outperform naively
%   tiled and compiler-guided loads, resulting in faster lookups for low beam
% widths. \end{itemize}
%
% We integrate these optimizations into Jasper, the first updatable GPU ANNS
% index. Jasper is built on the Vamana graph index~\cite{Subramanya2019}
% and uses the batch parallel algorithm from Manohar et al.~\cite{Manohar2024}
% for construction. Compared to \bang, the previous state of the art Vamana index
% for GPUs, Jasper achieves of an order of magnitude higher query performance.
% Compared to \cagra, the state of the art ANNs index for GPUs, Jasper achieves
% comparable performance while allowing for streaming updates.
%
%
% \para{Results}
% \begin{itemize}
%   \item \sysname is up to $1.93\times $faster or competitive for batched query
%     throughput compared to \cagra, the state of the art GPU ANNS index.   \item
%     \sysname is $19-131\times$ (up to two orders of magnitude) faster in terms
%     of batched query throughput compared to \bang (current state-of-the-art
%     Vamana index on GPUs).
%   \item Quantization techniques such as Product Quantization have shown less
%     impact on GPUs due to random probes and non-aligned loads compared to CPU
%     ANNS indices, where they help in accelerating ANNS. We show that RaBitQ, a
%     recently introduced quantization technique, can be ported to GPUs
%     efficiently and enable faster queries. We present the first
%     GPU-implementation of the RaBitQ quantization technique.
%   \item We show that
%     updatability, a crucial feature for streaming ANNS workloads, can be
%     efficiently implemented on GPU. Our algorithm uses the batch update
%     procedure from \parlayann and degrades gracefully - increasing the size of
%     the index 20x reduces insert speed by less than 50\%.
%   \item Using tiles to issue blocked loads of 16-bytes minimizes load latency
%     while maintaining peak load throughput, improving memory loads by up to
%     14\% compared to other load request strategies. This technique is
%     applicable to any GPU data structure that is queried using cooperative
%     group tiles. Using this technique, we construct ANNS kernels that maintain
%     90\% memory and compute utilization. 
%   \item We find that graph reordering is
%     not helpful for GPU ANNS indices. Our optimized search kernels achieve 90\%
%     GDDR utilization, and large ANNS vectors are well suited to being loaded in
%     sectors. At this high utilization, memory pipelines are almost always busy,
%     and only necessary data is loaded. Changing the graph structure does not
%     improve the floor of necessary loads and thus doesn't significnalty affect
%     throughput. 
% \end{itemize}




==> vldb26-revision/preliminary.tex <==
\section{Preliminary}

% \prashant{TODO: cut redundant background to make room for the
% GPU-characteristics story.}
This section describes the GPU execution and memory models relevant to building
high-throughput ANNS indexes. We first explain the GPU execution model and how
work is scheduled on the GPU. We then explain the GPU memory hierarchy and how
it affects achieving peak performance. We then examine how these hardware
characteristics affect existing GPU ANNS systems and introduce the roofline
model~\cite{Williams2009} as a framework for analyzing their performance.


\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/graphs/GPU_arch.pdf}
        \caption{GPU Memory Hierarchy}
        \label{fig:gpu-memory}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/graphs/roofline.pdf}
        \caption{Roofline model}
        \label{fig:roofline-model}
    \end{subfigure}
    \caption{GPU memory hierarchy and roofline model.}
    \vspace{-1em}
\end{figure}

\subsection{GPU execution model} 

A diagram of the GPU architecture is shown in~\Cref{fig:gpu-memory}. A GPU
consists of multiple \defn{streaming multiprocessors (SMs)}, each capable of
hosting up to 1024 concurrent threads. 
% Threads are scheduled in groups of 32, referred to as \emph{warps}, which
% execute in a single-instruction, multiple-thread (SIMT) regime. 
Tasks on a GPU are executed in a chunk of work called a \textbf{kernel}. Each
kernel is a single-instruction, multiple-thread (SIMT) function that is
executed in parallel by every thread. GPU kernels are executed as collections
of \emph{thread blocks} on SMs, each containing up to 1024 threads. Within a
block, threads are subdivided into \emph{warps} (groups of 32 threads) that
share execution resources and issue memory operations cooperatively. As a
result, performance is maximized when threads within a warp follow identical
control flow and access contiguous or nearby memory locations. Warps can be
further subdivided into \emph{tiles} that divides the resources within a warp
for multiple jobs.

ANNS workloads expose fine-grained parallelism during nearest neighbor search
as pairwise distances can be computed independently in parallel. Each vector is
examined by a \emph{tile}, allowing multiple candidate vectors to be accessed
and evaluated in parallel. 
%
\iftruncate
Tiles are densely packed into warps: larger tiles increase per-probe
parallelism by examining more individual vectors faster, while smaller tiles
improve latency hiding by enabling additional concurrent memory requests within
a warp.
\fi

The optimal block and tile configuration depends on the characteristics of the
ANNS index, including memory layout, probe fan-out, and candidate filtering
costs.

%
% index probing
% and candidate evaluation, as each vertex loaded has multiple neighbors whose
% distances can be computed in parallel. Each neighbor is examined by a
% \emph{tile} of threads, allowing multiple candidate elements to be accessed and
% evaluated in parallel. Tiles are densely packed into warps: larger tiles
% increase per-probe parallelism by examining more individual vectors faster,
% while smaller tiles improve latency hiding by enabling additional concurrent
% memory requests within a warp. \hunter{I changed this, I have no idea what the
% old version was trying to say - it's tabbed out below.}
%

% ANNS workloads naturally expose fine-grained parallelism during index probing
% and candidate evaluation. To exploit this structure, we organize nearby
% \prashant{define nearby.} index entries into fixed-size groups that can be
% processed collectively. Each group is examined by a \emph{tile} of threads,
% allowing multiple candidate elements to be accessed and evaluated in parallel.
% Tiles are densely packed into warps: larger tiles increase per-probe
% parallelism by examining more candidates at once, while smaller tiles improve
% latency hiding by enabling additional concurrent memory requests within a warp.


%As with many GPU-resident data structures, index capacity is fixed at kernel
%launch time, since CUDA does not permit dynamic memory reallocation within a
%running kernel. \prashant{Is this true given that we can use Gallatin? What's
%the point of this paragraph?}


%\subsection{Where we stand/So far}. Currently, we have a fully implemented
%version of \parlayann (vamana) running on the GPU. On the BigANN10M dataset,
%we get construction performance of 60.4K vectors added per second, compared to
%a peak throughput of 38.9K for cuVS! Recall with L=64, R=64 is .9858@1,
%9.656@10, and 46.23@50 with full vectors. With all objects placed on host,
%throughput is 3.934K/s due to the increased cost of object transfer. PQ
%vectors are currently not working due to the distance calculation not using
%the distances between the centroids.


\subsection{GPU memory model} \label{subsec:memory} 
% \zikun{We should delete this paragraph. It goes too deep into details not related to ANN index.} 

\iftruncate
The design of concurrent GPU data structures is fundamentally constrained by
the underlying memory consistency model, which governs how memory operations
from different threads become visible to one another. In contrast to CPUs that
are sequentially consistent, modern GPUs implement a weak memory model based on
Relaxed Memory Ordering (RMO)~\cite{Alglave2015}. Under RMO, reads and writes
may be freely reordered unless explicitly constrained, and a read in one thread
that logically follows a write in program order from a different thread is not
guaranteed to observe that write without additional synchronization. GPUs
prioritize throughput over latency. With thousands of concurrent threads on
GPUs, enforcing strong ordering requires expensive coherence traffic.
\fi

% This relaxed behavior arises from the internal organization of GPU hardware.




%% saving for space.
% Each streaming multiprocessor contains an L1 cache. All threads within an SM share this cache, which is not coherent with L1
% caches on other SMs. These per-SM caches connect to a globally coherent L2
% cache, which in turn backs the GPU’s main memory (GDDR).
% \prashant{Need to add  a paragraph on shared memory and how critical it is for performance.}

%%END of space saving 

% \prashant{Commenting as it doesn't connects to the story.}
% A key consequence of this design is the absence of L1 cache invalidation. Once
% a cache line is resident in an SM’s L1 cache, it may be repeatedly reused even
% if newer values are written to L2 or GDDR by other SMs. Although L2 and global
% memory are coherent, an L1 hit can prevent a thread from observing updates that
% have already propagated to coherent memory. Stronger visibility guarantees can
% be provided via specialized \textbf{acquire-release} instructions. These
% operations enforce ordering and visibility constraints when accesses are
% properly annotated (e.g., atomic or acquire--release) and paired with an
% appropriate thread fence. When these conditions are satisfied, updates become
% globally observable across SMs, enabling correct coordination between threads
% operating on shared data structures.


Each streaming multiprocessor contains an L1 cache shared among all threads in the SM. This shared L1 cache is crucial for achieving high performance in GPU
applications. A section of this cache can be designated as \textbf{shared
memory}. Unlike a regular cache, this shared memory is directly addressable and
acts as both a scratchpad and a means of efficiently passing data between
threads in an SM. The amount of shared memory utilized affects the potential
\textbf{occupancy}, \RTwoInline{D2}{the ratio of active warps to the maximum
number of warps an SM can schedule.} Every block in a kernel requests the same
amount of shared memory; if the SM cannot fit enough blocks to keep its warp
slots full, occupancy drops and fewer warps run in parallel, leaving threads
idle.

% \prashant{Need to establish the relevance of the above to ANNS indexing.}

To achieve high performance on GPUs, we must design GPU kernels for ANNS index
construction and querying that efficiently utilize shared memory to maximize
occupancy. Specifically, we aim to keep all frequently used data in shared
memory and carefully select data structures that fit within the available
resources without reducing maximum occupancy.

% \hunter{Tuned this paragraph, I
% think this ties it together better. Can we remove info on the weak memory
% model? It's doesn't feel as relevant to the story now.}


\subsection{Roofline model}

The roofline model~\cite{Williams2009} is a simple, quantitative performance
model that bounds the attainable performance of an application on a given
architecture using two hardware limits: peak compute throughput and peak memory
bandwidth. Performance is expressed as a function of \emph{arithmetic
intensity}, defined as the ratio of useful operations to bytes transferred from
main memory. For low arithmetic intensity kernels, performance is limited by
memory bandwidth and grows linearly with arithmetic intensity; for high
intensity kernels, performance saturates at the hardware’s peak compute rate.
Graphically, these bounds form a ``roofline'' (see~\Cref{fig:roofline-model}):
a sloped bandwidth roof intersecting a flat compute roof, making it easy to see
whether a workload is memory-bound or compute-bound and how close it is to
hardware limits.

%\prashant{Use of AI is a confusing. Maybe we should just use ``arithmetic intensity''.}

The roofline model is widely used to guide performance optimization and
architectural analysis as it abstracts complex microarchitectural details into
a small set of measurable parameters. Optimizations that increase data reuse
(e.g., blocking, caching, fusion) move kernels rightward by increasing
arithmetic intensity, while vectorization, parallelism, and instruction-level
efficiency move kernels upward towards the compute roof. 
\iftruncate
Extensions of the model incorporate multiple memory levels, ceilings for
specific bottlenecks, and heterogeneous devices, but the core insight remains:
achievable performance is fundamentally constrained by the balance between
computation and data movement. This framing has proven effective for reasoning
about performance portability across CPUs, GPUs, and accelerators, and for
communicating optimization priorities in both systems and data-intensive
workloads. \emph{We use the roofline model to evaluate both the achieved and
  potential performance of ANNS indices on GPUs.}
\fi

% \prashant{Need to establish the relevance of the above to ANNS indexing.}


% In this section, we discuss the GPU execution and memory models as they pertain
% to the high throughput, concurrent data structures used in approximate nearest
% neighbor search (ANNS). We first summarize the GPU memory hierarchy and its
% consistency guarantees, then describe how the execution model influences the
% design of parallel index traversal and lookup primitives. We discuss the
% implications of these properties for existing GPU-based ANNS systems, and
% discuss the roofline model as a way of systematically evaluating the potential
% and achieved performance of parallel algorithms on GPUs.

% In this section, we discuss the related CPU and GPU ANN algorithms. These
% include the state of the Art CPU and GPU ANNS algorithms and the previous
% iterations of the vamana index, DiskANN~\cite{Subramanya2019} and
% \parlayann~\cite{Manohar2024} on which our construction and search algorithm
% are based. All indices against which we directly compare are included here.
% Other ANNS indices, tools, and quantization techniques are included in
% \Cref{sec::related}.

% Listing all related works worth mentioning. There are like 50 so will focus on diskANN and GPU related.
% \begin{itemize}
%     \item NSG
%     \item filteredDiskANN
%     \item scann
%     \item spann
% \end{itemize}


% \prashant{We might not need this here.}
% \para{\textbf{DiskANN}} DiskANN~\cite{Subramanya2019} is a graph-based index that performs ANN by constructing and querying a navigable search graph. The graph is queried by a greedy beam search in which a small number of close neighbors are held in memory, and in iterative steps the closest vertex to the target is queried for its neighbor list. Graph construction is done using the Vamana algorithm which iteratively performs a greedy search for nodes and tunes the graph based on the result of that search. The details of these algorithms are discussed in more detail in \Cref{sec::diskann}.
% In this algorithm, each vector in the dataset is represented by a vertex. This vertices are initialized to have random neighbors, and the graph is then iteratively improved. Each vertex in the graph is queried one at a time in random order. The nodes visited along the way are used to generate a new neighborhood for the vertex, and the vertex is bidirectionally attached to them. When the degree of a node becomes too large, a pruning algorithm calle d robustPrune is run. This pruning strategy admits only the closest neighbors and prunes any neighbors who have close 2-hop connectivity. The exact details of this algorithm are discussed in more detail in \cref{sec::diskann}.

% The original implementation of this algorithm could not efficiently delete as they leave holes in the graph that impact output quality. FreshDiskANN~\cite{https://doi.org/10.48550/arxiv.2105.09613} uses a lazy deletion algorithm to process deletes: nodes are marked as deleted but left in the graph, and when enough nodes are deleted a stop-the-world approach is used. The graph is frozen and the ingoing neighbors of each node are connected to all outgoing neighbors of each node, with robustPrune executed on all of them. As nodes do not store their incoming neighbors, this results in a costly traverse of the entire graph.

% IPDiskANN~\cite{https://doi.org/10.48550/arxiv.2502.13826} reduces the cost of deletions by performing them on-the-fly and in place. To generate the incoming neighbors of a deleted vertex, greedySearch is run. A parameter $c$ controls how densely the in and out-going neighbors are connected. The incoming neighbors of the deleted node are connected to the ANN results of the greedy search. The outgoing neighbors of the deleted node are connected to the visited set.

% All of these implementations are parallelized using locks, which adds unnecessary overhead to parallel operations. \parlayann~\cite{Manohar2024} uses a batched and lock-free insertion algorithm to efficiently add new nodes to the graph. More detail on this algorithm is given in \Cref{sec::parlay}.


% \prashant{Move this to eval/related work.}
% \para{\textbf{BANG}} \bang~\cite{Venkatasubba2025} extends the query execution of DiskANN to GPUs. \bang uses product quantization to reduce the size of the vectors. The quantized vectors are stored in GPU memory while the graph and full vector data are stored in DRAM. The entirety of a CTA is used for each query. One thread is used for each distance calculation, as distances can be calculated using only PQ table lookups. To process queries more efficiently, bloom filters are used to represent the visited list, lowering the memory requirements for searching.

% \paragraph{\textbf{NEOS}} NEOS~\cite{Huang2024} pins GPU memory in CPU user space and offers several optimzations to improve GPU buffer design such as pinning NVME memory, custom memcopies, and faster CPU-GPU polling. NEOS is not a vector manager but instead offers a buffer tool that can be used by other managers such as HSNW. NEOS uses a large unsorted buffer to aggreagate incoming requests; using the parallelism of an A100 and cuBLAS matrix operations, the entirety of the buffer can be checked with low latency. This allows for other vector managers to process streaming updates while only possessing a batch insertion API, which can make these applications more flexible without compromising throughput.

% \paragraph{\textbf{FAISS}} FAISS~\cite{FAISS} is a library of approximate nearest neighbor algorithms implemented by Facebook. This includes algorithms for inverted file indexes, product quantization, three-level quantization, HNSW, anisotropic vector quanitization, NSG, and binary multi-index hashing. This library also has an algorithm for executing on GPUs, with a GPU implmentation of fast k-selection from Johnson et al.~\cite{johnson2017billionscalesimilaritysearchgpus}. This algorithm uses an in-register bitonic sorting network to efficiently implement nearest-k neighbors over a given input list.  This algorithm, called \textit{k}-selection, is used to efficiently find the nearest neighbors for a query from a set of inverted lists. The $\rho$ nearest inverted lists are queried, with the result after \textit{k}-selection being written back.


% \paragraph{\textbf{HNSW}} HNSW~\cite{Malkov2020} constructs a probabilistic search graph akin to a skip list. In HNSW, the graph is split into levels. Each level of the graph is connected, with queries starting at the top level and bleeding down through the graph. The top level of the graph contains long range connections, with the lower level graphs having shorter and more dense edges. When new vertices are added to the graph a random roll is used to determine to how many levels the object will belong.

% \prashant{Move this to eval/related work.}
% \para{\textbf{CAGRA}} 
% \prashant{This description needs rew-writing.}
% CAGRA~\cite{ootomo2024} is a GPU ANNS algorithm built on top of NNDescent~\cite{Dong2011}. NNDescent takes a graph and iteratively improves the neighborhood of nodes by pulling new neighbors from their 2-hop neighborhood. This provides a well-connected ANNS query graph, but the degree is too high for use on GPU. To reduce the memory use, \cagra executes a pruning algorithm after the graph is constructed. This prune occurs in three phases. In the first phase, the edges of each node are sorted in ascending order by their length. This ordering is then used in the second phase as a proxy for distance, allowing for pruning to avoid the high cost of vector distance calculations. In the second phase, any nodes that are directly connected but have a good 2-hop route will have their edge clipped. Finally, the graph is duplicated and reversed, and the two mirrored graphs are merged together, with a final pruning pass being executed to reduce the size of the output. This produces a 

% \paragraph{\textbf{SONG}} SONG~\cite{Zhao2020} uses a fixed-rank ANN search graph for ANN queries. SONG uses bulk computation processing, a priority queue, and a cuckoo-filter to efficiently process queries.. To improve performance, the algorithm only considers vertices with a distance smaller than those in the current Top-K. This reduces the number of vertices that need to be remembered, but comes at the cost of additional compute to re-measure distances. They additionally optimize hash table/filter usage by deleting keys that fall out of the current topK, as these nodes can't be re-added to the search due to having too far of a distance from the query.

% \paragraph{\textbf{GTS}} GTS~\cite{Zhu2024} is a GPU tree-based ANN index for exact K-nearest neighbors. This tree is constructed using a bulk-synchronous algorithm. Along with the main tree structure, the node value for each vector is written into a table. Objects are mapped to nodes using a FFT pivot selection, and the list is partitioned to place the objects contiguously next to each other in device memory. This process repeats to further partition nodes until all leaves in the tree are sufficiently small. A bulk \textit{cache list} is used to record streaming updates until a sufficient number of updates are recorded. The entire tree structure is then recomputed. For queries, they utilize a batched algorithm based on iterative range queries: A list of the top-K closest nodes is kept, and all children in a level are considered unless their distance from the query falls outside of the top-K largest distance - this search is iteratively refined until the leaves are reached and a final set of top-K results can be extracted. During updates, new keys are held in a buffer that is checked during every query. If the buffer becomes too large, then entire tree is regenerated.


% \paragraph{\textbf{FusionANNs}} FusionANNs~\cite{305214} is a coprocessor vector index that uses the GPU as a helper for performing expensive distance comparisons. The index is based off of the posting lists used in SPANN - the authors find that the main limit to scalability in the original SPANN algorithm is the distance comparisons used when selecting the top-K from posting lists. Therefore, the product-quantized representation of the vectors is kept on GPU memory. Posting lists are generated by using hierarchical balanced clustering~\cite{Hartigan1979}. During a query, the CPU traverses the graph to find the closest posting lists to the target query. The IDs from these posting lists are sent to the GPU, and the distances for every item in the lists is calculated in parallel. This listing is returned to the CPU, where a heuristic re-ranking algorithm is executed to locate the best vectors. The full vectors are then loaded from SSD, and an exact distance comparison is executed to determine the final set. The code for FusionANNs is not publicly available.

% \paragraph{\textbf{LoRANN}} LoRANN~\cite{NEURIPS2024_b939da39} introduces a new clustering methods called reduced-rank regression (RRR). This method is a built-in replacement for product quantization, and can be used both in setting clusters and for querying the posting lists of a cluster from the IVF. In RRR, the data is processed as a full batch, with the goal of minimizing the value of $\beta_{RRR} = argmin_{\beta} \Vert Y-X\beta \Vert^2_F$, where $Y$ are the true nearest neighbors. A fast randomized algorithm is used to compute the nearest neighbors of the training set, and predictions are made via a matrix multiplication $\hat{y} = x^T\beta_{RRR}$. To perform operations efficiently, the training set is first cast into a low-dimensional space by taking the eigenvectors from PCA. The result of this is then quantized via 8-bit integer quantization. These operations can be efficiently processed on both CPU and GPU. In testing, the authors find that their implementation can replace PQ in FAISS to improve performance on high-dimensional vector datasets.

% \paragraph{\textbf{GGNN}} GGNN is a KNN-based nearest neighbors algorithm parallelized for use on GPUs. The algorithm is performed in hierarchical rounds, with subgraphs being iteratively merged into a final hierarchical search graph. The connection algorithm utilizes a greedy search that terminates when the best list cannot be improved.
% To optimize for the GPU, a per-block heap and priority queue are used for searching. When querying, an entire thread blocks is allocated for each key. To optimize their queries, \cagra introduces a slack value when running the greedy bea a slack value is used to stop queries from getting stuck in local minima.

% \prashant{Move this to eval/related work.}
% \paragraph{\textbf{GANNS}} GANNS~\cite{Yu2022} is an implementation of the NSW and HNSW graph algorithms optimized for GPUs. The main improvement is the use of lazy data structures - rather than maintain a priority queue, GANNS maintains two lists (frontier and visited) and only occasionally updates the lists to mark vertices as visited. They avoid the use of a hash table for marking visited vertices during queries, and use multiple thread blocks per query. The construction algorithm for these graphs are non-trivial to parallelize, so the authors build many small graphs in parallel and then sequentially merge them.



==> vldb26-revision/pseudocode/cudaBeam.tex <==
\RestyleAlgo{ruled}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\SetArgSty{textrm} 
\begin{algorithm}

unvisited\_frontier = []\\
visited = []\\
\ForEach{key \textbf{in} batch \textbf{in parallel}}{%
      frontier[key] = {<key,medoid, 0>} \tcp{Distances start unitialized}
}
calculate\_distances(frontier) \tcp{Set distances}
unvisited\_frontier = set\_difference(frontier, visited)\\
\While{unvisited\_frontier.size() != 0}{%
    live\_frontier = []\\
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{
        \tcp{Grab the first W from each key in the batch}
        live\_frontier[key] = unvisited\_frontier[key:key+W]  
    }
    candidates = []\\
    \ForEach{edge \textbf{in} live\_frontier \textbf{in parallel}}{%
    candidates[edge] = graph[edge]
    }
    calculate\_distances(candidates)\\
    sort\_by\_distance(candidates)\\
    frontier = merge(frontier, candidates)\\
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{%
        frontier[key] = clip(frontier[key], beam\_width) \tcp{clip to beam width}
    }
    visited = merge(visited, live\_frontier)\\
    unvisited\_frontier = set\_difference(frontier, visited)\\
}
\textbf{Return} \{frontier, visited\}
\caption{Cuda Beam search}
\label{pseudo::cudaBeam}
\end{algorithm}


==> vldb26-revision/pseudocode/cudaPrune.tex <==
\RestyleAlgo{ruled}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\SetArgSty{textrm} 
\begin{algorithm}

work_list_id = blockDim.x;\\
tile = cg::tiled_partition<thread_block>;\\
write\_index = 0;\\
index = 0;\\
my\_edges = edges[work\_list\_id];\\
node my\_vertex = my\_edges[0].source;\\

\tcp{Iterate until edge list is full.}
\While{write\_index < R && index < my\_edges.size()}{

    \uIf{my\_edges[index] == dead\_edge}{
        index++;\\
        continue;\\
    }

    \tcp{Only one thread writes output.}
    \uIf{threadIdx.x == 0}{
        graph[my\_vertex].edges[write\_index] = my\_edges[index].sink;
    }

    \ForEach{clippable\_edge \textbf{in} my\_edges[index+1:] \textbf{in parallel}}{

        p\_star = my\_edges[index].sink;
        p\_prime = clippable\_edge.sink;
    
    }
    
    
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{
        \tcp{Grab the first W from each key in the batch}
        live\_frontier[key] = unvisited\_frontier[key:key+W]  
    }
    candidates = []\\
    \ForEach{edge \textbf{in} live\_frontier \textbf{in parallel}}{%
    candidates[edge] = graph[edge]
    }
    calculate\_distances(candidates)\\
    sort\_by\_distance(candidates)\\
    frontier = merge(frontier, candidates)\\
    \ForEach{key \textbf{in} batch \textbf{in parallel}}{%
        frontier[key] = clip(frontier[key], beam\_width) \tcp{clip to beam width}
    }
    visited = merge(visited, live\_frontier)\\
    unvisited\_frontier = set\_difference(frontier, visited)\\
}
\textbf{Return} \{frontier, visited\}
\caption{Cuda robustPrune implementation}
\label{pseudo::cudaBeam}
\end{algorithm}


==> vldb26-revision/pseudocode/parlayANN.tex <==
\RestyleAlgo{ruled}

\begin{algorithm}
\SetArgSty{textrm} 

flipped$\_$edges = []\\
\ForEach{key \textbf{in} batch \textbf{in parallel}}{%
      visited$_{\texttt{key}}$ = beamSearch(key)\\
      neighbors$_{\texttt{key}}$ = robustPrune(visited$_{\texttt{key}}$)\\
      graph[key].edges =  neighbors$_{\texttt{key}}$\\
      flipped = flip$\_$edges(neighbors$_{\texttt{key}}$)\\
      flipped$\_$edges.append(flipped)\\
}
semisorted$\_$edges = semisort(flipped$\_$edges)\\
\ForEach{key, edges \textbf{in} semisorted\_edges \textbf{in parallel}}{
  \uIf{graph[key].size() + len(edges) <= R}{
    graph[key].edges += edges
  } \Else {
    pruned = robustPrune(graph[key].edges+edges)\\
    graph[key].edges = pruned
  }

}
\label{pseudo::parlayANN}
\caption{Batch insertion in \parlayann}
\end{algorithm}


==> vldb26-revision/quantization.tex <==

\section{Vector quantization}
\label{sec::quant}

Modern embedding models produce vectors spanning hundreds to thousands of
dimensions, with per-vector sizes ranging from 96 bytes to over 6000 bytes as
shown in \bigann benchmarks~\cite{Simhadri2022}. ANNS is
memory-bound: each vector element is read once, used for a single arithmetic
operation, and discarded. Reducing vector size directly improves query
throughput.

% Modern ANNS benchmarks and production workloads are commonly composed of image,
% text, and multimodal embeddings that are encoded as vectors spanning hundreds
% to thousands of dimensions. The \bigann benchmark~\cite{Simhadri2022}
% illustrates the wide range of vector sizes encountered in practice: the smallest
% dataset size uses 96 bytes per vector, while the largest datasets use more than
% 6000 bytes per vector. 
%
% Reducing the size of each vector can improve query throughput as less data is
% transferred. ANN indices are often bounded by the volume of data that must be
% loaded from memory, as the distance calculations are not computationally
% complex: during distance comparisons, each index of a vector is used only once
% before being discarded. Shrinking the in-memory representation of a vector
% directly reduces both memory footprint consumed per query, which can in turn
% lead to an increase in query throughput as these lookups dominate query
% performance.

To reduce per-vector storage and I/O costs while preserving search accuracy, we
consider \emph{quantization}, which compresses vectors while approximately
preserving distances. The most widely used approach for ANNS is \emph{product
quantization} (PQ)~\cite{Jgou2011}. PQ divides each vector into $K$ disjoint
subvectors and quantizes each independently using a small codebook of 256
centroids. Each subvector is then encoded as a single byte indicating its
nearest centroid, compressing a high-dimensional vector to just $K$ bytes.
Distance computation uses a precomputed \emph{lookup table} storing
centroid-to-centroid distances for each subspace. This results in significant
compression with modest accuracy loss, as error arises only from the
approximation of each subvector by its nearest centroid.

% To reduce the per-vector storage while preserving high search accuracy, we use
% \textbf{quantization}, a technique that casts vectors into a lower dimensional
% space while preserving distance metrics as closely as possible. The most
% commonly used quantization method for vector quantization for ANN is
% \textbf{product quantization} (PQ)~\cite{Jgou2011}. PQ decomposes the original
% vector space into a Cartesian product of low-dimensional subspaces and
% independently quantizes each subspace. Concretely, product quantization trains
% $K$ independent quantizers, each of which is a small k-means model with 256
% clusters. Each of these quantizers trains on one of the disjoint subspaces,
% with each subvector of the original data base vectors being encoded by the
% index of its closest centroid. As an example, a product quantizer compressing
% down to 32 dimensions would have 32 subspaces, with each quantized vector being
% composed of 32 uint8\_t that represent the 32 closest centroids in each
% subspace. Comparisons between quantized vectors are done via the use of a
% lookup table that records the distances between each pair of centroids in every
% subspace. This approach yields significant compression while preserving most
% distance calculations, as the only source of error is the distance between a
% subvector and its centroid. \hunter{The PQ example can be clipped for space ?}

Although PQ compresses vectors effectively, its \emph{lookup table} access
pattern results in lower throughput on GPUs. GPU memory is organized into
32-byte \textit{sectors} that are loaded atomically—reading a single 4-byte
distance entry wastes the remaining 28 bytes, causing $8\times$ read
amplification. A straightforward solution is to place the lookup table in
shared memory, but even a modest configuration ($K=32$) requires
$32\times256\times256\times4$ bytes (8 MB), far exceeding shared memory
capacity. We implemented PQ in \sysname but found that throughput was 
strictly worse than unquantized search for all configurations tested. Similar
conclusions regarding the PQ performance on GPU has been presented in prior
research~\cite{ootomo2024}.

% Although product quantization can compress vector into compact codes, the
% lookup table access pattern used in PQ can paradoxically result in lower
% throughput when run on GPUs. On the GPU, memory is organized into
% \textit{sectors} of 32 bytes that are loaded contiguously - when any data from
% a sector is needed the entire sector must be brought in. This can read to read
% and write amplification when only a small part of each sector is used. While
% the PQ vector itself can be efficiently loaded, the lookup table poses a more
% significant issue. Each distance stored in the lookup table requires a read of
% only 4 bytes. Since the other 28 bytes in the sector won't be used, this
% results in an 8x read amplification for all queries to the lookup table. A
% natural solution to this would be to place the table in shared memory, a
% section of L1 cache directly managable on the GPU. However, even with a small
% encoding such as K=32, the PQ lookup table will require
% $32\times256\times256\times4$ bytes. This is 8 megabytes, the size of the
% entire l2 cache on modern GPUs and far too large to fit in shared memory. We
% implemented product quantization in Jasper, but do not use it in the final
% approach as throughput is strictly worse for all PQ sizes tested.
% \hunter{Example here could be simplified to - even the smallest practical sizes
% use 8 Megabytes of table, far too large to store in shared memory.}


% \begin{itemize}
%     \item For many ann datasets, vectors are large
%     \item \bigann benchmarks run from 96 to more than 6000 bytes.
%     \item reduceing the size of each vector improves query throughput as less data is transferred
%     \item We can reduce the size of the vectors without significantly reducing accuracy using quantization.
%     \item explain quantization of vectors in more detail
%     \item Start new subsection on product quantization
%     \item cite original paper
%     \item Product quantization compresses the vectors by clustering them using k-means clustering, and replacing each vector by the centroids that it is clustered to.
%     \item Each vector is sliced into $K$ subvectors, and a clustering algorithm on each set of subvectors. This algorithm maps each subvector to one of 256 clusters (storable in a uint8\_t).
%     \item The distances between the centroids of each cluster are calculated and stored in a lookup table
%     \item To compare two vectors in the quantized space, we iterate through each vector for each pair. For each pair of centroids we lookup the distance in the lookup table and add it to the running sum.
%     \item GPU lookup tables: Using product quantization, we can reduce the size of each vector to 32 bytes. However, using product quantization actually results in slower queries due to the lookup table.\
%     \item the quantized vectors can be efficiently loaded as the entire vector is contiguous in memory.
%     \item the lookup table is not contiguous and not efficient - it requires a series of random, small hops that cannot be loaded efficiently on GPU.
%     \item This results in a slowdown when using PQ.
%     \item We could fix this by storing the lookup table in shared memory, but it is too large - 256*256*32*4 = 8MB. This is the size of the entire l2 cache, far too large for the shared memory and even too large for the constant memory.
% \end{itemize}

\subsection{RaBitQ quantization}

% \begin{table}[t]
%     \centering
%     \begin{tabularx}{\columnwidth}{c X c} % X = column that expands
%         \hline
%         Variable Name & Description \\
%         \hline
%         $m$ & Quantize bits per dimension \\
%         $c$ & Centroid vector \\
%         $v$ & Original data vector \\
%         $q$ & Original query vector \\
%         $o$ & Rotated and normalized $v-c$ \\
%         $\bar{o}$ or \texttt{data} & Quantized data vector \\
%         $\Delta_x$ & The rescaling factor of $\bar{o}$ from $o$ \\
%         % \texttt{data\_add} & $||v-c||^2 + 2\cdot ||v-c||^2 \cdot {\langle c, \bar{o} \rangle \over \langle o, \bar{o} \rangle}$ \\
%         % \texttt{data\_rescale} & $-2\cdot \Delta_x / \langle o, \bar{o} \rangle$\\
%         % \texttt{rotated\_query\_vector} & Rotated and normalized $q-c$ \\
%         % \texttt{query\_add} & $||q-c||^2$ \\
%         % \texttt{query\_sumq} & $\sum (q-c) \cdot {2^{m-1}-1\over 2}$ \\
%         \hline
%     \end{tabularx}
%     \caption{RaBitQ variable definitions.}
%     \label{table:rabitq_variables}
% \end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/graphs/rabitq_distance.pdf}
%     \caption{RaBitQ distance estimation between a quantized data vector and a query vector.}
%     \label{fig:rabitq_distance}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/graphs/rabitq_memory_load.pdf}
    \caption{During L2 distance calculation, RaBitQ loads query vector and its
    metadata from shared memory, and it loads quantized data vector and its
  metadata from global memory.}
    \label{fig:rabitq_load}
\end{figure}

To effectively use quantization on the GPU, we must avoid random memory
accesses during distance computation. Previous GPU implementations treat
quantization as a trade-off: smaller vectors and lower memory I/O at the cost
of lower throughput~\cite{Venkatasubba2025, ootomo2024}. We show this trade-off
is not fundamental. \sysname employs RaBitQ~\cite{Gao2024}, a quantization
method that is well suited for GPUs. RaBitQ requires only sequential memory
access, simple arithmetic, and requires no lookup tables.

% In order to effectively use quantization on the GPU, we must avoid random
% accesses while computing the distance between two quantized vectors. Previous
% GPU-based implementations of quantization treat vector size and query speed as
% a trade-off: in exchange for their smaller space usage, quantized vectors
% always give worse or similar throughput compared to exact distance
% calculations~\cite{Venkatasubba2025, ootomo2024}. Our work shows that with the
% correct quantization technique, GPU vector indices can achieve higher
% throughput with a smaller memory footprint. In Jasper, we use
% RaBitQ~\cite{Gao2024}, a vector quantization method that requires no external
% lookups during distance calculations. This allows for the vectors to be
% directly compared in one round of memory loads, maximizing query performance on
% the GPU.

RaBitQ estimates the distance using the inner product between the quantized
data vector with the query vector. 
% \Cref{table:rabitq_variables} shows how the
% related variables and quantized vector are calculated. 
We define the following variables: $m$ is the number of quantized
bits per dimension, $c$ is the centroid vector, $v$ is the original data vector,
$q$ is the original query vector, $o$ is the rotated and normalized data vector 
$v-c$, $\bar{o}$ is the quantized data vector, and $\Delta_x$ is the rescaling 
factor of $\bar{o}$ from $o$.

During data quantization, RaBitQ compresses the
data vectors by first normalizing them and applying a random rotation matrix.
With high dimensional vectors, any rotated dimensions are likely tightly
clustered around 0: according to the Johnson-Lindenstrauss
lemma~\cite{Johnson1984}, the value of any coordinate is no further than
$\frac{2}{\sqrt{D}}$ away from 0 with high probability. This allows RaBitQ to
treat each dimension as an unbiased distribution and enables simple scalar
quantization. RaBitQ encodes each dimension with $m$ bits along with two
floating point metadata: \texttt{data\_add} and \texttt{data\_rescale}
, where they correspond to  $||v-c||^2 + 2\cdot ||v-c||^2 \cdot {\langle c, \bar{o} 
\rangle \over \langle o, \bar{o} \rangle}$ and $-2{\Delta_x \over \langle o, \bar{o}
\rangle}$. These precomputed values save computation during distance estimation.
In total, the size of the quantized vector is $\text{\#dims} \cdot m\,\text{
bits} + 2\cdot\mathrm{sizeof}(\text{float})$.

During querying, RaBitQ applies the same rotation matrix to the query vector,
and RaBitQ calculates each query vector's metadata: \texttt{query\_add} and
\texttt{query\_sumq}, where they correspond to $||q-c||^2$ and $\sum (q-c) 
\cdot {2^{m-1}-1\over 2}$. \Cref{fig:rabitq_load} shows how RaBitQ estimates
distances solely based on quantized vectors and rotated query vectors. The
RaBitQ estimator reduces the L2 distance calculation to estimating the inner
product between the quantized data vector (\texttt{data}) and rotated query
vector (\texttt{rotated\_query\_vector}). This process estimates the vector
distance without branching or randomized memory accesses while most of the
values are pre-computed, which makes it highly suitable for GPU execution.
RaBitQ's sequential memory access during distance calculation also allows us to
utilize the same loading technique for exact vector loading
in~\apxref{sec::microbenchmark}{Appendix~E}.

\sysname integrates GPU-accelerated RaBitQ. RaBitQ achieves $2\times$
compression for 8-bit vectors and up to $8\times$ for 32-bit vectors. On
datasets with large dimensions, our results demonstrate that \sysname with
RaBitQ performs significantly better than our exact distance calculation
version. In~\apxref{sec::microbenchmark}{Appendix~E}, we perform a detailed analysis between
RaBitQ's performance and PQ's performance.




==> vldb26-revision/related.tex <==
\section{Related work}

\label{sec::related}

In this section, we discuss the current state of the art in ANNS indexes that
are not directly evaluated against \sysname. These are indexes that are either
1) superseded in performance by the current state-of-the-art, 2) do not have a
publicly available implementation, or 3) are complementary to ANNS but not
directly comparable.

% Listing all related works worth mentioning. There are like 50 so will focus on diskANN and GPU related.
% \begin{itemize}
%     \item NSG
%     \item filteredDiskANN
%     \item scann
%     \item spann
% \end{itemize}


% \paragraph{\textbf{DiskANN}} DiskANN~\cite{Subramanya2019} is a graph-based index that performs ANN by constructing and querying a navigable search graph. The graph is queried by a greedy beam search in which a small number of close neighbors are held in memory, and in iterative steps the closest vertex to the target is queried for its neighbor list. The graph is constructed using the Vamana algorithm, which is discussed in more detail in \Cref{sec::diskann}.
% % In this algorithm, each vector in the dataset is represented by a vertex. This vertices are initialized to have random neighbors, and the graph is then iteratively improved. Each vertex in the graph is queried one at a time in random order. The nodes visited along the way are used to generate a new neighborhood for the vertex, and the vertex is bidirectionally attached to them. When the degree of a node becomes too large, a pruning algorithm calle d robustPrune is run. This pruning strategy admits only the closest neighbors and prunes any neighbors who have close 2-hop connectivity. The exact details of this algorithm are discussed in more detail in \cref{sec::diskann}.

% % The original implementation of this algorithm could not efficiently delete as they leave holes in the graph that impact output quality. FreshDiskANN~\cite{https://doi.org/10.48550/arxiv.2105.09613} uses a lazy deletion algorithm to process deletes: nodes are marked as deleted but left in the graph, and when enough nodes are deleted a stop-the-world approach is used. The graph is frozen and the ingoing neighbors of each node are connected to all outgoing neighbors of each node, with robustPrune executed on all of them. As nodes do not store their incoming neighbors, this results in a costly traverse of the entire graph.

% % IPDiskANN~\cite{https://doi.org/10.48550/arxiv.2502.13826} reduces the cost of deletions by performing them on-the-fly and in place. To generate the incoming neighbors of a deleted vertex, greedySearch is run. A parameter $c$ controls how densely the in and out-going neighbors are connected. The incoming neighbors of the deleted node are connected to the ANN results of the greedy search. The outgoing neighbors of the deleted node are connected to the visited set.

% % All of these implementations are parallelized using locks, which adds unnecessary overhead to parallel operations. \parlayann~\cite{Manohar2024} uses a batched and lock-free insertion algorithm to efficiently add new nodes to the graph. More detail on this algorithm is given in \Cref{sec::parlay}.

% \bang~\cite{Venkatasubba2025} extends the query execution of diskANN to GPUs. The product quantized vectors are stored in GPU memory, with the graph and full vector data stored in DRAM. To process queries more efficiently, bloom filters are used to represent the visited list, lowering the memory requirements for searching.


\para{\textbf{FAISS}} FAISS~\cite{FAISS} is a library for efficient similarity
search and clustering of vectors. It provides a broad collection of approximate
and exact nearest neighbor algorithms, with efficient CPU and GPU
implementations. FAISS supports multiple indexing strategies and techniques,
including inverted file indexes, product quantization, three-level
quantization, HNSW, anisotropic vector quanitization, NSG, and binary
multi-index hashing. On GPUs, FAISS leverages massive parallelism to accelerate
both index construction and query processing, making it a common choice for
large-scale similarity search workloads.



% % \paragraph{\textbf{HNSW}} HNSW~\cite{Malkov2020} constructs a probabilistic search graph akin to a skip list. In HNSW, the graph is split into levels. Each level of the graph is connected, with queries starting at the top level and bleeding down through the graph. The top level of the graph contains long range connections, with the lower level graphs having shorter and more dense edges. When new vertices are added to the graph a random roll is used to determine to how many levels the object will belong.

% \paragraph{\textbf{CAGRA}} \cagra~\cite{ootomo2024} is a GPU ANN algorithm built on top of NNDescent~\cite{Dong2011}. NNDescent takes a graph and iteratively improves the neighborhood of nodes by pulling new neighbors from their 2-hop neihgborhood. This provides a good ANN query graph, but the degree is too high for use on GPU. To reduce the memory use, \cagra executes a pruning algorithm after the graph is constructed. This prune occurs in three phases. In the first phase, the edges of each node are sorted in ascending order by their length. This ordering is then used in the second phase as a proxy for distance. In the second phase, any nodes that are directly connected but have a good 2-hop route will have their edge clipped. To avoid PQ vector comparisons in this phase, the distance between two nodes is approximated by the ranking of their edge in the outgoing vertex's edge list. This allows for this phase to be executed quickly inside of GPU memory. Finally, the graph duplicated and reversed, and the two graphs are merged together, with a final pruning pass being executed to reduce the size.

\para{\textbf{SONG}} SONG~\cite{Zhao2020} is a GPU ANNS that uses a fixed-rank
ANN search graph for ANN queries. SONG uses bulk computation processing, a
priority queue, and a cuckoo-filter to efficiently process queries. To improve
performance, the algorithm only considers vertices with a distance smaller than
those in the current Top-K. This reduces the number of vertices that need to be
remembered, but comes at the cost of additional compute to re-measure
distances. They additionally optimize hash table/filter usage by deleting keys
that fall out of the current top-\textit{K}, as these nodes can't be re-added
to the search due to having too far of a distance from the query.

\para{\textbf{GTS}} GTS~\cite{Zhu2024} is a GPU tree-based ANN index for exact
K-nearest neighbors. This tree is constructed using a bulk-synchronous
algorithm. Along with the main tree structure, the node value for each vector
is written into a table. Objects are mapped to nodes using a FFT pivot
selection, and the list is partitioned to place the objects contiguously next
to each other in device memory. This process repeats to further partition nodes
until all leaves in the tree are sufficiently small. A bulk \textit{cache list}
is used to record streaming updates until a sufficient number of updates are
recorded. The entire tree structure is then recomputed. For queries, they
utilize a batched algorithm based on iterative range queries: A list of the
top-$K$ closest nodes is kept, and all children in a level are considered
unless their distance from the query falls outside of the top-$K$ largest
distance - this search is iteratively refined until the leaves are reached and
a final set of top-$K$ results can be extracted. During updates, new keys are
held in a buffer that is checked during every query. If the buffer becomes too
large, then entire tree is regenerated.

\para{\textbf{NEOS}} NEOS~\cite{Huang2024} is an ANNS tool library that pins
GPU memory in CPU user space and offers several optimizations to improve GPU
buffer design such as pinning NVME memory, custom CPU to GPU memory copies, and
faster CPU-GPU polling. NEOS is not a vector index but instead is a buffer tool
that can be used by other indices such as HSNW. NEOS uses a large unsorted
buffer to aggreagate incoming requests; using the parallelism of an A100 and
cuBLAS matrix operations, the entirety of the buffer can be checked with low
latency. This allows for other vector managers to process streaming updates
while only possessing a batch insertion API, which can make these applications
more flexible without compromising throughput.

\para{\textbf{FusionANNs}} FusionANNs~\cite{305214} is a coprocessor vector
index that uses the GPU as a helper for performing expensive distance
comparisons. The index is based off of the posting lists used in SPANN - the
authors find that the main limit to scalability in the original SPANN algorithm
is the distance comparisons used when selecting the top-$K$ from posting lists.
Therefore, the product-quantized representation of the vectors is kept on GPU
memory. Posting lists are generated by using hierarchical balanced
clustering~\cite{Hartigan1979}. During a query, the CPU traverses the graph to
find the closest posting lists to the target query. The IDs from these posting
lists are sent to the GPU, and the distances for every item in the lists is
calculated in parallel. This listing is returned to the CPU, where a heuristic
re-ranking algorithm is executed to locate the best vectors. The full vectors
are then loaded from SSD, and an exact distance comparison is executed to
determine the final set. The code for FusionANNs is not publicly available.

\para{\textbf{LoRANN}} LoRANN~\cite{NEURIPS2024_b939da39} introduces a new
clustering methods called reduced-rank regression (RRR). This method is a
built-in replacement for product quantization, and can be used both in setting
clusters and for querying the posting lists of a cluster from the IVF. In RRR,
the data is processed as a full batch, with the goal of minimizing the value of
$\beta_{RRR} = argmin_{\beta} \Vert Y-X\beta \Vert^2_F$, where $Y$ are the true
nearest neighbors. A fast randomized algorithm is used to compute the nearest
neighbors of the training set, and predictions are made via a matrix
multiplication $\hat{y} = x^T\beta_{RRR}$. To perform operations efficiently,
the training set is first cast into a low-dimensional space by taking the
eigenvectors from PCA. The result of this is then quantized via 8-bit integer
quantization. These operations can be efficiently processed on both CPU and
GPU. In testing, the authors find that their implementation can replace PQ in
FAISS to improve performance on high-dimensional vector datasets.

% \paragraph{\textbf{GGNN}} GGNN is a KNN-based nearest neighbors algorithm parallelized for use on GPUs. The algorithm is performed in hierarchical rounds, with subgraphs being iteratively merged into a final hierarchical search graph. The connection algorithm utilizes a greedy search that terminates when the best list cannot be improved.
% To optimize for the GPU, a per-block heap and priority queue are used for searching. Entire thread blocks are allocated for individual keys. In queries, a slack value is used to stop queries from getting stuck in local minima.

% \paragraph{\textbf{GANN}} GANN is an implementation of the NSW graph algorithm optimized for GPUs. The main improvement is the use of lazy data structures - rather than maintain a priority queue, GANN maintains two lists (frontier and visited) and only occasionally updates the lists to mark vertices as visited. They avoid the use of a hash table for marking visited vertices during queries, and use multiple thread blocks per query. The construction algorithm for an NSW graph is non-trivial to parallelize, so the authors build many small graphs in parallel and then sequentially merge them.
%\subsection{Where we stand/So far}. Currently, we have a fully implemented version of \parlayann (vamana) running on the GPU. On the BigANN10M dataset, we get construction performance of 60.4K vectors added per second, compared to a peak throughput of 38.9K for cuVS! Recall with L=64, R=64 is .9858@1, 9.656@10, and 46.23@50 with full vectors. With all objects placed on host, throughput is 3.934K/s due to the increased cost of object transfer. PQ vectors are currently not working due to the distance calculation not using the distances between the centroids.


==> vldb26-revision/title.tex <==
\title{GPU-Accelerated ANNS: Quantized for Speed, Built for Change}


\author{Hunter McCoy}
\affiliation{%
  \institution{Northeastern University}
  \city{Boston}
  \country{United States}
  \postcode{02115}
}
\email{mccoy.hu@northeastern.edu}

\author{Zikun Wang}
\affiliation{%
  \institution{Northeastern University}
  \city{Boston}
  \country{United States}
  \postcode{02115}
}
\email{wang.zikun@northeastern.edu}


\author{Prashant Pandey}
\affiliation{%
  \institution{Northeastern University}
  \city{Boston}
  \country{United States}
  \postcode{02115}
}
\email{p.pandey@northeastern.edu}

